Stable Reinforcement Learning for Optimal Frequency Control: A Distributed Averaging-Based Integral Approach

Frequency control plays a pivotal role in reliable power system operations. It is conventionally performed in a hierarchical way that first rapidly stabilizes the frequency deviations and then slowly recovers the nominal frequency. However, as the generation mix shifts from synchronous generators to renewable resources, power systems experience larger and faster frequency fluctuations due to the loss of inertia, which adversely impacts the frequency stability. This has motivated active research in algorithms that jointly address frequency degradation and economic efficiency in a fast timescale, among which the distributed averaging-based integral (DAI) control is a notable one that sets controllable power injections directly proportional to the integrals of frequency deviation and economic inefficiency signals. Nevertheless, DAI do not typically consider the transient performance of the system following power disturbances and has been restricted to quadratic operational cost functions. This manuscript aims to leverage nonlinear optimal controllers to simultaneously achieve optimal transient frequency control and find the most economic power dispatch for frequency restoration. To this end, we integrate reinforcement learning (RL) to the classic DAI, which results in RL-DAI. Specifically, we use RL to learn a neural network-based control policy mapping from the integral variables of DAI to the controllable power injections which provides optimal transient frequency control, while DAI inherently ensures the frequency restoration and optimal economic dispatch. Compared to existing methods, we provide provable guarantees on the stability of the learned controllers and extend allowable cost functions to a much larger class. Simulations on the 39-bus New England system illustrate our results.

==> Secondary Control_Arxiv/DAI.tex <==
We start this section by briefly reviewing distributed averaging-based integral (DAI) control and then generalizing it to account for nonlinear control laws. We show that the closed-loop system is stable as long as the nonlinearity satisfies conditions on continuity and monotonicity. Interestingly, the steady-state performance objectives are still achieved under our proposed generalized DAI even for nonquadratic cost functions provided that the gradients of the cost functions on individual buses satisfy a certain condition, which we describe below.

\subsection{Review and Generalization of DAI}
DAI control~\cite{Zhao2015acc, Johannes2016ecc, SCHIFFER2017auto, weitenberg2018exponential} is an established choice of frequency control strategy  to meet the steady-state performance objectives discussed in Section~\ref{ssec:metric}.  However, most works restrict the cost functions to be quadratic, i.e., 
\begin{align}\label{eq:cost-quad}
    C_i(u_i) =\dfrac{1}{2}c_i u_i^2\,,\qquad\forall i\in\mathcal{N}\,,
\end{align}
where $c_i>0$ is the cost coefficient. With the cost functions given by \eqref{eq:cost-quad}, the power injections $\boldsymbol{u}$ in the system \eqref{eq:sys-dyn-vec} under DAI are
\begin{subequations}\label{eq:DAI}
\begin{align}\label{eq:u(s)-linear}
    u_i(s_i) = k_i s_i\,,\qquad\forall i\in\mathcal{N}\,,
\end{align}
with 
\begin{align}\label{eq:DAI-s}
    \dot {s}_{i} =&-2 \pi f_0\omega_i -c_i \sum_{j=1}^n Q_{ij}\left(c_i u_i-c_j u_j\right)\,,
\end{align}
\end{subequations}
where $k_i>0$ is a tunable control gain and $Q_{ij}\geq0$ is the weight associated with an undirected connected communication graph $\left(\mathcal{V},\mathcal{E}_\mathrm{Q} \right)$ (not necessarily the same as the physical system) such that $Q_{ij}=Q_{ji}>0$ if buses $i$ and $j$ communicate, i.e., $\{i,j\} \in\mathcal{E}_\mathrm{Q} \subset \Set*{\{i,j\}}{i,j\in\mathcal{N},i\not=j}$, and $Q_{ij}=Q_{ji}=0$ otherwise, $\forall i,j\in\mathcal{N}$. 

The core idea behind DAI is that the control dynamics can settle down only if the nominal frequency restoration, i.e., $\omega_i=0$, $\forall i\in\mathcal{N}$, and the identical marginal costs, i.e., $\nabla C_i (u_i) =c_i u_i=c_j u_j= \nabla C_j (u_j)$, $\forall i,j\in\mathcal{N}$, are simultaneously achieved. Thus ensuring  $\boldsymbol{\omega}^\ast=\mathbbold{0}_n$ and $\boldsymbol{u}^\ast$ is the solution of the optimal steady-state economic dispatch problem \eqref{eq:opt-ss}.

However, DAI in \eqref{eq:DAI} does not address the transient behavior of the system. Therefore, trajectories that eventually reaches the equilibrium may have poor transient performances. Thus, it is desirable to modify it so that we have better flexibility in improving the transient performance. Inspired by the fact that the control policy $u_i(s_i)$ of DAI in \eqref{eq:u(s)-linear} is directly proportional to the integral variable $s_i$, we generalize DAI by allowing $u_i(s_i)$ to be any Lipschitz continuous and strictly increasing function of $s_i$, with $u_i(0)=0$. This extends $u_i(s_i)$ from a linear function to any nonlinear function satisfying these requirements. The added nonlinearity provides us with a good way to optimize the transient frequency performance while remaining optimal for the steady-state economic dispatch. 
% control problem \eqref{eq:opt-ts}.

\begin{ass}[Continuity and monotonicity of $\boldsymbol{u}$]\label{ass:nonlinear-u}
$\forall i\in\mathcal{N}$, the function $u_i(\cdot):\real\mapsto \real$ is Lipschitz continuous and strictly increasing with $u_i(0)=0$.
\end{ass}
In Section~\ref{sec:RL}, we will show how this assumption can be imposed on controllers parameterized by neural networks. Namely, we can explicitly design the weights and biases of a neural network such that the required structure on the controller is explicitly satisfied. 

Next, we also relax the restriction to quadratic cost functions by allowing DAI to handle cost functions that satisfy the following assumption.

\begin{ass}[Scaled cost gradient functions]\label{ass-cost-grad-scale} There exists a strictly convex and continuously differentiable function $C_\mathrm{o}(\cdot):\real\mapsto \real$ and positive scaling factors $\boldsymbol{\zeta}:=\left(\zeta_i, i \in \mathcal{N} \right) \in \real^n_{+}$ such that
\begin{align} \label{eqn:cost_condition}
\nabla C_i(u_i)=\nabla C_\mathrm{o}(\zeta_i u_i)\,,\qquad \forall i\in\mathcal{N}\,.\end{align}
\end{ass}

Assumption~\ref{ass-cost-grad-scale} admits any strictly convex cost functions whose gradients are identical up to heterogeneous scaling factors. To look in greater detail at how this generalizes beyond quadratic cost functions, we provide some examples of common strictly convex functions that satisfy Assumption~\ref{ass-cost-grad-scale}. If the cost functions on individual buses are:
\begin{itemize}
%     \item (linear-quadratic functions with identical linear coefficients)
%     \begin{align}
%         C_i(u_i)= \dfrac{1}{2}c_i u_i^2 + b u_i + a_i\ \text{with}\ c_i>0\,,
%     \end{align}
%     then
%     \begin{align}
% \nabla C_i(u_i)=c_i u_i+b\,,\qquad\forall i\in\mathcal{N}\,. \end{align}
% Thus, we can choose
% \begin{align}
% C_\mathrm{o}(\cdot)= \dfrac{1}{2}(\cdot)^2+b(\cdot)\,,   
% \end{align}
% which satisfies 
% \begin{align}
% \nabla C_i(u_i)=c_i u_i+b=\nabla C_\mathrm{o}(c_i u_i)\,,\qquad\forall i\in\mathcal{N}\,. \end{align}
\item \emph{power functions with positive even integer powers:}
    \begin{align}\label{eq:cost-power}
        C_i(u_i)= \dfrac{c_i}{r} u_i^r+b_i\,,
    \end{align}
where $c_i>0$ and $r$ is a positive even integer, then
    \begin{align}\label{eq:cost-power-grad}
\nabla C_i(u_i)=c_i u_i^{r-1}\,,\qquad\forall i\in\mathcal{N}\,. \end{align}
Thus, we can choose
\begin{align} \label{eq:zeta}
C_\mathrm{o}(\cdot)= \dfrac{1}{r}(\cdot)^r\qquad\ \text{and}\qquad\zeta_i=c_i^{\frac{1}{r-1}}\,,   
\end{align}
which satisfies the condition in~\eqref{eqn:cost_condition}.
% $\forall i\in\mathcal{N}$, 
% \begin{align*}
% \nabla C_i(u_i)\!=\!c_i u_i^{r-1}\!=\!\!\left(\!c_i^{\frac{1}{r-1}} u_i\!\right)^{r-1}\!\!\!=\!\left(\zeta_i u_i\right)^{r-1}\!=\!\nabla C_\mathrm{o}(\zeta_i u_i)\,. \end{align*}
\item \emph{arbitrary strictly convex and continuously differentiable functions that are identical up to constant terms:}
    \begin{align*}
        C_i(u_i)= C_\mathrm{o}(u_i)+b_i\,,
    \end{align*}
and its straightforward to check \eqref{eqn:cost_condition} is satisfied. 
% \begin{align*}
% \nabla C_i(u_i)=\nabla C_\mathrm{o}(u_i)=\nabla C_\mathrm{o}(\zeta_i u_i)\ \text{with}\ \zeta_i=1\,,\ \forall i\in\mathcal{N}\,. \end{align*}
\end{itemize}
Clearly, the quadratic cost functions in \eqref{eq:cost-quad} belong to the first scenario since \eqref{eq:cost-power} reduces exactly to \eqref{eq:cost-quad} if $r=2$ and $b_i=0$, which validates our generalization through Assumption~\ref{ass-cost-grad-scale}. 

Now, under Assumptions~\ref{ass:nonlinear-u} and~\ref{ass-cost-grad-scale}, we are ready to propose the \emph{generalized DAI} as follows: 
\begin{align}\label{eq:DAI-s-general}
    \dot {s}_{i} \!=\!-2 \pi f_0\omega_i \!-\!\zeta_i\!\! \sum_{j=1}^n\! Q_{ij}\!\left(\nabla C_i(u_i(s_i))\!-\!\nabla C_j(u_j(s_i))\right)\!\!\,.
\end{align}
Although not obvious at first sight, the generalized DAI in \eqref{eq:DAI-s-general} preserves the ability of the classic DAI to restore the nominal frequency and solves the optimal steady-state economic dispatch problem \eqref{eq:opt-ss} for cost functions satisfying Assumption~\ref{ass-cost-grad-scale}. In addition, the more general nonlinear form of $\boldsymbol{u}$ introduced in Assumption~\ref{ass:nonlinear-u} provides us with more degrees of freedom to better deal with the optimal transient frequency control problem \eqref{eq:opt-ts}. All of these statements would become clear as the analysis unfolds.

After combining \eqref{eq:sys-dyn-vec} and \eqref{eq:DAI-s-general}, we can write the overall closed-loop system dynamics under our proposed generalized DAI compactly as  
% \begin{subequations}\label{eq:sys-dyn-distribute}
% \begin{align*} 
%     \dot{\theta}_i =&\ 2 \pi f_0 \omega_i\,,\\
%     m_i \dot{\omega}_i =& -
%     \alpha_i \omega_i- \sum_{j=1}^n v_iv_jB_{ij}\sin{\left(\theta_i-\theta_j\right)} + p_{i} + u_{i}(s_i)\,,\\
%     \dot {s}_{i} =&\ -2 \pi f_0\omega_i -c_i \sum_{j=1}^n Q_{ij}\left(c_i u_i-c_j u_j\right)\,, \label{eq:bus-dyn}
% \end{align*}
% \end{subequations}
\begin{subequations}\label{eq:sys-dyn-vec-distribute}
\begin{align}
    \dot{\boldsymbol{\delta}} =&\ 2 \pi f_0\left(I_n-\frac{1}{n}\mathbbold{1}_n\mathbbold{1}_n^T\right) \boldsymbol{\omega}\,,\label{eq:sys-dyn-vec-distribute-delta}\\
    \boldsymbol{M} \dot{\boldsymbol{\omega}}_\mathcal{G} =& -
    \boldsymbol{A}_\mathcal{G} \boldsymbol{\omega}_\mathcal{G}- \nabla_\mathcal{G} U (\boldsymbol{\delta}) + \boldsymbol{p}_\mathcal{G} + \boldsymbol{u}_\mathcal{G}(\boldsymbol{s})\,,\\
    \mathbbold{0}_{|\mathcal{L}|} =& -
    \boldsymbol{A}_\mathcal{L} \boldsymbol{\omega}_\mathcal{L}- \nabla_\mathcal{L} U (\boldsymbol{\delta}) + \boldsymbol{p}_\mathcal{L} + \boldsymbol{u}_\mathcal{L}(\boldsymbol{s})\,,\label{eq:sys-dyn-vec-distribute-omegaL}\\
     \dot {\boldsymbol{s}} =& -2 \pi f_0 \boldsymbol{\omega} - \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))\,,\label{eq:bus-dyn}
     \end{align}
\end{subequations}
where $\boldsymbol{s}:=\left(s_i, i \in \mathcal{N} \right) \in \real^n$, $\boldsymbol{Z} := \diag{\zeta_i, i \in \mathcal{N}} \in \real^{n \times n}$, $\boldsymbol{L}_\mathrm{Q}:=\left[ L_{\mathrm{Q},ij}\right]\in \real^{n \times n}$ is the Laplacian matrix associated with the communication graph whose $ij$th element is
\begin{align*}
    \forall i,j \in \mathcal{N},\qquad L_{\mathrm{Q},ij}:=
    \begin{dcases}
    -Q_{ij} & \text{if}\ i\neq j\\
    \sum_{j^\prime=1,j^\prime\neq i}^n Q_{ij^\prime}& \text{if}\ i=j
    \end{dcases}\ \;,
\end{align*} 
and $\boldsymbol{u}(\boldsymbol{s}) := \left(u_{i}(s_i),i \in \mathcal{N} \right) \in \real^n$ with each $u_i(s_i)$ satisfying Assumption~\ref{ass:nonlinear-u}.

We conclude this subsection by stating a useful property of the inverse functions of the cost gradient functions on individual buses, which is a consequence of Assumption~\ref{ass-cost-grad-scale}. We make use of it later in 
the stability analysis of the closed-loop system~\eqref{eq:sys-dyn-vec-distribute}.

\begin{lem}[Identical scaled controllable power injections]\label{lem:inverse-id} If Assumption~\ref{ass-cost-grad-scale} holds, then  
\begin{align}\label{eq:inverse-id}
\zeta_i \nabla C_i^{-1}(\cdot)=\nabla C_\mathrm{o}^{-1}(\cdot)\,,\qquad \forall i\in\mathcal{N}\,,\end{align}
where $\nabla C_i^{-1}(\cdot)$ and $\nabla C_\mathrm{o}^{-1}(\cdot)$ denote the inverse functions of $\nabla C_i(\cdot)$ and $\nabla C_\mathrm{o}(\cdot)$, respectively.
\end{lem}
\begin{proof}
See the Appendix \ref{app:lem1-pf}.
\end{proof}

Provided that the cost functions on individual buses satisfy Assumption~\ref{ass-cost-grad-scale}, Lemma~\ref{lem:inverse-id} indicates that, for any given marginal price, each generator or load contributes the same amount of controllable power injection up to a scaling factor. 

\begin{rem}[Existence and monotonicity of $\nabla C_i^{-1}(\cdot)$ and $\nabla C_\mathrm{o}^{-1}(\cdot)$]\label{rem:inverse} Note that the existence of $\nabla C_i^{-1}(\cdot)$ is guaranteed by the strict convexity of $C_i(\cdot)$, which implies that $\nabla C_i(\cdot)$ is a strictly increasing function~\cite{rockafellar1998}. By a standard result in analysis, any strictly increasing function has an inverse that is also strictly increasing~\cite{binmore1977mathanalysis}. 
% precisely, by~\cite[Theorem~2.14]{rockafellar1998}, the strict convexity of $C_i(\cdot)$ implies that $\nabla C_i(\cdot)$ is a strictly increasing function. According to~\cite[Chapter~12.9]{binmore1977mathanalysis}, this further implies that $\nabla C_i(\cdot)$ has an inverse function $\nabla C_i^{-1}(\cdot)$ which is also strictly increasing. The same argument holds for $\nabla C_\mathrm{o}^{-1}(\cdot)$.
\end{rem}

\subsection{Closed-Loop Equilibrium Analysis}
The first result we show is that the steady-state performance objectives are still achieved under the generalized DAI. This is captured by the following theorem. 

\begin{thm}[Closed-loop equilibrium]\label{thm:equilibrium}
Suppose Assumptions~\ref{ass:nonlinear-u} and~\ref{ass-cost-grad-scale} hold. Assume $\forall \{i,j\} \in\mathcal{E}$, $|\delta_i^\ast-\delta_j^\ast|\in [0,\pi/2)$.\footnote{This is the counterpart of the model assumption, $\forall \{i,j\} \in\mathcal{E}$, $|\theta_i^\ast-\theta_j^\ast|\in [0,\pi/2)$ in Remark~\ref{rem:model}.} Then the equilibrium $(\boldsymbol{\delta}^\ast, \boldsymbol{\omega}^\ast, \boldsymbol{s}^\ast)$ of the closed-loop system \eqref{eq:sys-dyn-vec-distribute} is a unique point satisfying
\begin{subequations}\label{eq:equ-DAI} 
\begin{align}
\boldsymbol{\omega}^\ast=&\ \mathbbold{0}_n\,,\\ \nabla U (\boldsymbol{\delta}^\ast) =&\ \boldsymbol{p} + \boldsymbol{u}(\boldsymbol{s}^\ast)\,,\label{eq:equ-DAI-delta}\\ \boldsymbol{u}(\boldsymbol{s}^\ast) =&\ \nabla C_\mathrm{o}^{-1}(\gamma)\boldsymbol{Z}^{-1}\mathbbold{1}_n\,, \label{eq:equ-DAI-u}   \end{align}
\end{subequations}
with $\gamma$ uniquely determined by
\begin{align}\label{eq:gamma}
\nabla C_\mathrm{o}^{-1}(\gamma)=-\dfrac{\sum_{i=1}^n p_i}{\sum_{i=1}^n \zeta_i^{-1}}\,.    
\end{align}
% \begin{align}\label{eq:gamma}
% \sum_{i=1}^n\nabla C_i^{-1}(\gamma)=-\sum_{i=1}^n p_i\,.    
% \end{align}
\end{thm}
\begin{proof}
The equilibrium analysis is similar to the one presented in Section~\ref{ssec:goal}, except that the effect of the integral variables $\boldsymbol{s}$ introduced by the generalized DAI should be considered. Hence, in steady-state, \eqref{eq:sys-dyn-vec-distribute} yields
\begin{subequations}
\begin{align}\label{eq:equli-dai}
 \mathbbold{0}_n =& -
    \boldsymbol{A} \mathbbold{1}_n\omega^\ast- \nabla U (\boldsymbol{\delta}^\ast) + \boldsymbol{p} + \boldsymbol{u}(\boldsymbol{s}^\ast)\,,\\
    2 \pi f_0 \mathbbold{1}_n\omega^\ast =& -\boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}^\ast))\,,\label{eq:equli-dai-s}
    \end{align}
\end{subequations}
where we have used the equilibria characterizations $\boldsymbol{\omega}^\ast=\mathbbold{1}_n\omega^\ast$ and \eqref{eq:equli-sync-omega}.

We then proceed to investigate the equilibrium by following a similar argument as in~\cite[Lemma~4.2]{Johannes2016ecc}. Premultiplying \eqref{eq:equli-dai-s} by $\mathbbold{1}_n^T\boldsymbol{Z}^{-1}$ yields 
\begin{align}
2 \pi f_0 \mathbbold{1}_n^T\boldsymbol{Z}^{-1}\mathbbold{1}_n\omega^\ast =& - \mathbbold{1}_n^T\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}^\ast)) = 0\,, \label{eq:omegastar-eq}
\end{align}
where the second equality is due to the property of the Laplacian matrix~\cite{FB-LNS} that $\mathbbold{1}_n^T\boldsymbol{L}_\mathrm{Q}=\mathbbold{0}_n^T$. Note that $\mathbbold{1}_n^T\boldsymbol{Z}^{-1}\mathbbold{1}_n>0$ since $\boldsymbol{Z}^{-1}\succ 0$ by construction. Thus, \eqref{eq:omegastar-eq} implies that $\omega^\ast=0$. Then, \eqref{eq:equli-dai-s} becomes $\boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}^\ast))=\mathbbold{0}_n$, which indicates that $\nabla C(\boldsymbol{u}(\boldsymbol{s}^\ast))\in\range{\mathbbold{1}_n}$, i.e., $\nabla C(\boldsymbol{u}(\boldsymbol{s}^\ast)) = \gamma\mathbbold{1}_n$ for some constant $\gamma$. Thus, $\boldsymbol{u}(\boldsymbol{s}^\ast)=\left(\nabla C_i^{-1}(\gamma),i \in \mathcal{N} \right)$. Note that $\boldsymbol{Z}\boldsymbol{u}(\boldsymbol{s}^\ast)= \left(\zeta_i\nabla C_i^{-1}(\gamma),i \in \mathcal{N} \right)=\nabla C_\mathrm{o}^{-1}(\gamma)\mathbbold{1}_n$ by Lemma~\ref{lem:inverse-id}, which further implies that $\boldsymbol{u}(\boldsymbol{s}^\ast)=\nabla C_\mathrm{o}^{-1}(\gamma)\boldsymbol{Z}^{-1}\mathbbold{1}_n$.

Now, applying $\omega^\ast=0$ and $\boldsymbol{u}(\boldsymbol{s}^\ast) = \nabla C_\mathrm{o}^{-1}(\gamma)\boldsymbol{Z}^{-1}\mathbbold{1}_n$ to \eqref{eq:equli-dai} yields
\begin{align}\label{eq:equli-dai-gamma}
 \nabla U (\boldsymbol{\delta}^\ast) = \boldsymbol{p} + \nabla C_\mathrm{o}^{-1}(\gamma)\boldsymbol{Z}^{-1}\mathbbold{1}_n\,.
    \end{align}
Then, premultiplying \eqref{eq:equli-dai-gamma} by $\mathbbold{1}_n^T$ yields the equation that determines $\gamma$ as shown in \eqref{eq:gamma},
where $\mathbbold{1}_n^T\nabla U (\boldsymbol{\delta})=0$ is used again. We can show that the solution $\gamma$ to \eqref{eq:gamma} is unique by way of contradiction. Suppose that both $\gamma$ and $\tilde{\gamma}$ satisfy \eqref{eq:gamma}, where $\gamma\neq\tilde{\gamma}$. Then,
\begin{align}\label{eq:gamma-diff}
\nabla C_\mathrm{o}^{-1}(\gamma)-\nabla C_\mathrm{o}^{-1}(\tilde{\gamma})=&\left(-\dfrac{\sum_{i=1}^n p_i}{\sum_{i=1}^n \zeta_i^{-1}}\right)-\left(-\dfrac{\sum_{i=1}^n p_i}{\sum_{i=1}^n \zeta_i^{-1}}\right)\nonumber\\=&\ 0\,.  \end{align}
Multiplying \eqref{eq:gamma-diff} by $\left(\gamma-\tilde{\gamma}\right)$ yields
\begin{align}\label{eq:gamma-diff-prod}
0=& \left(\gamma-\tilde{\gamma}\right)\left(\nabla C_\mathrm{o}^{-1}(\gamma)-\nabla C_\mathrm{o}^{-1}(\tilde{\gamma})\right)>0\,,
\end{align}
where the inequality is due to the fact that $\nabla C_\mathrm{o}^{-1}(\cdot)$ is strictly increasing as discussed in Remark~\ref{rem:inverse}. Clearly, \eqref{eq:gamma-diff-prod} is a contradiction. Thus, $\gamma$ is unique.
% \begin{align}\label{eq:gamma-diff}
% \!\!\!\!\sum_{i=1}^n\! \nabla C_i^{-1}(\gamma)\!-\!\!\sum_{i=1}^n\! \nabla C_i^{-1}(\tilde{\gamma})\!=\!\!\left(\!\!-\!\!\sum_{i=1}^n p_i\!\!\right)\!\!-\!\!\left(\!\!-\!\!\sum_{i=1}^n p_i\!\!\right)\!\!=\!0\,.  \end{align}
% Multiplying \eqref{eq:gamma-diff} by $\left(\gamma-\tilde{\gamma}\right)$ yields
% \begin{align}\label{eq:gamma-diff-prod}
% 0=& \left(\gamma-\tilde{\gamma}\right)\left(\sum_{i=1}^n \nabla C_i^{-1}(\gamma)-\sum_{i=1}^n \nabla C_i^{-1}(\tilde{\gamma})\right)\nonumber \\
% =&\left(\gamma-\tilde{\gamma}\right)\sum_{i=1}^n\left( \nabla C_i^{-1}(\gamma)- \nabla C_i^{-1}(\tilde{\gamma})\right)\nonumber\\=&\sum_{i=1}^n\left(\gamma-\tilde{\gamma}\right)\left( \nabla C_i^{-1}(\gamma)- \nabla C_i^{-1}(\tilde{\gamma})\right)>0\,,
% \end{align}
% where the inequality is due to the fact that $\nabla C_i^{-1}(\cdot)$ is strictly increasing. Clearly, \eqref{eq:gamma-diff-prod} is a contradiction. Thus, $\gamma$ is unique.

% where $\nabla C_i^{-1}(\cdot)$ denotes the inverse function of $\nabla C_i(\cdot)$. Note that the existence of $\nabla C_i^{-1}(\cdot)$ is guaranteed by the strict convexity of $C_i(\cdot)$. More precisely, by~\cite[Theorem~2.14]{rockafellar1998}, the strict convexity of $C_i(\cdot)$ implies that $\nabla C_i(\cdot)$ is a strictly increasing function. According to~\cite[Chapter~12.9]{binmore1977mathanalysis}, this further implies that $\nabla C_i(\cdot)$ has an inverse function $\nabla C_i^{-1}(\cdot)$ which is also strictly increasing.

% Now, applying $\omega^\ast=0$ and $\boldsymbol{u}(\boldsymbol{s}^\ast) = \left(\nabla C_i^{-1}(\gamma),i \in \mathcal{N} \right)$ to \eqref{eq:equli-dai} yields
% \begin{align}\label{eq:equli-dai-gamma}
%  \nabla U (\boldsymbol{\delta}^\ast) = \boldsymbol{p} + \left(\nabla C_i^{-1}(\gamma),i \in \mathcal{N} \right)\,.
%     \end{align}
% Then, premultiplying \eqref{eq:equli-dai-gamma} by $\mathbbold{1}_n^T$ yields the equation that determines $\gamma$ as shown in \eqref{eq:gamma},
% where $\mathbbold{1}_n^T\nabla U (\boldsymbol{\delta})=0$ is used again. We can show the solution $\gamma$ to \eqref{eq:gamma} is unique by way of contradiction. Suppose that both $\gamma$ and $\tilde{\gamma}$ satisfy \eqref{eq:gamma}, where $\gamma\neq\tilde{\gamma}$. Then,
% \begin{align}\label{eq:gamma-diff}
% \!\!\!\!\sum_{i=1}^n\! \nabla C_i^{-1}(\gamma)\!-\!\!\sum_{i=1}^n\! \nabla C_i^{-1}(\tilde{\gamma})\!=\!\!\left(\!\!-\!\!\sum_{i=1}^n p_i\!\!\right)\!\!-\!\!\left(\!\!-\!\!\sum_{i=1}^n p_i\!\!\right)\!\!=\!0\,.  \end{align}
% Multiplying \eqref{eq:gamma-diff} by $\left(\gamma-\tilde{\gamma}\right)$ yields
% \begin{align}\label{eq:gamma-diff-prod}
% 0=& \left(\gamma-\tilde{\gamma}\right)\left(\sum_{i=1}^n \nabla C_i^{-1}(\gamma)-\sum_{i=1}^n \nabla C_i^{-1}(\tilde{\gamma})\right)\nonumber \\
% =&\left(\gamma-\tilde{\gamma}\right)\sum_{i=1}^n\left( \nabla C_i^{-1}(\gamma)- \nabla C_i^{-1}(\tilde{\gamma})\right)\nonumber\\=&\sum_{i=1}^n\left(\gamma-\tilde{\gamma}\right)\left( \nabla C_i^{-1}(\gamma)- \nabla C_i^{-1}(\tilde{\gamma})\right)>0\,,
% \end{align}
% where the inequality is due to the fact that $\nabla C_i^{-1}(\cdot)$ is strictly increasing. Clearly, \eqref{eq:gamma-diff-prod} is a contradiction. Thus, $\gamma$ is unique.

It remains to show that the equilibrium point is unique. We focus on the uniqueness of $\boldsymbol{s}^\ast$. By way of contradiction, suppose that both $\boldsymbol{s}^\ast$ and $\boldsymbol{s}^\star$ satisfy \eqref{eq:equ-DAI-u}, where $\boldsymbol{s}^\ast\neq\boldsymbol{s}^\star$. Then,
\begin{align}\label{eq:u-diff}
\boldsymbol{u}(\boldsymbol{s}^\ast) - \boldsymbol{u}(\boldsymbol{s}^\star)=& \nabla C_\mathrm{o}^{-1}(\gamma)\boldsymbol{Z}^{-1}\mathbbold{1}_n-\nabla C_\mathrm{o}^{-1}(\gamma)\boldsymbol{Z}^{-1}\mathbbold{1}_n\nonumber\\=&\ \mathbbold{0}_n \,. 
\end{align}
% \begin{align}\label{eq:u-diff}
% \boldsymbol{u}(\boldsymbol{s}^\ast) - \boldsymbol{u}(\boldsymbol{s}^\star)=& \left(\nabla C_i^{-1}(\gamma),i \in \mathcal{N} \right)-\left(\nabla C_i^{-1}(\gamma),i \in \mathcal{N} \right)\nonumber\\=&\ \mathbbold{0}_n \,. 
% \end{align}
Premultiplying \eqref{eq:u-diff} by $\left(\boldsymbol{s}^\ast-\boldsymbol{s}^\star\right)^T$ yields
\begin{align}\label{eq:u-diff-prod}
0=&\left(\boldsymbol{s}^\ast-\boldsymbol{s}^\star\right)^T\left(\boldsymbol{u}(\boldsymbol{s}^\ast) - \boldsymbol{u}(\boldsymbol{s}^\star)\right)\nonumber\\=&\sum_{i=1}^n \left(s_i^\ast-s_i^\star\right)\left(u_i(s_i^\ast)-u_i(s_i^\star)\right)>0 \,,  
\end{align}
where the inequality results from our requirement that $u_i(s_i)$ is strictly increasing with respect to $s_i$. Clearly, \eqref{eq:u-diff-prod} is a contradiction. Thus, $\boldsymbol{s}^\ast$ is unique. By~\cite[Lemma~1]{weitenberg2017exponentialarxiv}, the solution $\boldsymbol{\delta}^\ast$ to \eqref{eq:equli-dai-gamma} is unique. This concludes the proof of the uniqueness of the equilibrium.
\end{proof}

Theorem~\ref{thm:equilibrium} verifies that the generalized DAI preserves the steady-state performance of the normal DAI. It forces the closed-loop system \eqref{eq:sys-dyn-vec-distribute} to settle down at a unique equilibrium point where the frequency is nominal, i.e., $\boldsymbol{\omega}^\ast=\mathbbold{0}_n$, and the controllable power injections $\boldsymbol{u}^\ast$ meet the identical marginal cost requirement \eqref{eq:id-marginal} since, $\forall i\in\mathcal{N}$, 
\begin{align*}
\nabla C_i (u_i^\ast) =&\nabla C_i (u_i(s_i^\ast))\stackrel{\text{\eqref{eq:equ-DAI-u}}}{=}\nabla C_i (\nabla C_\mathrm{o}^{-1}(\gamma)\zeta_i^{-1})\\\stackrel{\text{\eqref{eq:inverse-id}}}{=}&\nabla C_i (\zeta_i\nabla C_i^{-1}(\gamma)\zeta_i^{-1})=\nabla C_i (\nabla C_i^{-1}(\gamma)) =\gamma \,.   
\end{align*}
Thus, the objectives of nominal steady-state frequency and optimal steady-state economic dispatch for a broader range of cost functions are both achieved. 

\subsection{Lyapunov Stability Analysis}
Having characterized the equilibrium point and confirmed the steady-state performance of the closed-loop system \eqref{eq:sys-dyn-vec-distribute} under the generalized DAI, we are now ready to investigate the system stability by performing Lyapunov stability analysis. More precisely, the stability under the generalized DAI can be certified by finding a well-defined ``weak'' Lyapunov function
%
%\marginJC{Should we refer to it as "weak Lyapunov" since evolution is only nonincreasing (where "strong Lyapunov" will be for strictly decreasing)}
%
that is nonincreasing along the trajectories of the closed-loop system~\eqref{eq:sys-dyn-vec-distribute}. The main result of this whole subsection is presented below, whose proof is enabled by a sequence of smaller results that we discuss next.

\begin{thm}[Asymptotic stability]\label{thm:as-stable}
Under Assumptions~\ref{ass:nonlinear-u} and~\ref{ass-cost-grad-scale}, any trajectory of \eqref{eq:sys-dyn-vec-distribute} that starts from the neighborhood $\Set*{(\boldsymbol{\delta}, \boldsymbol{\omega}, \boldsymbol{s})\!\in \!\real^n \!\!\times\! \real^{n}\!\!\times\! \real^n}{|\delta_i-\delta_j|\in [0,\pi/2), \forall \{i,j\}\!\in \!\mathcal{E}}$
of the equilibrium characterized by \eqref{eq:equ-DAI} with $|\delta_i^\ast-\delta_j^\ast|\in [0,\pi/2)$, $\forall \{i,j\} \in\mathcal{E}$, converges asymptotically to the equilibrium.
\end{thm}

%
%\marginJC{Starting from here, we have a whole sequence of steps that eventually lead to the conclusion in Theorem 2. How about having the theorem statement first, right here, and then saying that the proof of it is enabled by a sequence of smaller results that we discuss next. The subsection could conclude with the proof of the theorem 2. This has the advantage that the reader gets the most important result first, and can safely skip stuff on a first read if he/she's more interested in what comes later.}
%

%
%\marginJC{I think I'd say this differently. I'd start by saying  that (18c) fully determines $\boldsymbol{\omega}_\mathcal{L}$ as a function of $\boldsymbol{\delta}$ and $\boldsymbol{s}$ (and write here the explicit formula). This means that we only need to consider the evolution of $(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})$.}
%

First note that the algebraic equation \eqref{eq:sys-dyn-vec-distribute-omegaL} fully determines $\boldsymbol{\omega}_\mathcal{L}$ as a function of $\boldsymbol{\delta}$ and $\boldsymbol{s}$, i.e.,
$$ \boldsymbol{\omega}_\mathcal{L} = \boldsymbol{A}_\mathcal{L}^{-1}\left(- \nabla_\mathcal{L} U (\boldsymbol{\delta}) + \boldsymbol{p}_\mathcal{L} + \boldsymbol{u}_\mathcal{L}(\boldsymbol{s})\right)\,,$$
which means that we only need to explicitly consider the evolution of $(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})$. Thus,
in what follows, we only focus on the state component $(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})$ for a neighborhood $\mathcal{D}:=\! \Set*{(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})\!\in \!\real^n \!\!\times\! \real^{|\mathcal{G}|}\!\!\times\! \real^n}{|\delta_i-\delta_j|\in [0,\pi/2), \forall \{i,j\}\!\in \!\mathcal{E}}$ of the equilibrium $(\boldsymbol{\delta}^\ast, \mathbbold{0}_{|\mathcal{G}|}, \boldsymbol{s}^\ast)$.
%We do not 
%explicitly consider $\boldsymbol{\omega}_\mathcal{L}$ because
%it is determined by $\boldsymbol{\delta}$ and $\boldsymbol{s}$ through the algebraic equation \eqref{eq:sys-dyn-vec-distribute-omegaL}. 
The following result formalizes this thought by showing that the distance from the whole state $(\boldsymbol{\delta}, \boldsymbol{\omega}, \boldsymbol{s})$ to $(\boldsymbol{\delta}^\ast, \mathbbold{0}_n, \boldsymbol{s}^\ast)$ is lower and upper bounded by the distance from the partial state $(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})$ to $(\boldsymbol{\delta}^\ast, \mathbbold{0}_{|\mathcal{G}|}, \boldsymbol{s}^\ast)$.

\begin{lem}[Bounds on whole state distance]\label{lem:bound-state}Let $\|\cdot\|_2$ denote the Euclidean norm. Under Assumptions~\ref{ass:nonlinear-u} and~\ref{ass-cost-grad-scale}, there exists some constant $\nu>0$ such that, $\forall(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G},\boldsymbol{s})\in \mathcal{D}$,
 %Define $\|(\boldsymbol{\delta}-\boldsymbol{\delta}^\ast, \boldsymbol{\omega}, \boldsymbol{s}-\boldsymbol{s}^\ast)\|^2:=\|\boldsymbol{\delta}-\boldsymbol{\delta}^\ast\|_2^2+\|\boldsymbol{\omega}\|_2^2+\|\boldsymbol{s}-\boldsymbol{s}^\ast\|_2^2$ and $\|(\boldsymbol{\delta}-\boldsymbol{\delta}^\ast, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s}-\boldsymbol{s}^\ast)\|^2:=\|\boldsymbol{\delta}-\boldsymbol{\delta}^\ast\|_2^2+\|\boldsymbol{\omega}_\mathcal{G}\|_2^2+\|\boldsymbol{s}-\boldsymbol{s}^\ast\|_2^2$, where $\|\cdot\|_2^2$ denotes the squared Euclidean norm. Then
% \begin{align*}
% \|(\boldsymbol{\delta}-\boldsymbol{\delta}^\ast, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s}-\boldsymbol{s}^\ast)\|^2\leq& \|(\boldsymbol{\delta}-\boldsymbol{\delta}^\ast, \boldsymbol{\omega}, \boldsymbol{s}-\boldsymbol{s}^\ast)\|^2\\\leq& \nu\|(\boldsymbol{\delta}-\boldsymbol{\delta}^\ast, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s}-\boldsymbol{s}^\ast)\|^2    
% \end{align*}
\begin{align*}
&\ \|\boldsymbol{\delta}-\boldsymbol{\delta}^\ast\|_2^2+\|\boldsymbol{\omega}_\mathcal{G}\|_2^2+\|\boldsymbol{s}-\boldsymbol{s}^\ast\|_2^2\\\leq&\ \|\boldsymbol{\delta}-\boldsymbol{\delta}^\ast\|_2^2+\|\boldsymbol{\omega}\|_2^2+\|\boldsymbol{s}-\boldsymbol{s}^\ast\|_2^2\\\leq&\ \nu\left(\|\boldsymbol{\delta}-\boldsymbol{\delta}^\ast\|_2^2+\|\boldsymbol{\omega}_\mathcal{G}\|_2^2+\|\boldsymbol{s}-\boldsymbol{s}^\ast\|_2^2\right)\,,   
\end{align*}
where $(\boldsymbol{\delta}^\ast, \mathbbold{0}_n, \boldsymbol{s}^\ast)$ is the equilibrium of the closed-loop system \eqref{eq:sys-dyn-vec-distribute} characterized by \eqref{eq:equ-DAI} with $|\delta_i^\ast-\delta_j^\ast|\in [0,\pi/2)$, $\forall \{i,j\} \in\mathcal{E}$.
\end{lem}
\begin{proof} 
See Appendix \ref{app:lem2-pf}.
\end{proof}

Lemma~\ref{lem:bound-state} indicates that it suffices to investigate the evolution of $(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})$.
%since the whole state $(\boldsymbol{\delta}, \boldsymbol{\omega}, \boldsymbol{s})$ can blow up only if the partial state $(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})$ does so. 
To do so, we need to first find a well-defined Lyapunov function $W(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})$ such that $W(\boldsymbol{\delta}^\ast, \mathbbold{0}_{|\mathcal{G}|}, \boldsymbol{s}^\ast)=0$ and $W(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G},\boldsymbol{s})>0$, $\forall(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G},\boldsymbol{s})\in \mathcal{D}\setminus{(\boldsymbol{\delta}^\ast, \mathbbold{0}_{|\mathcal{G}|}, \boldsymbol{s}^\ast)}$, and then verify $\dot{W}(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})\leq0$, $\forall(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G},\boldsymbol{s})\in \mathcal{D}$.

Following the same method in \cite{DORFLER2017Auto}, we begin our construction of a Lyapunov function by defining the following integral function:
\begin{align}\label{eq:L(s)}
L(\boldsymbol{s}):=\sum_{i=1}^n \int_0^{s_i}u_i(\xi)\ \mathrm{d}\xi\,,    
\end{align}
which clearly satisfies $\nabla L (\boldsymbol{s})=\boldsymbol{u}(\boldsymbol{s})$. Another useful property related to $L(\boldsymbol{s})$ is given in the next lemma. 
% that it is strictly convex since $u_i(s_i)$ is strictly increasing with respect to $s_i$, $\forall i\in\mathcal{N}$.
\begin{lem}[Strict convexity of $L(\boldsymbol{s})$]\label{lem:strict-conv-L}
If Assumption~\ref{ass:nonlinear-u} holds, then the function $L(\boldsymbol{s})$ defined in \eqref{eq:L(s)} is strictly convex.
\end{lem}
\begin{proof} 
See the Appendix \ref{app:lem3-pf}.
\end{proof}

Having characterized the properties of $L(\boldsymbol{s})$, we consider the following Lyapunov function candidate:
\begin{align}\label{eq: Lyapunov}
W(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s}):=&\ \pi f_0 \boldsymbol{\omega}_\mathcal{G}^T\boldsymbol{M}\boldsymbol{\omega}_\mathcal{G} \\&+ U(\boldsymbol{\delta})-U(\boldsymbol{\delta^\ast})-\nabla U (\boldsymbol{\delta^\ast})^T\left(\boldsymbol{\delta}-\boldsymbol{\delta^\ast}\right)\nonumber\\&+ L(\boldsymbol{s})-L(\boldsymbol{s^\ast})-\nabla L (\boldsymbol{s^\ast})^T\left(\boldsymbol{s}-\boldsymbol{s^\ast}\right)\,,\nonumber    \end{align}
where $(\boldsymbol{\delta}^\ast, \mathbbold{0}_{|\mathcal{G}|}, \boldsymbol{s}^\ast)$ corresponds to the unique equilibrium point of the closed-loop system \eqref{eq:sys-dyn-vec-distribute} satisfying \eqref{eq:equ-DAI}. The next result shows that this is  a well-defined candidate Lyapunov function on~$\mathcal{D}$.

\begin{lem}[Well-defined Lyapunov function]\label{lem:W}
Let Assumptions~\ref{ass:nonlinear-u} and~\ref{ass-cost-grad-scale} hold. The function $W(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})$ defined in \eqref{eq: Lyapunov} satisfies
$W(\boldsymbol{\delta}^\ast, \mathbbold{0}_{|\mathcal{G}|}, \boldsymbol{s}^\ast)=0$ and $W(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})>0, \forall(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})\in \mathcal{D}\setminus{(\boldsymbol{\delta}^\ast, \mathbbold{0}_{|\mathcal{G}|}, \boldsymbol{s}^\ast)}$.
\end{lem}
\begin{proof}
See the Appendix \ref{app:lem4-pf}.
\end{proof}

%Lemma~\ref{lem:W} verifies that the Lyapunov function $W(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})$ in~\eqref{eq: Lyapunov} is well-defined. 
Next, we examine the system stability through the derivative of $W(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})$ along the trajectories of the closed-loop system \eqref{eq:sys-dyn-vec-distribute}, whose expression is provided by the next result.

\begin{lem}[Directional derivative of Lyapunov function]\label{lem:Wdot}
Let Assumptions~\ref{ass:nonlinear-u} and~\ref{ass-cost-grad-scale} hold. Then the derivative of the Lyapunov function $W(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})$ defined in \eqref{eq: Lyapunov} along the trajectories of the closed-loop system \eqref{eq:sys-dyn-vec-distribute} is given by
\begin{align}\label{eq:Wdot-distribute}
    &\dot{W}(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s}) = \\
    &-2\pi f_0 \boldsymbol{\omega}_\mathcal{G}^T\boldsymbol{A}_\mathcal{G} \boldsymbol{\omega}_\mathcal{G}- \boldsymbol{u}(\boldsymbol{s})^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))\nonumber\\
    &-2\pi f_0 \left(\nabla_\mathcal{L} U (\boldsymbol{\delta}^\ast)-\nabla_\mathcal{L} U (\boldsymbol{\delta})+\boldsymbol{u}_\mathcal{L}(\boldsymbol{s})-\boldsymbol{u}_\mathcal{L}(\boldsymbol{s}^\ast)\right)^T\boldsymbol{A}_\mathcal{L}^{-1}\nonumber\\&\quad\cdot\left(\nabla_\mathcal{L} U (\boldsymbol{\delta}^\ast)- \nabla_\mathcal{L} U (\boldsymbol{\delta})  + \boldsymbol{u}_\mathcal{L}(\boldsymbol{s})\!-\boldsymbol{u}_\mathcal{L}(\boldsymbol{s}^\ast)\right)\,.\nonumber
\end{align}
\end{lem}
\begin{proof}
See the Appendix \ref{app:lem5-pf}.
\end{proof}

Our next step is to show that $\dot{W}(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})$ is nonpositive. From \eqref{eq:Wdot-distribute}, we observe that the quadratic terms defined by $\boldsymbol{A}_\mathcal{G}$ and  $\boldsymbol{A}_\mathcal{L}^{-1}$ are clearly negative. Thus, it only remains to determine the sign of the the cross-term $\boldsymbol{u}(\boldsymbol{s})^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))$ defined by the scaled Laplacian matrix $\boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}$. % Taking this into account, we have to make a detour to investigate this cross term at length. 
The first thing we notice is that this term as a bilinear form with respect to the scaled Laplacian matrix $\boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}$ can be expanded as the expression provided in the next result.
%
%\marginJC{Not sure what you want to say here: obviously the term is bilinear, by definition (it's like proving that the quadratic terms above are quadratic). Maybe you mean to say that the result shows the specific expression? }
%
%The following lemma characterizes such a property.

% \begin{lem}[Identical scaled controllable power injections]\label{lem:inverse-id} If Assumption~\ref{ass-cost-grad-scale} holds, then  
% \begin{align}\label{eq:inverse-id}
% \zeta_i \nabla C_i^{-1}(\cdot)=\nabla C_\mathrm{o}^{-1}(\cdot)\,,\qquad \forall i\in\mathcal{N}\,.\end{align}
% \end{lem}
% \begin{proof}
% $\forall y\in\real$, let $\tilde{u}_i=\nabla C_i^{-1}(y)$. Clearly, $y=\nabla C_i(\tilde{u}_i)$ by the definition of the inverse function. Also, under Assumption~\ref{ass-cost-grad-scale}, $\nabla C_i(\tilde{u}_i)=\nabla C_\mathrm{o}(\zeta_i \tilde{u}_i)$, $\forall i\in\mathcal{N}$. Thus, $y=\nabla C_i(\tilde{u}_i)=\nabla C_\mathrm{o}(\zeta_i \tilde{u}_i)$, which implies that $\zeta_i \tilde{u}_i=\nabla C_\mathrm{o}^{-1}(y)$. Therefore, we have $\zeta_i \nabla C_i^{-1}(y)=\zeta_i \tilde{u}_i=\nabla C_\mathrm{o}^{-1}(y)$, $\forall i\in\mathcal{N}$,
% which concludes the proof.
% \end{proof}

% Lemma~\ref{lem:inverse-id} indicates that, for any given marginal price, each generator or load contributes the same amount of controllable power injection up to a scaling factor, provided that the cost functions on individual buses satisfy Assumption~\ref{ass-cost-grad-scale}. This property can significantly simplifying our analysis on the cross term $\left(\boldsymbol{u}(\boldsymbol{s})-\boldsymbol{u}(\boldsymbol{s}^\ast)\right)^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))$ in \eqref{eq:Wdot-distribute}. The first thing we notice is the following corollary.

% \begin{cor}[$\boldsymbol{u}(\boldsymbol{s}^\ast)$ in the left null space of the scaled $\boldsymbol{L}_\mathrm{Q}$]\label{cor:ustar-null}
% Let Assumptions~\ref{ass:nonlinear-u} and~\ref{ass-cost-grad-scale} hold. Then
% % $\boldsymbol{u}(\boldsymbol{s}^\ast)^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}= \mathbbold{0}_n^T$.
% \begin{align*}
%     \boldsymbol{u}(\boldsymbol{s}^\ast)^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}= \mathbbold{0}_n^T\,.
% \end{align*}
% \end{cor}
% \begin{proof}
% An easy computation shows that
% \begin{align*}
%     \boldsymbol{u}(\boldsymbol{s}^\ast)^T \boldsymbol{Z}= \left(\zeta_i\nabla C_i^{-1}(\gamma),i \in \mathcal{N} \right)^T=\nabla C_\mathrm{o}^{-1}(\gamma)\mathbbold{1}_n^T\,,
% \end{align*}
% where the first equality uses \eqref{eq:equ-DAI-u} from Theorem~\ref{thm:equilibrium} and the second equality uses \eqref{eq:inverse-id} from Lemma~\ref{lem:inverse-id}. The result follows from the property of the Laplacian matrix that $\mathbbold{1}_n^T\boldsymbol{L}_\mathrm{Q}=\mathbbold{0}_n^T$~\cite{FB-LNS}.
% \end{proof}

% Clearly, by Corollary~\ref{cor:ustar-null}, $\left(\boldsymbol{u}(\boldsymbol{s})-\boldsymbol{u}(\boldsymbol{s}^\ast)\right)^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))$ directly reduces to $\boldsymbol{u}(\boldsymbol{s})^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))$, which can be considered as a bilinear form with respect to the scaled Laplacian matrix $\boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}$ addressed in the next lemma.

\begin{lem}[Bilinear form on $\real^n$ for scaled $\boldsymbol{L}_\mathrm{Q}$]\label{lem:bilinear-L}
$\forall\boldsymbol{x}:=\left(x_i, i \in \mathcal{N} \right) \in \real^n, \boldsymbol{y}:=\left(y_i, i \in \mathcal{N} \right)\in\real^n$,
\begin{align*}
\boldsymbol{x}^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q} \boldsymbol{y}=\sum_{\{i,j\} \in\mathcal{E}_\mathrm{Q}}\!\!\!Q_{ij}\left( y_i  - y_j \right)\left(\zeta_i x_i-\zeta_j x_j\right)\,.
\end{align*}
\end{lem}
\begin{proof}
See the Appendix \ref{app:lem6-pf}.
\end{proof}
%
%\marginJC{This lemma is a good candidate to have in the appendix (not just the proof, but the statement itself).}
%

With the help of Lemma~\ref{lem:bilinear-L}, the problem of determining the sign of the cross term $\boldsymbol{u}(\boldsymbol{s})^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))$ can be solved using the following corollary.

% \begin{cor}[Sign parity]\label{cor:sign}
% If Assumption~\ref{ass-cost-grad-scale} holds, then
% \begin{align*}
%   \sign{\left( \nabla C_i(u_i)\!-\!\nabla C_j(u_j)\right)}=\sign{\left(\zeta_iu_i-\zeta_j u_j\right)}\,,\ \forall i,j \in\mathcal{N}\,,
% \end{align*}
% where $\sign$ denotes the sign function.
% \end{cor}
% \begin{proof}
% See the Appendix \ref{app:cor1-pf}.
% \end{proof}
%
%\marginJC{I will only have Corollary 2 (so remove Corollary 1), and have the proof of the fact in Corollary 1 as the first part of the proof of Corollary 2. This is to not distract the reader with too many incremental results, and instead focus on more relevant (the sign of the bilinear term).}
%

%Corollary~\ref{cor:sign} allows us to determine the sign of the cross term $\boldsymbol{u}(\boldsymbol{s})^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))$.

\begin{cor}[Sign of cross term]\label{cor:sign-cross}
If Assumption~\ref{ass-cost-grad-scale} holds, then
\begin{align*}
    \boldsymbol{u}(\boldsymbol{s})^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))\geq0
\end{align*}
with equality holding if and only if when $\nabla C(\boldsymbol{u}(\boldsymbol{s}))\in\range{\mathbbold{1}_n}$.
\end{cor}
\begin{proof}
See the Appendix \ref{app:cor2-pf}.
\end{proof}

We now have all the elements necessary to establish the stability of the equilibrium as summarized in Theorem~\ref{thm:as-stable} by using $W$ as a Lyapunov function. Therefore, we are ready to finish the proof of Theorem~\ref{thm:as-stable}. Using the expression of $\dot{W}(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})$ in~\eqref{eq:Wdot-distribute},
it follows directly from the fact that $\boldsymbol{A}_\mathcal{G}\succ0$, $\boldsymbol{A}_\mathcal{L}^{-1}\succ0$, and $\boldsymbol{u}(\boldsymbol{s})^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))\geq0$ by Corollary~\ref{cor:sign-cross} that $\dot{W}(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})\leq0$. Observe from \eqref{eq:Wdot-distribute} that $\dot{W}(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})\equiv0$ directly enforces $\boldsymbol{\omega}_\mathcal{G}\equiv\mathbbold{0}_{|\mathcal{G}|}$, $\boldsymbol{u}(\boldsymbol{s})^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))\equiv0$, and $\nabla_\mathcal{L} U (\boldsymbol{\delta})-\boldsymbol{u}_\mathcal{L}(\boldsymbol{s})\equiv\nabla_\mathcal{L} U (\boldsymbol{\delta}^\ast)-\boldsymbol{u}_\mathcal{L}(\boldsymbol{s}^\ast)=\boldsymbol{p}_\mathcal{L}$. Clearly, $\boldsymbol{\omega}_\mathcal{G}\equiv\mathbbold{0}_{|\mathcal{G}|}$ implies that $\dot{\boldsymbol{\omega}}_\mathcal{G}\equiv\mathbbold{0}_{|\mathcal{G}|}$. By \eqref{eq:sys-dyn-vec-distribute-omegaL}, $\nabla_\mathcal{L} U (\boldsymbol{\delta})-\boldsymbol{u}_\mathcal{L}(\boldsymbol{s})\equiv\boldsymbol{p}_\mathcal{L}$ ensures that $\boldsymbol{\omega}_\mathcal{L}\equiv\mathbbold{0}_{|\mathcal{L}|}$. It follows from $\boldsymbol{\omega}_\mathcal{G}\equiv\mathbbold{0}_{|\mathcal{G}|}$ and $\boldsymbol{\omega}_\mathcal{L}\equiv\mathbbold{0}_{|\mathcal{L}|}$ that $\boldsymbol{\omega}\equiv\mathbbold{0}_{n}$, which further indicates that $\dot{\boldsymbol{\delta}}\equiv\mathbbold{0}_n$ by \eqref{eq:sys-dyn-vec-distribute-delta}. Finally, by Corollary~\ref{cor:sign-cross}, $\boldsymbol{u}(\boldsymbol{s})^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))\equiv0$ is equivalent to $\nabla C(\boldsymbol{u}(\boldsymbol{s}))\in\range{\mathbbold{1}_n}$ constantly. Hence, $\boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))\equiv\mathbbold{0}_{n}$, which together with $\boldsymbol{\omega}\equiv\mathbbold{0}_{n}$ implies that $\dot{\boldsymbol{s}}\equiv\mathbbold{0}_n$ based on \eqref{eq:bus-dyn}. Thus, we have shown that $\dot{W}(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})\equiv0$ implies $\dot{\boldsymbol{\delta}}\equiv\mathbbold{0}_n$, $\dot{\boldsymbol{\omega}}_{\mathcal{G}}\equiv\mathbbold{0}_{|\mathcal{G}|}$, and $\dot{\boldsymbol{s}}\equiv\mathbbold{0}_n$. This means that the largest invariant set contained in the set of points where $\dot{W}$ vanishes is actually the set of equilibria. Therefore, by the LaSalle invariance principle~\cite[Theorem~4.4]{khalil2002nonlinear}, every trajectory of the closed-loop system \eqref{eq:sys-dyn-vec-distribute} starting within $\mathcal{D}$ converges to the equilibrium set, which by Theorem~\ref{thm:equilibrium} consists of a unique  point satisfying \eqref{eq:equ-DAI}. This concludes the proof of local asymptotic stability.

% \begin{thm}[Local asymptotic stability]\label{thm:as-stable}
% Under Assumptions~\ref{ass:nonlinear-u} and~\ref{ass-cost-grad-scale}, the equilibrium of the closed-loop system \eqref{eq:sys-dyn-vec-distribute} characterized by \eqref{eq:equ-DAI} with $|\delta_i^\ast-\delta_j^\ast|\in [0,\pi/2)$, $\forall \{i,j\} \in\mathcal{E}$, is locally asymptotically stable.
%
%\marginJC{We're not using the notation $\mathcal{D}$ anymore?}
%
%\end{thm}
%
%\marginJC{The way the proof is worded, I don't see why the convergence is local. It sounds to me like the region of attraction is $\mathcal{D}$, no? So the result is global on this set.}
%
%\begin{proof}
% Using the expression of $\dot{W}(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})$ in~\eqref{eq:Wdot-distribute},
% it follows directly from the fact that $\boldsymbol{A}_\mathcal{G}\succ0$, $\boldsymbol{A}_\mathcal{L}^{-1}\succ0$, and $\boldsymbol{u}(\boldsymbol{s})^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))\geq0$ by Corollary~\ref{cor:sign-cross} that $\dot{W}(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})\leq0$.
% Applying Corollary~\ref{cor:ustar-null} to \eqref{eq:Wdot-distribute} yields
% \begin{align}\label{eq:Wdot-neg}
%     &\dot{W}(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})\\=&-2\pi f_0 \boldsymbol{\omega}_\mathcal{G}^T\boldsymbol{A}_\mathcal{G} \boldsymbol{\omega}_\mathcal{G}- \boldsymbol{u}(\boldsymbol{s})^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))\nonumber\\
%     &-2\pi f_0 \left(\nabla_\mathcal{L} U (\boldsymbol{\delta}^\ast)-\nabla_\mathcal{L} U (\boldsymbol{\delta})+\boldsymbol{u}_\mathcal{L}(\boldsymbol{s})-\boldsymbol{u}_\mathcal{L}(\boldsymbol{s}^\ast)\right)^T\boldsymbol{A}_\mathcal{L}^{-1}\nonumber\\&\quad\cdot\left(\nabla_\mathcal{L} U (\boldsymbol{\delta}^\ast)- \nabla_\mathcal{L} U (\boldsymbol{\delta})  + \boldsymbol{u}_\mathcal{L}(\boldsymbol{s})\!-\boldsymbol{u}_\mathcal{L}(\boldsymbol{s}^\ast)\right)\nonumber
%     \\
%     \leq&\ 0\nonumber\,,
% \end{align}
%where the inequality results from the fact that $\boldsymbol{A}_\mathcal{G}\succ0$, $\boldsymbol{A}_\mathcal{L}^{-1}\succ0$, and $\boldsymbol{u}(\boldsymbol{s})^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))\geq0$ by Corollary~\ref{cor:sign-cross}.
% Observe from \eqref{eq:Wdot-distribute} that $\dot{W}(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})\equiv0$ directly enforces $\boldsymbol{\omega}_\mathcal{G}\equiv\mathbbold{0}_{|\mathcal{G}|}$, $\boldsymbol{u}(\boldsymbol{s})^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))\equiv0$, and $\nabla_\mathcal{L} U (\boldsymbol{\delta})-\boldsymbol{u}_\mathcal{L}(\boldsymbol{s})\equiv\nabla_\mathcal{L} U (\boldsymbol{\delta}^\ast)-\boldsymbol{u}_\mathcal{L}(\boldsymbol{s}^\ast)=\boldsymbol{p}_\mathcal{L}$. Clearly, $\boldsymbol{\omega}_\mathcal{G}\equiv\mathbbold{0}_{|\mathcal{G}|}$ implies that $\dot{\boldsymbol{\omega}}_\mathcal{G}\equiv\mathbbold{0}_{|\mathcal{G}|}$. By \eqref{eq:sys-dyn-vec-distribute-omegaL}, $\nabla_\mathcal{L} U (\boldsymbol{\delta})-\boldsymbol{u}_\mathcal{L}(\boldsymbol{s})\equiv\boldsymbol{p}_\mathcal{L}$ ensures that $\boldsymbol{\omega}_\mathcal{L}\equiv\mathbbold{0}_{|\mathcal{L}|}$. It follows from $\boldsymbol{\omega}_\mathcal{G}\equiv\mathbbold{0}_{|\mathcal{G}|}$ and $\boldsymbol{\omega}_\mathcal{L}\equiv\mathbbold{0}_{|\mathcal{L}|}$ that $\boldsymbol{\omega}\equiv\mathbbold{0}_{n}$, which further indicates that $\dot{\boldsymbol{\delta}}\equiv\mathbbold{0}_n$ by \eqref{eq:sys-dyn-vec-distribute-delta}. Finally, by Corollary~\ref{cor:sign-cross}, $\boldsymbol{u}(\boldsymbol{s})^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))\equiv0$ is equivalent to $\nabla C(\boldsymbol{u}(\boldsymbol{s}))\in\range{\mathbbold{1}_n}$ constantly. Hence, $\boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))\equiv\mathbbold{0}_{n}$, which together with $\boldsymbol{\omega}\equiv\mathbbold{0}_{n}$ implies that $\dot{\boldsymbol{s}}\equiv\mathbbold{0}_n$ based on \eqref{eq:bus-dyn}. Thus, we have shown that $\dot{W}(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})\equiv0$ implies $\dot{\boldsymbol{\delta}}\equiv\mathbbold{0}_n$, $\dot{\boldsymbol{\omega}}_{\mathcal{G}}\equiv\mathbbold{0}_{|\mathcal{G}|}$, and $\dot{\boldsymbol{s}}\equiv\mathbbold{0}_n$. This means that the largest invariant set contained in the set of points where  $\dot{W}$ vanishes is actually the set of equilibria.  Therefore, by the LaSalle invariance principle~\cite[Theorem~4.4]{khalil2002nonlinear},
%
%\marginJC{So, after calling $W$ a Lyapunov function all the time above, it turns out it's not :-) since we use LaSalle.}
%
% every trajectory of the closed-loop system \eqref{eq:sys-dyn-vec-distribute} converges to the equilibrium set, which by Theorem~\ref{thm:equilibrium} consists of a unique  point satisfying \eqref{eq:equ-DAI}. This concludes the proof of local asymptotic stability.
% The stability under the generalized DAI can be certified by finding a well-defined Lyapunov function that is nonincreasing along the trajectories of the closed-loop system \eqref{eq:sys-dyn-vec-distribute}. In what follows, we study only the state $(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})$ without $\boldsymbol{\omega}_\mathcal{L}$ for a neighborhood $\mathcal{D}:=\! \Set*{(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})\!\in \!\real^n \!\!\times\! \real^{|\mathcal{G}|}\!\!\times\! \real^n}{|\delta_i-\delta_j|\in [0,\pi/2), \forall \{i,j\}\!\in \!\mathcal{E}}$ of the equilibrium $(\boldsymbol{\delta}^\ast, \mathbbold{0}_{|\mathcal{G}|}, \boldsymbol{s}^\ast)$ since $\boldsymbol{\omega}_\mathcal{L}$ is determined by $\boldsymbol{\delta}$ and $\boldsymbol{s}$ through the algebraic equation \eqref{eq:sys-dyn-vec-distribute-omegaL} which ensures that
% \begin{align*}
% &\ \|\boldsymbol{\delta}-\boldsymbol{\delta}^\ast\|^2+\|\boldsymbol{\omega}_\mathcal{G}\|^2+\|\boldsymbol{s}-\boldsymbol{s}^\ast\|^2\\\leq&\ \|\boldsymbol{\delta}-\boldsymbol{\delta}^\ast\|^2+\|\boldsymbol{\omega}\|^2+\|\boldsymbol{s}-\boldsymbol{s}^\ast\|^2\\\leq&\ \nu\left(\|\boldsymbol{\delta}-\boldsymbol{\delta}^\ast\|^2+\|\boldsymbol{\omega}_\mathcal{G}\|^2+\|\boldsymbol{s}-\boldsymbol{s}^\ast\|^2\right)    
% \end{align*}
% for some constant $\nu>0$
% by a similar argument as in~\cite[Lemma~4]{weitenberg2018exponential} provided that each $u_i(s_i)$ is Lipschitz continuous. This indicates that it suffices to investigate $(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})$. Therefore, we need to first find a well-defined Lyapunov function $W(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})$ such that $W(\boldsymbol{\delta}^\ast, \mathbbold{0}_{|\mathcal{G}|}, \boldsymbol{s}^\ast)=0$ and $W(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G},\boldsymbol{s})>0$, $\forall(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G},\boldsymbol{s})\in \mathcal{D}\setminus{(\boldsymbol{\delta}^\ast, \mathbbold{0}_{|\mathcal{G}|}, \boldsymbol{s}^\ast)}$, and then verify $\dot{W}(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})\leq0$, $\forall(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G},\boldsymbol{s})\in \mathcal{D}$.
% Inspired by \cite{DORFLER2017Auto}, we begin by defining the following integral function:
% \begin{align*}
% L(\boldsymbol{s}):=\sum_{i=1}^n \int_0^{s_i}u_i(\xi)\ \mathrm{d}\xi\,,    
% \end{align*}
% which clearly satisfies $\nabla L (\boldsymbol{s})=\boldsymbol{u}(\boldsymbol{s})$. We claim that $L(\boldsymbol{s})$ is strictly convex if $u_i(s_i)$ is strictly increasing with respect to $s_i$, $\forall i\in\mathcal{N}$. To see this, we note that, $\forall\boldsymbol{x}\neq\boldsymbol{y}\in\real^n$,
% \begin{align}
%     \left(\nabla L (\boldsymbol{x})-\nabla L (\boldsymbol{y})\right)^T\!\!\left(\boldsymbol{x}-\boldsymbol{y}\right)=&\left(\boldsymbol{u}(\boldsymbol{x})-\boldsymbol{u}(\boldsymbol{y})\right)^T\left(\boldsymbol{x}-\boldsymbol{y}\right)\nonumber\\=&\sum_{i=1}^n\!\left(u_i(x_i)-u_i(y_i)\right)\!\left(x_i-y_i\right)\nonumber\\>&\ 0\,,\label{eq:mono-gradL}
% \end{align}
% where the inequality results from the monotonicity of each $u_i(s_i)$. Thus, by~\cite[Theorem~2.14]{rockafellar1998}, \eqref{eq:mono-gradL} indicates the strict convexity of $L(\boldsymbol{s})$.
% After characterizing the properties of $L(\boldsymbol{s})$, we consider the following Lyapunov function candidate:
% \begin{align}\label{eq: Lyapunov}
% W(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s}):=&\ \pi f_0 \boldsymbol{\omega}_\mathcal{G}^T\boldsymbol{M}\boldsymbol{\omega}_\mathcal{G} \\&+ U(\boldsymbol{\delta})-U(\boldsymbol{\delta^\ast})-\nabla U (\boldsymbol{\delta^\ast})^T\left(\boldsymbol{\delta}-\boldsymbol{\delta^\ast}\right)\nonumber\\&+ L(\boldsymbol{s})-L(\boldsymbol{s^\ast})-\nabla L (\boldsymbol{s^\ast})^T\left(\boldsymbol{s}-\boldsymbol{s^\ast}\right)\,,\nonumber    \end{align}
% where $(\boldsymbol{\delta}^\ast, \mathbbold{0}_{|\mathcal{G}|}, \boldsymbol{s}^\ast)$ corresponds to the unique equilibrium point of the closed-loop system \eqref{eq:sys-dyn-vec-distribute} satisfying \eqref{eq:equ-DAI}.
% To see that \eqref{eq: Lyapunov} is a well-defined Lyapunov function on $\mathcal{D}$, we can bound it term by term. Clearly, the kinetic energy term $\pi f_0 \boldsymbol{\omega}_\mathcal{G}^T\boldsymbol{M}\boldsymbol{\omega}_\mathcal{G}>0$, $\forall \boldsymbol{\omega}_\mathcal{G}\neq \mathbbold{0}_{|\mathcal{G}|}$. By~\cite[Lemma~4]{weitenberg2018exponential}, the potential energy term $U(\boldsymbol{\delta})-U(\boldsymbol{\delta}^\ast)-\nabla U (\boldsymbol{\delta}^\ast)^T\left(\boldsymbol{\delta}-\boldsymbol{\delta}^\ast\right)\geq \beta\left\|\boldsymbol{\delta}-\boldsymbol{\delta}^{\ast}\right\|_2^2>0$, $\forall \boldsymbol{\delta}\neq \boldsymbol{\delta}^\ast$ satisfying $|\delta_i-\delta_j|\in [0,\pi/2)$, $\forall \{i,j\}\in \mathcal{E}$, for some constants $\beta>0$. By~\cite[Theorem~2.14]{rockafellar1998}, the strict convexity of $L(\boldsymbol{s})$ ensures that $L(\boldsymbol{s})-L(\boldsymbol{s^\ast})-\nabla L (\boldsymbol{s^\ast})^T\left(\boldsymbol{s}-\boldsymbol{s^\ast}\right)>0$, $\forall \boldsymbol{s}\neq \boldsymbol{s}^\ast$. It follows directly that $W(\boldsymbol{\delta}^\ast, \mathbbold{0}_{|\mathcal{G}|}, \boldsymbol{s}^\ast)=0$ and $W(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})>0, \forall(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})\in \mathcal{D}\setminus{(\boldsymbol{\delta}^\ast, \mathbbold{0}_{|\mathcal{G}|}, \boldsymbol{s}^\ast)}$, which means that the Lyapunov function $W(\boldsymbol{\delta}, \boldsymbol{\omega}, \boldsymbol{s})$ in~\eqref{eq: Lyapunov} is well-defined. 
% Now, we can examine the system stability through the derivative of  $W(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})$ along the trajectories of the closed-loop system \eqref{eq:sys-dyn-vec-distribute}, whose expression is given by
% \begin{alignat}{3}\label{eq:Wdot-distribute}
% &\dot{W}(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})\\
% =&\ 2\pi f_0 \boldsymbol{\omega}_\mathcal{G}^T\left(-
%     \boldsymbol{A}_\mathcal{G} \boldsymbol{\omega}_\mathcal{G}- \nabla_\mathcal{G} U (\boldsymbol{\delta}) + \boldsymbol{p}_\mathcal{G} + \boldsymbol{u}_\mathcal{G}(\boldsymbol{s})\right) \nonumber\\&+2\pi f_0\left(\nabla U (\boldsymbol{\delta})-\nabla U (\boldsymbol{\delta}^\ast)\right)^T\left(I_n-\frac{1}{n}\mathbbold{1}_n\mathbbold{1}_n^T\right)\boldsymbol{\omega}\nonumber\\&+ \left(\boldsymbol{u}(\boldsymbol{s})-\boldsymbol{u}(\boldsymbol{s}^\ast)\right)^T\left(-2 \pi f_0 \boldsymbol{\omega} - \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))\right)\nonumber\\
% &-2\pi f_0 \boldsymbol{\omega}_\mathcal{G}^T\left(- \nabla_\mathcal{G} U (\boldsymbol{\delta}^\ast) + \boldsymbol{p}_\mathcal{G} + \boldsymbol{u}_\mathcal{G}(\boldsymbol{s}^\ast)\right)\nonumber\\
% =&-2\pi f_0 \boldsymbol{\omega}_\mathcal{G}^T\boldsymbol{A}_\mathcal{G} \boldsymbol{\omega}_\mathcal{G}- \left(\boldsymbol{u}(\boldsymbol{s})-\boldsymbol{u}(\boldsymbol{s}^\ast)\right)^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))\nonumber\\
%     &-2\pi f_0 \left(\nabla_\mathcal{L} U (\boldsymbol{\delta}^\ast)-\nabla_\mathcal{L} U (\boldsymbol{\delta})+\boldsymbol{u}_\mathcal{L}(\boldsymbol{s})-\boldsymbol{u}_\mathcal{L}(\boldsymbol{s}^\ast)\right)^T\boldsymbol{\omega}_\mathcal{L}\nonumber\\
% =&-2\pi f_0 \boldsymbol{\omega}_\mathcal{G}^T\boldsymbol{A}_\mathcal{G} \boldsymbol{\omega}_\mathcal{G}- \boldsymbol{u}(\boldsymbol{s})^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))\nonumber\\
%     &-2\pi f_0 \left(\nabla_\mathcal{L} U (\boldsymbol{\delta}^\ast)-\nabla_\mathcal{L} U (\boldsymbol{\delta})+\boldsymbol{u}_\mathcal{L}(\boldsymbol{s})-\boldsymbol{u}_\mathcal{L}(\boldsymbol{s}^\ast)\right)^T\boldsymbol{A}_\mathcal{L}^{-1}\nonumber\\&\quad\cdot\left(- \nabla_\mathcal{L} U (\boldsymbol{\delta}) + \boldsymbol{p}_\mathcal{L} + \boldsymbol{u}_\mathcal{L}(\boldsymbol{s})\right)\nonumber\\
% =&-2\pi f_0 \boldsymbol{\omega}_\mathcal{G}^T\boldsymbol{A}_\mathcal{G} \boldsymbol{\omega}_\mathcal{G}- \boldsymbol{u}(\boldsymbol{s})^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))\nonumber\\
%     &-2\pi f_0 \left(\nabla_\mathcal{L} U (\boldsymbol{\delta}^\ast)-\nabla_\mathcal{L} U (\boldsymbol{\delta})+\boldsymbol{u}_\mathcal{L}(\boldsymbol{s})-\boldsymbol{u}_\mathcal{L}(\boldsymbol{s}^\ast)\right)^T\boldsymbol{A}_\mathcal{L}^{-1}\nonumber\\&\quad\cdot\left[- \!\nabla_\mathcal{L} U (\boldsymbol{\delta}) \!+\! \boldsymbol{p}_\mathcal{L} \!+\! \boldsymbol{u}_\mathcal{L}(\boldsymbol{s})\!-\!\left(- \!\nabla_\mathcal{L} U (\boldsymbol{\delta}^\ast) \!+\! \boldsymbol{p}_\mathcal{L} \!+\! \boldsymbol{u}_\mathcal{L}(\boldsymbol{s}^\ast)\right)\right]\nonumber\\
%     =&-2\pi f_0 \boldsymbol{\omega}_\mathcal{G}^T\boldsymbol{A}_\mathcal{G} \boldsymbol{\omega}_\mathcal{G}- \boldsymbol{u}(\boldsymbol{s})^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}))\nonumber\\
%     &-2\pi f_0 \left(\nabla_\mathcal{L} U (\boldsymbol{\delta}^\ast)-\nabla_\mathcal{L} U (\boldsymbol{\delta})+\boldsymbol{u}_\mathcal{L}(\boldsymbol{s})-\boldsymbol{u}_\mathcal{L}(\boldsymbol{s}^\ast)\right)^T\boldsymbol{A}_\mathcal{L}^{-1}\nonumber\\&\quad\cdot\left(\nabla_\mathcal{L} U (\boldsymbol{\delta}^\ast)- \nabla_\mathcal{L} U (\boldsymbol{\delta})  + \boldsymbol{u}_\mathcal{L}(\boldsymbol{s})\!-\boldsymbol{u}_\mathcal{L}(\boldsymbol{s}^\ast)\right)\nonumber\\
%     \leq&\ 0\nonumber\,.
% \end{alignat}
% Here, some tricks are used to add or remove terms for constructing a quadratic format without affecting the original value of  $\dot{W}(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})$. In the second equality, the property that $- \nabla_\mathcal{G} U (\boldsymbol{\delta}^\ast) + \boldsymbol{p}_\mathcal{G} + \boldsymbol{u}_\mathcal{G}(\boldsymbol{s}^\ast)=\mathbbold{0}_{|\mathcal{G}|}$ by Theorem~\ref{thm:equilibrium} is used. In the third equality, the fact that 
%  $\nabla U (\boldsymbol{\delta})^T\mathbbold{1}_n=0$ is used. In the fourth equality, the fact that $\boldsymbol{\omega}_\mathcal{L}$ is determined by $\boldsymbol{\delta}$ and $\boldsymbol{s}$ through the algebraic equation \eqref{eq:sys-dyn-vec-distribute-omegaL} and the property that $\boldsymbol{u}(\boldsymbol{s}^\ast)^T \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}= \mathbbold{0}_n^T$ by Corollary~\ref{cor:ustar-null} are used. In the fifth equality, the property that $- \nabla_\mathcal{L} U (\boldsymbol{\delta}^\ast) + \boldsymbol{p}_\mathcal{L} + \boldsymbol{u}_\mathcal{L}(\boldsymbol{s}^\ast)=\mathbbold{0}_{|\mathcal{L}|}$ by Theorem~\ref{thm:equilibrium} is used.
% Observe from \eqref{eq:Wdot-distribute} that $\dot{W}(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})\equiv0$ directly enforces $\boldsymbol{\omega}_\mathcal{G}\equiv\mathbbold{0}_{|\mathcal{G}|}$, $\boldsymbol{u}(\boldsymbol{s})^T \boldsymbol{C}\boldsymbol{L}_\mathrm{Q}\boldsymbol{C}\boldsymbol{u}(\boldsymbol{s})\equiv0$, and $\nabla_\mathcal{L} U (\boldsymbol{\delta})-\boldsymbol{u}_\mathcal{L}(\boldsymbol{s})\equiv\nabla_\mathcal{L} U (\boldsymbol{\delta}^\ast)-\boldsymbol{u}_\mathcal{L}(\boldsymbol{s}^\ast)=\boldsymbol{p}_\mathcal{L}$. Clearly, $\boldsymbol{\omega}_\mathcal{G}\equiv\mathbbold{0}_{|\mathcal{G}|}$ implies that $\dot{\boldsymbol{\omega}}_\mathcal{G}\equiv\mathbbold{0}_{|\mathcal{G}|}$. By \eqref{eq:sys-dyn-vec-distribute-omegaL}, $\nabla_\mathcal{L} U (\boldsymbol{\delta})-\boldsymbol{u}_\mathcal{L}(\boldsymbol{s})\equiv\boldsymbol{p}_\mathcal{L}$ ensures that $\boldsymbol{\omega}_\mathcal{L}\equiv\mathbbold{0}_{|\mathcal{L}|}$. It follows from $\boldsymbol{\omega}_\mathcal{G}\equiv\mathbbold{0}_{|\mathcal{G}|}$ and $\boldsymbol{\omega}_\mathcal{L}\equiv\mathbbold{0}_{|\mathcal{L}|}$ that $\boldsymbol{\omega}\equiv\mathbbold{0}_{n}$, which further indicates that $\dot{\boldsymbol{\delta}}\equiv\mathbbold{0}_n$ by \eqref{eq:sys-dyn-vec-distribute-delta}. Finally, since the Laplacian matrix is positive semidefinite~\cite{FB-LNS}, i.e., $\boldsymbol{L}_\mathrm{Q}\succeq 0$, by~\cite[Observation 7.1.6]{Horn2012MA}, $\boldsymbol{u}(\boldsymbol{s})^T \boldsymbol{C}\boldsymbol{L}_\mathrm{Q}\boldsymbol{C}\boldsymbol{u}(\boldsymbol{s})\equiv0$ is equivalent to $\boldsymbol{C}\boldsymbol{L}_\mathrm{Q}\boldsymbol{C}\boldsymbol{u}(\boldsymbol{s})\equiv\mathbbold{0}_{n}$, which together with $\boldsymbol{\omega}\equiv\mathbbold{0}_{n}$ implies that $\dot{\boldsymbol{s}}\equiv\mathbbold{0}_n$ based on \eqref{eq:bus-dyn}. Thus, we have shown that the invariant set $\dot{W}(\boldsymbol{\delta}, \boldsymbol{\omega}_\mathcal{G}, \boldsymbol{s})\equiv0$ enforces $\dot{\boldsymbol{\delta}}\equiv\mathbbold{0}_n$, $\dot{\boldsymbol{\omega}}_{\mathcal{G}}\equiv\mathbbold{0}_{|\mathcal{G}|}$, and $\dot{\boldsymbol{s}}\equiv\mathbbold{0}_n$. Therefore, by LaSalle invariance principle~\cite[Theorem~4.4]{khalil2002nonlinear}, every trajectory of the closed-loop system \eqref{eq:sys-dyn-vec-distribute} converges to an equilibrium set, which by Theorem~\ref{thm:equilibrium} possess a unique equilibrium point satisfying \eqref{eq:equ-DAI}. This concludes the proof of local asymptotic stability.
%\end{proof}

Theorem~\ref{thm:as-stable} shows that the closed-loop system \eqref{eq:sys-dyn-vec-distribute} under the generalized DAI is locally asymptotically stabilized to the unique equilibrium point characterized by Theorem~\ref{thm:equilibrium}, where the steady-state performance objectives are achieved even for a broader range of cost functions beyond quadratic ones. 



==> Secondary Control_Arxiv/RL.tex <==
In the previous section, we showed that any controller $\boldsymbol{u}$ that is monotonic and through the origin would drive the system to the optimal steady-state solution. However, different controllers in this class may lead to very different transient behaviors. In this section, we focus on integrating reinforcement learning (RL) into our proposed generalized DAI to design a controller that optimizes the transient performance of the system without jeopardizing its stability. Basically, after parameterizing the control policy $u_i(s_i)$ that maps the integral variable $s_i$ of the generalized DAI to the controllable power injection $u_i$ on each bus as a monotonic neural network, we train those neural networks by a RL algorithm based on a recurrent neural network (RNN)~\cite{cui2022tps}. 
% We now discuss this in more detail by mostly following the approach from~\cite{cui2022tps}. 

\subsection{Monotonic Neural Networks for Stability Guarantee}
% RL is a powerful tool for learning from interactions with an uncertain environment how to map situations to actions such that certain performance is optimized~\cite{Sutton2018RL}, which makes it quite suitable to address the optimal transient frequency control problem \eqref{eq:opt-ts} under unknown power disturbances. Yet, the Achilles' heel of standard RL algorithms is their lack of provable stability guarantees, which might pose a threat to the operation of power systems. Fortunately, we can overcome this stability issue by an ingenious parameterization of the control policy $u_i(s_i)$ that maps the integral variable $s_i$ of the generalized DAI to the controllable power injection $u_i$ on each bus.

Recall from Section~\ref{sec:Generalized-DAI} that the stability of the closed-loop system \eqref{eq:sys-dyn-vec-distribute} under the generalized DAI is ensured by any nonlinear control policy $u_i(s_i)$ that is a Lipschitz continuous and strictly increasing function of $s_i$ with $u_i(0)=0$ provided that the cost of each buses satisfy Assumption~\ref{ass-cost-grad-scale}. Within this class of stabilizing controllers, we want to find one that has the best transient performance. That is, we want to minimize the frequency excursions and control efforts when the frequencies are recovering to their nominal values. 

In principle, optimizing all controllers satisfying Assumption~\ref{ass:nonlinear-u} is an infinite-dimensional problem. To make the problem tractable, we need to parameterize $u_i(s_i)$ in some way. Neural networks emerge as as a natural candidate due to their potential for universal approximation~\cite{zhouNIPS2017express}. The key requirement we impose on any neural network used is that $u_i$ should be an increasing function that goes through the origin. 

Here we use the result in~\cite[Theorem~2]{cui2022tps}, which states any function of our interest can be approximated accurately enough by a single hidden layer fully-connected neural network with rectified linear unit (ReLU) activation functions\footnote{ReLU is a widely used activation function which applies  $\max \left(0,x\right)$ to any element $x$ of its argument.} for properly designed weights and biases of the neural network. Such a neural network is called a \emph{stacked ReLU monotonic neural network} whose architecture is provided in Fig.~\ref{fig:stack-relu-diagram}.


% Thus, it is desirable to parameterize $u_i(s_i)$ in a way such that there is a potential for universal approximation~\cite{zhouNIPS2017express} to any function satisfying above requirements summarized in Assumption~\ref{ass:nonlinear-u}. However, we also would like to avoid an infinite-dimensional optimization problem that is intractable. Clearly, neural networks are viable options for parameterizing $u_i(s_i)$ due to their expressiveness through a limited number of parameters~\cite{zhouNIPS2017express}. According to~\cite[Theorem~2]{cui2022tps}, any function of our interest can be approximated accurately enough by a single hidden layer fully-connected neural network with rectified linear unit (ReLU) activation functions for properly designed weights and biases of the neural network. Such a neural network is called a \emph{stacked ReLU monotonic neural network}~\cite[Lemma~5]{cui2022tps} whose architecture is provided in Fig.~\ref{fig:stack-relu-diagram}. 

As illustrated in Fig.~\ref{fig:stack-relu-diagram}, each stacked ReLU monotonic neural network is essentially a parameterized mapping from the state $s_i$ to the control $u_i$ with parameters $\boldsymbol{k}^{+}_{i}:=\left(k^+_{i,j}, j \in \mathcal{D} \right)$, $\boldsymbol{b}^{+}_{i}:=\left(b^+_{i,j}, j \in \mathcal{D} \right)$, $\boldsymbol{k}^{-}_{i}:=\left(k^-_{i,j}, j \in \mathcal{D} \right)$, and $\boldsymbol{b}^{-}_{i}:=\left(b^-_{i,j}, j \in \mathcal{D} \right)$, where $\mathcal{D}:=\{1,\dots, d\}$ and $2d$ is the number of neurons in the hidden layer. Here, the vectors $\boldsymbol{k}^{+}_{i}$ and $\boldsymbol{k}^{-}_{i}$ are referred to as the ``weight'' vectors and the vectors $\boldsymbol{b}^{+}_{i}$ and $\boldsymbol{b}^{-}_{i}$ are referred to as the ``bias'' vectors. 

\begin{figure}[ht]
\centering
\includegraphics[width=0.6\columnwidth]{monotonic_NN_v2}
\caption{Stacked ReLU monotonic neural network.}
\label{fig:stack-relu-diagram}
\end{figure}

These weights and biases restrict the shape of $u_i(s_i)$. The output of the top $d$ neurons in the hidden layer is zero to $s_i \leq 0$. Similarly, the bottom $d$ neurons zeros out any positive inputs. Therefore, we write $u_i(s_i)=u_i^+(s_i)+u_i^-(s_i)$, where $u_i^+(s_i)$ corresponds to the top $d$ neurons and operate if the input is positive, and $u_i^-(s_i)$ corresponds to the bottom $d$ neurons and operate if the input is negative. 
% Because of this symmetry, it suffices to study the function $u_i^+$ and show it is increasing for positive inputs. 

The input layer transforms the input $s_i$ linearly as $\left(s_i-b^+_{i,j}\right)$ and then processed by the ReLU in the $j$th hidden neuron, $\forall j \in \mathcal{D}$.  Denote ReLU operator as $\sigma(\cdot)$ for simplicity. Then, the output of the $j$th hidden neuron in the top part becomes $\sigma(s_i-b^+_{i,j})=\max \left(0,s_i-b^+_{i,j}\right)$, which is linearly weighted by $k^+_{i,j}$ before contributing to the final output. Therefore, the contribution from the $j$th hidden neuron to the final output is $k^+_{i,j}\sigma(s_i-b^+_{i,j})= k^+_{i,j}\max \left(0,s_i-b^+_{i,j}\right)$. Therefore, the $j$th hidden neuron is activated only if the state $s_i$ exceeds the threshold $b^+_{i,j}$, as illustrated in Fig.~\ref{fig:principle-stack}. At the output layer, the contributions from all $d$ hidden neurons in the top part yield  
\begin{align*}
u^{+}_i(s_i):=\sum_{j=1}^dk^+_{i,j}\sigma(s_i-b^+_{i,j})=\left(\boldsymbol{k}^{+}_{i}\right)^T\sigma\left(\mathbbold{1}_d s_i-\boldsymbol{b}^+_{i}\right)\,.    
\end{align*}
The negative part $u_i^-$ can be treated the same way. 

% \begin{align*}
% k^+_{i,j}\sigma(s_i-b^+_{i,j})=&\ k^+_{i,j}\max \left(0,s_i-b^+_{i,j}\right)\\=&
%     \begin{cases}
%     k^+_{i,j}(s_i-b^+_{i,j}) & \text{if}\ s_i>b^+_{i,j}\\
%     0 & \text{if}\ s_i\leq b^+_{i,j}
%     \end{cases}\,,\quad\forall j \in \mathcal{D}\,.\end{align*}
% To put it another way, 

Of course, for $u_i$ to be increasing, the weights and biases need to be constrained. We do this by making the slope always positive, as shown in Fig.~\ref{fig:control-curve}. This gives rise to the following requirements on weights and biases:  
\begin{subequations}\label{eq:cons-bk}
\begin{align}
    b^{-}_{i,d}\leq \dots \leq b^{-}_{i,2}\leq b^{-}_{i,1}\!=0&=b^{+}_{i,1}\leq b^{+}_{i,2}\leq\!\dots\leq b^{+}_{i,d}\,,\label{eq:bias}\\-\infty<\sum_{j=1}^{\iota} k^-_{i,j}<0&<\sum_{j=1}^{\iota} k^+_{i,j}<\infty\,,\ \forall \iota \in\! \mathcal{D}\,.\label{eq:weights}
\end{align}
\end{subequations}
If these are satisfied, the stacked ReLU monotonic neural network is a control policy $u_i(s_i)$ satisfying Assumption~\ref{ass:nonlinear-u}.
% with a shape as sketched in Fig.~\ref{fig:control-curve}.

\begin{figure}[t!]
\centering
\subfigure[Monotonic Control policy]
{\includegraphics[width=1\columnwidth]{control_policy_2.pdf}\label{fig:control-curve}}
\hfil
\subfigure[Principle of stacking hidden neurons]
{\includegraphics[width=1\columnwidth]{stacked_relu_2.pdf}\label{fig:principle-stack}}
\caption{Sketch of how hidden neurons in the $i$th stacked ReLU monotonic neural network help to form a control policy $u_i(s_i)$.}
\label{fig:piece-linear}
\end{figure}

The inequality constraints in \eqref{eq:cons-bk} are not trivial to enforce when training the neural network. It turns out there is a simple trick to address this challenge. We introduce a group of intermediate parameters $\boldsymbol{\mu}^{+}_{i}:=\left(\mu^+_{i,j}, j \in \mathcal{D} \right)\in \real^d$, $\boldsymbol{\chi}^{+}_{i}:=\left(\chi^+_{i,j}, j \in \mathcal{D}\setminus{\{d\}} \right)\in \real^{d-1}$, $\boldsymbol{\mu}^{-}_{i}:=\left(\mu^-_{i,j}, j \in \mathcal{D} \right)\in \real^d$, and $\boldsymbol{\chi}^{-}_{i}:=\left(\chi^-_{i,j}, j \in \mathcal{D}\setminus{\{d\}} \right)\in \real^{d-1}$ that are unconstrained. The original parameters $\boldsymbol{k}^{+}_{i}$, $\boldsymbol{b}^{+}_{i}$, $\boldsymbol{k}^{-}_{i}$, and $\boldsymbol{b}^{-}_{i}$ are given by
\begin{subequations}
\begin{align}
\!\!\!\!&k^+_{i,1}\!=\!\left(\mu^+_{i,1}\right)^2\!\!\!\,,\  k^+_{i,j}\!=\!\left(\mu^+_{i,j}\right)^2\!\!-\!\left(\mu^+_{i,j-1}\right)^2\!\!\,,\ \!\forall j \!\in\! \mathcal{D}\!\setminus{\!\{1\}}\,,\\
\!\!\!\!&k^-_{i,1}\!=-\left(\mu^-_{i,1}\right)^2\,,\  k^-_{i,j}=-\left(\mu^-_{i,j}\right)^2+\left(\mu^-_{i,j-1}\right)^2\,,\\
\!\!\!\!&b^+_{i,1}\!=b^-_{i,1}\!=0\,,\ b^+_{i,j}\!=\!\!\sum_{l=1}^{j-1}\!\left(\chi^+_{i,l}\right)^2\!\!\!\,,\ b^-_{i,j}\!=\!-\!\!\sum_{l=1}^{j-1}\!\left(\chi^-_{i,l}\right)^2\!\!\!\,.
\end{align}
\end{subequations}
In this way, the requirements in \eqref{eq:cons-bk} naturally hold. Thus, the remaining problem is just the search of optimal parameters $\boldsymbol{\mu}^{+}_{i}$, $\boldsymbol{\chi}^{+}_{i}$, $\boldsymbol{\mu}^{-}_{i}$, and $\boldsymbol{\chi}^{-}_{i}$ through the training of neural networks. To highlight the dependence of the control policy $u_i(s_i)$ generated by the $i$th neural network on parameters $\boldsymbol{\mu}^{+}_{i}$, $\boldsymbol{\chi}^{+}_{i}$, $\boldsymbol{\mu}^{-}_{i}$, and $\boldsymbol{\chi}^{-}_{i}$, we will use the notation $u_i(s_i;\Xi_i(d))$ in the rest of this manuscript, where $\Xi_i(d)$ denote a set of parameters $\Xi_i:=\{\boldsymbol{\mu}^{+}_{i},\boldsymbol{\chi}^{+}_{i},\boldsymbol{\mu}^{-}_{i},\boldsymbol{\chi}^{-}_{i}\}$ associated with a stacked ReLU monotonic neural network that has $2d$ hidden neurons.

% The requirements on biases in \eqref{eq:bias} assign the top $d$ and bottom $d$ hidden neurons to take charge of the control policy $u_i(s_i)$ for $s_i\geq 0$ and $s_i\leq 0$, respectively, since they are deactivated if it is the other way around, where a by-product of $b^{-}_{i,1}=0=b^{+}_{i,1}$ is $u_i(0)=0$. The requirements on weights in \eqref{eq:weights} simply ensure that the slope of the control policy curve $u_i(s_i)$ is always positive and finite.

% To see how this neural network architecture finesses the task of providing the desired continuity and monotonicity of the mapping $u_i(s_i)$, we now explain the operations it performs in more detail. Firstly, observe from Fig.~\ref{fig:stack-relu-diagram} that the top $d$ hidden neurons perform similar operations to produce $u_i^+(s_i)$ and the bottom $d$ hidden neurons perform similar operations to produce $u_i^-(s_i)$, where $u_i(s_i)=u_i^+(s_i)+u_i^-(s_i)$. Thus, it is natural to investigate the neural network by this partition. 

% For the top part, the state $s_i$ is transformed linearly as $\left(s_i-b^+_{i,j}\right)$ and then processed by the ReLU in the $j$th hidden neuron, $\forall j \in \mathcal{D}$.  

% Denote ReLU operator as $\sigma(\cdot)$ for simplicity. Then, the output of the $j$th hidden neuron in the top part becomes $\sigma(s_i-b^+_{i,j})=\max \left(0,s_i-b^+_{i,j}\right)$, which is linearly weighted by $k^+_{i,j}$ before contributing to the final output. Therefore, the contribution from the $j$th hidden neuron to the final output is 
% \begin{align*}
% k^+_{i,j}\sigma(s_i-b^+_{i,j})=&\ k^+_{i,j}\max \left(0,s_i-b^+_{i,j}\right)\\=&
%     \begin{cases}
%     k^+_{i,j}(s_i-b^+_{i,j}) & \text{if}\ s_i>b^+_{i,j}\\
%     0 & \text{if}\ s_i\leq b^+_{i,j}
%     \end{cases}\,,\quad\forall j \in \mathcal{D}\,.\end{align*}
% To put it another way, the $j$th hidden neuron is activated only if the state $s_i$ exceeds the threshold $b^+_{i,j}$, as illustrated in Fig.~\ref{fig:principle-stack}. At the output layer, the contributions from all $d$ hidden neurons in the top part yield  
% \begin{align*}
% u^{+}_i(s_i):=\sum_{j=1}^dk^+_{i,j}\sigma(s_i-b^+_{i,j})=\left(\boldsymbol{k}^{+}_{i}\right)^T\sigma\left(\mathbbold{1}_d s_i-\boldsymbol{b}^+_{i}\right)\,.    
% \end{align*}
% The bottom part follows the similar logic, where the $d$ hidden neurons produce
% \begin{align*}
% u^{-}_i(s_i):=\sum_{j=1}^dk^-_{i,j}\sigma(b^-_{i,j}-s_i)=\left(\boldsymbol{k}^{-}_{i}\right)^T\sigma\left(\boldsymbol{b}^-_{i}-\mathbbold{1}_d s_i\right)\,.    
% \end{align*}
% Clearly, the final output is a result of contributions from all $2d$ hidden neurons, which means $u_i(s_i)=u_i^+(s_i)+u_i^-(s_i)$. Last but not least, in order to let $u_i(s_i)$ satisfy Assumption~\ref{ass:nonlinear-u}, we have to adopt weights and biases that are tailor-made rather than allow them to be arbitrarily trainable. 

% This can be done by taking a lot of inspiration from Fig.~\ref{fig:piece-linear}, where the control policy $u_i(s_i)$ satisfies Assumption~\ref{ass:nonlinear-u} since the top $d$ hidden neurons form a control policy $u_i^+(s_i)$ satisfying Assumption~\ref{ass:nonlinear-u} for any state $s_i\geq 0$ and the bottom $d$ hidden neurons form a control policy $u_i^-(s_i)$ satisfying Assumption~\ref{ass:nonlinear-u} for any state $s_i\leq 0$. Intuitively, no matter where the state $s_i$ is, the net slope it experiences on the control policy curve $u_i(s_i)$ should always be positive and finite, as shown in Fig.~\ref{fig:control-curve}. This intuition gives rise to the following requirements on weights and biases:  
% \begin{subequations}\label{eq:cons-bk}
% \begin{align}
%     b^{-}_{i,d}\leq \dots \leq b^{-}_{i,2}\leq b^{-}_{i,1}\!=0&=b^{+}_{i,1}\leq b^{+}_{i,2}\leq\!\dots\leq b^{+}_{i,d}\,,\label{eq:bias}\\-\infty<\sum_{j=1}^{\iota} k^-_{i,j}<0&<\sum_{j=1}^{\iota} k^+_{i,j}<\infty\,,\ \forall \iota \in\! \mathcal{D}\,.\label{eq:weights}
% \end{align}
% \end{subequations}
% The requirements on biases in \eqref{eq:bias} assign the top $d$ and bottom $d$ hidden neurons to take charge of the control policy $u_i(s_i)$ for $s_i\geq 0$ and $s_i\leq 0$, respectively, since they are deactivated if it is the other way around, where a by-product of $b^{-}_{i,1}=0=b^{+}_{i,1}$ is $u_i(0)=0$. The requirements on weights in \eqref{eq:weights} simply ensure that the slope of the control policy curve $u_i(s_i)$ is always positive and finite. If these requirements are satisfied, the stacked ReLU monotonic neural network shown in Fig.~\ref{fig:stack-relu-diagram} is ensured to produce a control policy $u_i(s_i)$ satisfying Assumption~\ref{ass:nonlinear-u} with a shape as sketched in Fig.~\ref{fig:control-curve}.

% % \begin{align}
% %     b^{+}_{i,1}=b^{-}_{i,1}=0\,,b^{+}_{i,j}<b^{+}_{i,j+1}\,,b^{-}_{i,j}>b^{-}_{i,j+1}\,,\forall j \in \mathcal{D}\setminus{\{d\}}\\\sum_{j=1}^{\iota} k^+_{i,j}
% % \end{align}



\subsection{Recurrent Neural Network-Based Reinforcement Learning}\label{ssec:RNN-train}
A recurrent neural network (RNN) is a class of neural networks that have a looping mechanism to allow information learned from the previous step to flow to the next step.
% This feature makes a RNN an expert in learning parameters related to dynamic systems, where the prior states usually affect the following states. 
Thus, to efficiently train the stacked ReLU monotonic neural networks for parameters $\Xi_i(d)$, $\forall i \in\! \mathcal{N}$,  we adopt the RNN-based RL algorithm proposed by~\cite{cui2022tps}, whose scheme is shown in Fig.~\ref{fig:RL}. 

To fit into the RNN architecture, we have to discretize the problem \eqref{eq:opt-ts}. Let the $l$th sampling instant after the initial time $t_0$ be $(t_0 + lh)$, where $h$ is the sampling interval that is small enough. Then, using voltage angles $\boldsymbol{\theta}:=\left(\theta_i, i \in \mathcal{N} \right) \in \real^n$ as an example, we would like to approximate the continuous-time state at the $l$th sampling instant $\boldsymbol{\theta}(t_0 + lh)$ as a discrete-time state $\boldsymbol{\theta}^{\langle l\rangle}$. Provided that $\boldsymbol{\theta}^{\langle 0\rangle} = \boldsymbol{\theta}(t_0)$, the simplest way to obtain $\boldsymbol{\theta}^{\langle l\rangle} \approx \boldsymbol{\theta}(t_0 + lh)$ is through the reccurence relation via Euler method, i.e., $\boldsymbol{\theta}^{\langle l+1\rangle} \!= \boldsymbol{\theta}^{\langle l\rangle} + 2 \pi f_0 h \boldsymbol{\omega}^{\langle l\rangle}$. We solve the discretized problem below instead:   
\begin{eqnarray}
		\label{eq:opt-ts-obj-dt}
		\min_{\Xi_i(d), i \in \mathcal{N}} \!\!\!\!\!\!\!&& \sum_{i \in \mathcal{G}} \|\omega_i^{\langle l\rangle}\|_\infty+\rho\sum_{i=1}^n\tilde{C}_{i,T}  \label{eq:opt-ts-dis} \\
		\label{eq:opt-ts-con-dis}
		\mathrm{s.t.} \!\!\!\!\!\!\!\!&& \boldsymbol{\omega}_\mathcal{G}^{\langle l+1\rangle} \!\!=\! \left(I_{|\mathcal{G}|}-
    h\boldsymbol{M}^{-1}\boldsymbol{A}_\mathcal{G}\right) \boldsymbol{\omega}_\mathcal{G}^{\langle l\rangle}\nonumber\\&&\qquad\qquad\!\!+h\boldsymbol{M}^{-1}\!\left(\! - \nabla_\mathcal{G} U (\boldsymbol{\theta}^{\langle l\rangle})\!+\!\boldsymbol{p}_\mathcal{G}\!+\! \boldsymbol{u}_\mathcal{G}(\boldsymbol{s}^{\langle l\rangle})\right)\!\!\,,\nonumber\\
    && \boldsymbol{\omega}_\mathcal{L}^{\langle l\rangle} = \ \boldsymbol{A}_\mathcal{L}^{-1}\left(- \nabla_\mathcal{L} U (\boldsymbol{\theta}^{\langle l\rangle}) + \boldsymbol{p}_\mathcal{L} + \boldsymbol{u}_\mathcal{L}(\boldsymbol{s}^{\langle l\rangle})\right)\,,\nonumber\\
    &&  
    \boldsymbol{\theta}^{\langle l+1\rangle} \!= \boldsymbol{\theta}^{\langle l\rangle} + 2 \pi f_0 h \boldsymbol{\omega}^{\langle l\rangle}\,,\nonumber\\
    &&\boldsymbol{s}^{\langle l+1\rangle} \!= \boldsymbol{s}^{\langle l\rangle}\! -\!h\!\left(2 \pi f_0 \boldsymbol{\omega}^{\langle l\rangle}\! +\! \boldsymbol{Z}\boldsymbol{L}_\mathrm{Q}\nabla C(\boldsymbol{u}(\boldsymbol{s}^{\langle l\rangle}))\right)\!\!\,,\nonumber\\&&\boldsymbol{u}(\boldsymbol{s}^{\langle l\rangle}):=\left(u_i(s_i^{\langle l\rangle};\Xi_i(d)), i \in \mathcal{N} \right)\,,\nonumber
	\end{eqnarray}
with
\begin{subequations}\label{eq:compute-loss}
\begin{align}
    &\|\omega_i^{\langle l\rangle}\|_\infty:=\max_{l\in\{0,\dots, \lfloor T/h\rfloor-1\}} |\omega_i^{\langle l+1\rangle}|\,,\\ &\tilde{C}_{i,T}:=\dfrac{1}{\lfloor T/h\rfloor} \!\!\!\sum_{l=0}^{\lfloor T/h\rfloor-1}\!\!\!C_i(u_i(s_i^{\langle l\rangle};\Xi_i(d)))\,,
\end{align}
\end{subequations}
where $\lfloor T/h\rfloor$ denotes the floor of $T/h$.

\begin{figure}[t!]
\centering
\subfigure[RL scheme for training stacked ReLU monotonic neural networks]
{\includegraphics[width=0.75\columnwidth]{RL_scheme.pdf}\label{fig:RL}}
\hfil
\subfigure[Structure of the recurrent neural network cell]
{\includegraphics[width=0.9\columnwidth]{RNN_cell.pdf}\label{fig:rnn-cell}}
\caption{Illustration of the RNN-based RL algorithm.}
\end{figure}


After a random initialization of $\{\Xi_i(d), i \in\mathcal{N}\}$, the RNN-based RL algorithm solves the problem \eqref{eq:opt-ts-obj-dt} by gradually learning the optimal $\{\Xi_i(d), i \in\mathcal{N}\}$ through an iterative process mainly composed of three parts --- sampled trajectories generation, loss function evaluation, and backpropagation-based policy improvement --- as illustrated in Fig.~\ref{fig:RL}. For a given operating point $(\boldsymbol{\theta}^{\langle 0\rangle}, \boldsymbol{\omega}_\mathcal{G}^{\langle 0\rangle}, \boldsymbol{s}^{\langle 0\rangle})$ of the power system, a sample of system trajectory over a time horizon $T$ following sudden power disturbances can be generated by randomly initializing the constant input $\boldsymbol{p}$ to the RNN cell and then simulating forward $\lfloor T/h\rfloor$ time steps. The detailed structure of the RNN cell is shown in Fig.~\ref{fig:rnn-cell}, where the control signals $\boldsymbol{u}(\boldsymbol{s}^{\langle l\rangle})$ produced by $n$ stacked ReLU monotonic neural networks with parameters $\{\Xi_i(d), i \in\mathcal{N}\}$ are applied to the discretized closed-loop system with states $(\boldsymbol{\theta}^{\langle l\rangle}, \boldsymbol{\omega}_\mathcal{G}^{\langle l\rangle}, \boldsymbol{s}^{\langle l\rangle})$ for the generation of $(\boldsymbol{\theta}^{\langle l+1\rangle}, \boldsymbol{\omega}_\mathcal{G}^{\langle l+1\rangle}, \boldsymbol{s}^{\langle l+1\rangle})$. In this way, the RNN cell evolves forward for $l=0,\dots, \lfloor T/h\rfloor-1$, which yields one trajectory under the parameters $\{\Xi_i(d), i \in\mathcal{N}\}$ that are shared temporally. The loss function related to this trajectory is defined as the objective function of the problem \eqref{eq:opt-ts-obj-dt}, which can be computed by applying \eqref{eq:compute-loss} to the stored historical outputs of the RNN cell. Usually, to improve the efficiency of training, multiple trajectories are generated parallelly, where each of them is excited by a randomly initialized constant input $\boldsymbol{p}$. The collection of these  trajectories is called a batch and the number of such trajectories is called the batch size. Then, the loss function related to a batch of size $|\mathcal{B}|$ is defined as the mean of the losses related to individual trajectories in the batch, i.e.,
\begin{align*}
    J(\{\Xi_i(d), i \in \mathcal{N}\}):=\!\dfrac{1}{|\mathcal{B}|}\!\sum_{b=1}^{|\mathcal{B}|}\!\left(\sum_{i \in \mathcal{G}} \|\omega_i^{\langle l\rangle}\|_\infty+\rho\sum_{i=1}^n\tilde{C}_{i,T}\right)^{[b]}\!\!\!\,,
\end{align*}
where, with abuse of notation, we simply introduce a superscript $[b]$ to denote the loss along the $b$th trajectory in the batch rather than accurately distinguish $\|\omega_i^{\langle l\rangle}\|_\infty$ and $\tilde{C}_{i,T}$ along different trajectories to avoid complicating the notations too much. Once the loss of the batch $J(\{\Xi_i(d), i \in \mathcal{N}\})$ has been calculated, the parameters $\{\Xi_i(d), i \in\mathcal{N}\}$ are adjusted according to the batch gradient descent method with a suitable learning rate $\xi$, i.e.,
\begin{align*}
    \{\Xi_i(d), i \in \mathcal{N}\}\leftarrow\{\Xi_i(d), i \in \mathcal{N}\}-\xi\nabla J(\{\Xi_i(d), i \in \mathcal{N}\})\,,
\end{align*}
where the gradient is approximated efficiently through backward gradient propagation. This ends one epoch of the iterative training process. The procedure is repeated until the number of epochs $E$ is reached, which produces the optimal $\{\Xi_i(d), i \in\mathcal{N}\}$ for the stacked ReLU monotonic neural networks so that the corresponding control policy $u_i(s_i;\Xi_i(d))$ on each bus helps the generalized DAI to best handle the optimal transient frequency control problem \eqref{eq:opt-ts}.
% After the optimal control policy $\boldsymbol{u}(\boldsymbol{s})=\left(u_i(s_i;\Xi_i(d)), i \in \mathcal{N} \right)$ is learned, the complete generalized DAI can be used in real-time power systems.






% backpropagation to minimize the objective function of the optimal transient frequency control problem \eqref{eq:opt-ts} along a batch of sampled trajectories generated by running the control policies .



%With this in mind,

==> Secondary Control_Arxiv/intro.tex <==
\IEEEPARstart{T}{he} key to the normal operation of a power system is the balance between electric power supply and demand over the network~\cite{Kirschen2019eco}. For instance, the main cause of the 2021 Texas power crisis is that the deficient supply of power due to frozen equipment could not meet the high demand for electricity in cold weather. A system frequency deviation from its nominal value is a reflection of a power imbalance~\cite{Eto2010lbnl}, which makes frequency control a vital task of grid operators. Traditionally, this task is performed in a hierarchical structure composed of three layers with timescale separation: primary---droop control ($\SI{<20}{\second}$), secondary---frequency restoration ($\SI{30}{\second}$--$\SI{10}{\minute}$), and tertiary---economic dispatch ($\SI{>15}{\minute}$)~\cite{Eto2010lbnl}. 

Nowadays, power systems are experiencing a change in the mix of generation, where conventional synchronous generators are gradually being replaced by renewable energy sources like solar and wind energy~\cite{benjamin2017}. It is anticipated that the renewable share of the electricity generation mix in the United States will double from $21\%$ in 2020 to $42\%$ in 2050~\cite{eia2021outlook}. Intermittent renewable sources are typically inverter-interfaced, which may adversely affect the robustness of the frequency dynamics due to the loss of inertia~\cite{nrel2013renew}. This exposes power systems to larger and faster frequency fluctuations than before, which has motivated
active research on flexible distributed frequency control schemes that can break the hierarchy by addressing simultaneously frequency degradation
%
%\marginJC{We've talked about 'frequency dynamics' and 'frequency stability'. Is that what you mean by 'frequency security'? I wouldn't introduce a new term}
%
and economic efficiency at a fast timescale.

A key challenge in frequency control is that the power imbalances across the network are not explicitly known. A number of studies have proposed distributed algorithms to overcome this challenge. The works in~\cite{Zhao2015acc, li2016tcns, mallada2017optimal, DORFLER2017Auto, SCHIFFER2017auto, weitenberg2018exponential, Wang2019tsg, you2021tac,TS-AC-CDP-AJS-JC:21-auto} focus on optimizing the steady-state frequency and economic performance using a principled design of fixed updating rules involving agent communication for control dynamics. The approaches mainly fall in two categories. The first category~\cite{li2016tcns, mallada2017optimal, Wang2019tsg, you2021tac,TS-AC-CDP-AJS-JC:21-auto} rests on a primal-dual interpretation of power system dynamics under a properly designed optimization problem. This approach, however, always requires the estimation of certain system parameters. The second category~\cite{Zhao2015acc, DORFLER2017Auto, SCHIFFER2017auto, weitenberg2018exponential} builds upon various consensus algorithms to converge to an equilibrium with nominal frequency and economic efficiency. A notable example in this category is the distributed averaging-based integral (DAI) mechanism~\cite{Zhao2015acc, Johannes2016ecc, SCHIFFER2017auto, weitenberg2018exponential}, where the controllable
power injections are directly proportional to the integrals of frequency deviation and economic inefficiency signals. A key caveat to this approach is that DAI control has been so far restricted to quadratic cost functions. 

The works above focus on the optimization of the steady-state performance and do not typically consider the transient performance along the system trajectories following power disturbances. In fact, the optimization of transient performance is a challenging problem due to the nonlinearity of power dynamics and the uncertainty in power disturbances. Reinforcement learning (RL)~\cite{Sutton2018RL} is a powerful tool for learning from interactions with uncertain environments and determining how to map situations to actions so that a desired performance is optimized. By virtue of the above feature, RL has emerged~\cite{Ernst2004tps,Chen_2022tsg}  as an effective instrument to address the optimal transient frequency control problem in nonlinear power systems under unknown power disturbances. Nevertheless, the Achilles' heel of standard RL algorithms is their lack of provable stability guarantees, which presents a significant barrier to its practical implementation for the operation of power systems. In fact, many works~\cite{Ye2011tps, Singh2017tie, Yan2020tps, Chen2021tii}
optimize the transient performance by learning control policies that exhibit good performance against data but without any provable guarantees on steady-state performance. The recent paper~\cite{cui2022tps} on RL for optimal primary frequency control proposes a way to address the stability issue by identifying a set of properties that make a control design stabilizing and then restricting the search space of neural network-based controllers. In this paper, we extend this idea to achieve provable guarantees on frequency restoration and economic efficiency at the steady-state. 
%
%\marginJC{Since we're doing the lit review here, I think this is the best place to introduce the idea of~\cite{cui2022tps} (instead of later). We can say something like "\cite{cui2022tps} proposes a way to address these shortcomings by identifying a set of properties that make a control design stabilizing and then restricting the search space of RL to such controllers. In this way, the obtained design enjoys provable guarantees on stability" or something like that. We can point out that here we build on this approach.}
%

With the aim of filling the gap between the optimization of steady-state and transient frequency control performance, we propose to unify
these two perspectives by integrating RL into DAI control. In our approach, we employ RL to seek optimal control policies in terms of the transient performance as a map from the integral variables of DAI to the controllable power injections, while DAI inherently ensures the optimal steady-state performance. This results in a nonlinear optimal frequency controller which we term \emph{RL-DAI control} that generalizes the standard DAI approach.
%
% \marginJC{Maybe we can come up with a more informative name? "Generalized" is too generic, i think. How about RL-DAI or something like that?}
%
Specifically, the generalization is manifold:
\begin{itemize}
\item Unlike the classic DAI control that only addresses quadratic operational cost functions,  RL-DAI control admits any strictly convex cost functions
whose gradients are identical up to heterogeneous scaling
factors;
\item Unlike RL methods that do not  provide stability guarantees, RL-DAI control encodes the stabilization requirement on the control policy as mild conditions on its continuity and monotonicity properties. Such conditions can be easily realized by an ingenious parameterization of the control policy as a monotonic neural network,
% to be
which is trained by a RL algorithm based on recurrent neural networks (RNNs);
%
%\marginJC{This last sentence is the one that I'd move to the discussion earlier.}
%
\item RL-DAI control jointly optimizes both steady-state and transient frequency control performance by leveraging the added degrees of freedom in tuning parameters that characterize the nonlinear control policy.
\end{itemize}

The rest of this manuscript is organized as follows. Section~\ref{Sec:modelling}
describes the power system model and formalizes the optimal frequency control problem. Section~\ref{sec:Generalized-DAI} describes the proposed generalized DAI control and shows how it guarantees the asymptotic convergence of the closed-loop system to the equilibrium that achieves the steady-state
performance objectives. Section~\ref{sec:RL} illustrates how to integrate RL with DAI control such that the transient performance can be optimized without jeopardizing stability. Section~\ref{sec:simu} validates our results
through detailed simulations. We gather our conclusions and ideas for future work in Section~\ref{sec:conclusion}.










==> Secondary Control_Arxiv/model.tex <==
In this section, we describe the power system model used in this paper for analysis and the frequency control problem we aim to address.

\subsection{Power System Model}
We consider\footnote{Throughout this manuscript, vectors are denoted in lower case bold and matrices are denoted in upper case bold, while scalars are unbolded, unless otherwise specified. Also, $\mathbbold{1}_n, \mathbbold{0}_n \in \real^n$ denote the vectors of all ones and all zeros, respectively.} a $n$-bus power system whose topology can be characterized by a weighted undirected connected graph $\left(\mathcal{V},\mathcal{E} \right)$, where buses indexed by $i,j \in \mathcal{N} :=\{1,\dots, n\} $ are linked through transmission lines denoted by unordered pairs $\{i,j\} \in \mathcal{E} \subset \Set*{\{i,j\}}{i,j\in\mathcal{N},i\not=j}$.

Within the set of buses $\mathcal{N}$, we consider two subsets: the buses with generators\footnote{The generator buses can have collocated loads}  $\mathcal{G}$ and buses that are purely loads $\mathcal{L}$. Generator buses are described with differential equations, while load buses are treated as frequency-sensitive loads governed by algebraic equations. 
% disjoint union of the set of generator buses $\mathcal{G}$ and the set of load buses $\mathcal{L}$, i.e., $\mathcal{N}=\mathcal{G}\uplus\mathcal{I}$.
%
% \marginJC{I'm not familiar with the notation $\uplus$. How is it different from just $\cup$?}
%
More precisely, given net power injections $\boldsymbol{p} := \left(p_{i}, i \in \mathcal{N} \right) \in \real^n$
%
%\marginJC{How about $\{p_{i}\}_{i \in \mathcal{N}} \subset \real^n$ instead?}
%
on each bus, the dynamics of the voltage angle $\theta_i$ (in $\SI{}{\radian/s}$) and the frequency deviation $\omega_i$ (in $\SI{}{\pu}$) from the nominal frequency $f_0$ ($\SI{50}{\hertz}$ or $\SI{60}{\hertz}$ depending on the particular system) evolve according to
% \begin{subequations}\label{eq:sys-dyn-theta}
% \begin{align}
%     \dot{\theta}_i =&\ 2 \pi f_0 \omega_i\,,\!\!\!\!&&\forall i\in\mathcal{N}\!\,,\\
%     m_i \dot{\omega}_i \!=\!& -
%     \alpha_i \omega_i\!-\!\! \sum_{j=1}^n\! v_iv_jB_{ij}\sin{\left(\theta_i\!-\!\theta_j\right)}\! +\! p_{i} \!+\! u_{i}\,,\!\!\!\!&&\forall i\in\mathcal{G}\,,\\
%     0 =& -
%     \alpha_i \omega_i-\!\! \sum_{j=1}^n\! v_iv_jB_{ij}\sin{\left(\theta_i\!-\!\theta_j\right)} \!+\! p_{i} \!+\! u_{i}\,,\!\!\!\!&&\forall i\in\mathcal{L}\,,\label{eq:bus-dyn}\end{align}
% \end{subequations}
\begin{subequations}\label{eq:sys-dyn-theta}
\begin{align}
    \dot{\theta}_i \!=&\!\ 2 \pi f_0 \omega_i\,,\!\!\!\!\!\!&&\!\forall i\!\in\!\mathcal{N}\!\!\,,\\
    m_i \dot{\omega}_i \!=\!& -\!
    \alpha_i \omega_i\!-\!\! \!\sum_{j=1}^n\! v_iv_jB_{ij}\!\sin{\left(\theta_i\!-\!\theta_j\right)}\! +\! p_{i} \!+\! u_{i}\,,\!\!\!\!\!\!&&\forall i\!\in\!\mathcal{G}\!\,,\\
    0 \!=&\! -\!
    \alpha_i \omega_i\!-\!\!\! \sum_{j=1}^n\! v_iv_jB_{ij}\!\sin{\left(\theta_i\!-\!\theta_j\right)} \!+\! p_{i} \!+\! u_{i}\,,\!\!\!\!\!\!&&\forall i\!\in\!\mathcal{L}\!\,,\end{align}
\end{subequations}
where the parameters are defined as: $m_i:=2H_i>0$ --- generator inertia constant (in $\SI{}{\second}$), $\alpha_i>0$ --- frequency sensitivity coefficient from generator or load (in $\SI{}{\pu}$) depending on whether $i \in \mathcal{G}$ or $i \in \mathcal{L}$, $v_i>0$ --- voltage magnitude (in $\SI{}{\pu}$), and $B_{ij}$ --- susceptance (in $\SI{}{\pu}$). The susceptances define coupling between buses in the system and satisfies $B_{ij}=B_{ji}>0$ if $\{i,j\} \in\mathcal{E}$ and $B_{ij}=B_{ji}=0$ if $\{i,j\} \not\in\mathcal{E}$. Finally, $u_{i}$ is a controllable power injection to be designed for secondary frequency control.



\begin{rem}[Model assumptions]\label{rem:model}
We make the following assumptions: 
\begin{itemize}
\item Lossless lines: $\forall \{i,j\}\in\mathcal{E}$, the line resistance is zero.
\item Constant voltage profile: $\forall i \in \mathcal{N}$, the bus voltage magnitude $v_i$ is constant. 
\item Decoupling: Reactive power flows do not affect bus voltage angles.
\item $\forall \{i,j\} \in\mathcal{E}$, the equilibrium bus voltage angle difference is within $\pm \pi/2$, i.e., $\forall \{i,j\} \in\mathcal{E}$, $|\theta_i^\ast-\theta_j^\ast|\in [0,\pi/2)$.
\end{itemize}
These assumptions are standard assumption made in the literature and are used in most works that study for frequency control in transmission networks (for more information, see~\cite{Zhao:2014bp, mallada2017optimal}).
\end{rem}

\subsection{Frequency Control}\label{ssec:goal}
The basic goal of frequency control is to keep the frequency of the power system close to its nominal value. We now illustrate this in more detail by following the same line of argument as in~\cite{Zhao2015acc, DORFLER2017Auto, weitenberg2018exponential, weitenberg2018robust}. 

Since the frequency dynamics depend only on the phase angle differences, for easy of analysis, we express the dynamics in center-of-inertia coordinates~\cite{weitenberg2018exponential, weitenberg2018robust} by making the following change of variables:
$$\delta_i:=\theta_i-\dfrac{1}{n}\sum_{j=1}^{n} \theta_j\,,\qquad\forall i\in\mathcal{N}\,.$$
Then, the dynamics in \eqref{eq:sys-dyn-theta} can be rewritten and stacked into a vector form as:
\begin{subequations}\label{eq:sys-dyn-vec}
\begin{align}
    \dot{\boldsymbol{\delta}} =&\ 2 \pi f_0\left(I_n-\frac{1}{n}\mathbbold{1}_n\mathbbold{1}_n^T\right) \boldsymbol{\omega}\,,\\
    \boldsymbol{M} \dot{\boldsymbol{\omega}}_\mathcal{G} =& -
    \boldsymbol{A}_\mathcal{G} \boldsymbol{\omega}_\mathcal{G}- \nabla_\mathcal{G} U (\boldsymbol{\delta}) + \boldsymbol{p}_\mathcal{G} + \boldsymbol{u}_\mathcal{G}\,,\\
    \mathbbold{0}_{|\mathcal{L}|} =& -
    \boldsymbol{A}_\mathcal{L} \boldsymbol{\omega}_\mathcal{L}- \nabla_\mathcal{L} U (\boldsymbol{\delta}) + \boldsymbol{p}_\mathcal{L} + \boldsymbol{u}_\mathcal{L}\,,\end{align}
\end{subequations}
with $$U(\boldsymbol{\delta}):=- \dfrac{1}{2}\sum_{i=1}^n \sum_{j=1}^n v_i v_j B_{ij}\cos{\left(\delta_i-\delta_j\right)}\,,$$
where $\boldsymbol{\delta}:=\left(\delta_i, i \in \mathcal{N} \right) \in \real^n$, $\boldsymbol{\omega}:=\left(\omega_i, i \in \mathcal{N} \right) \in \real^n$, $\boldsymbol{p}:=\left(p_i, i \in \mathcal{N} \right) \in \real^n$, $\boldsymbol{u} := \left(u_{i},i \in \mathcal{N} \right) \in \real^n$, $\boldsymbol{M} := \diag{m_i, i \in \mathcal{N}} \in \real^{n \times n}$, $\boldsymbol{A}_\mathcal{G} := \diag{\alpha_{i}, i \in \mathcal{G}} \in \real^{|\mathcal{G}| \times |\mathcal{G}|}$, $\boldsymbol{A}_\mathcal{L} := \diag{\alpha_{i}, i \in \mathcal{L}} \in \real^{|\mathcal{L}| \times |\mathcal{L}|}$. Here, a vector with a set as subscript denotes the subvector composed only of the elements from that set, e.g., $\boldsymbol{\omega}_\mathcal{G}:=\left(\omega_i, i \in \mathcal{G} \right) \in \real^{|\mathcal{G}|}$.\footnote{For a finite set $\mathcal{G}$, $|\mathcal{G}|$ denotes the cardinality of $\mathcal{G}$.}

The function $U(\boldsymbol{\delta})$ allows us to compactly summarize the power flow in the system, since the vector of power flows between the buses are given by $\nabla U$. The equilibria of~\eqref{eq:sys-dyn-vec} satisfy
\begin{subequations}\label{eq:sys-dyn-vec-ss}
\begin{align}
    \boldsymbol{\omega}^\ast =&\ \frac{1}{n}\mathbbold{1}_n\mathbbold{1}_n^T \boldsymbol{\omega}^\ast\,,\label{eq:omega-i-eq}\\
    \mathbbold{0}_{|\mathcal{G}|} =& -
    \boldsymbol{A}_\mathcal{G} \boldsymbol{\omega}_\mathcal{G}^\ast- \nabla_\mathcal{G} U (\boldsymbol{\delta}^\ast) + \boldsymbol{p}_\mathcal{G} + \boldsymbol{u}_\mathcal{G}^\ast\,,\label{eq:delta-i-eq-g}\\
    \mathbbold{0}_{|\mathcal{L}|} =& -
    \boldsymbol{A}_\mathcal{L} \boldsymbol{\omega}_\mathcal{L}^\ast- \nabla_\mathcal{L} U (\boldsymbol{\delta}^\ast) + \boldsymbol{p}_\mathcal{L} + \boldsymbol{u}_\mathcal{L}^\ast\,.\label{eq:delta-i-eq-l}\end{align}
\end{subequations}
Clearly, \eqref{eq:omega-i-eq} implies that there exists a scalar $\omega^\ast$ such that $\boldsymbol{\omega}^\ast=\mathbbold{1}_n\omega^\ast$. Then, \eqref{eq:delta-i-eq-g} and \eqref{eq:delta-i-eq-l} can be combined into 
\begin{align}\label{eq:equli-sync-omega}
 \mathbbold{0}_n =& -
    \boldsymbol{A} \mathbbold{1}_n\omega^\ast- \nabla U (\boldsymbol{\delta}^\ast) + \boldsymbol{p} + \boldsymbol{u}^\ast
    \end{align}
with $\boldsymbol{A} := \diag{\alpha_{i}, i \in \mathcal{N}} \in \real^{n \times n}$. Moreover, after premultiplying \eqref{eq:equli-sync-omega} by $\mathbbold{1}_n^T$, we can characterize $\omega^\ast$ as
\begin{align}\label{eq:omega-syn}
\omega^\ast = \dfrac{\sum_{i=1}^n p_i+\sum_{i=1}^n u_i^\ast}{\sum_{i=1}^n \alpha_i}\,,
\end{align}
where we have used the zero net power flow balance  $\mathbbold{1}_n^T\nabla U (\boldsymbol{\delta})=0$ of a lossless power system.

Observe from \eqref{eq:omega-syn} that, in the absence of frequency control, the system undergoing power disturbances $\boldsymbol{p}$ will synchronize to a nonzero frequency deviation, i.e., $\omega^{\ast} \neq 0$, since $\omega^{\ast} = 0$ only if $\sum_{i=1}^n p_i+\sum_{i=1}^n u_i^\ast=0$. Therefore, the main goal of frequency control is to regulate the frequency such that $\omega^{\ast} = 0$ by providing appropriate controllable power injections $\boldsymbol{u}$ to meet power disturbances $\boldsymbol{p}$.
Note that the existence of equilibrium points $(\boldsymbol{\delta}^\ast, \mathbbold{1}_n\omega^\ast)$ such that \eqref{eq:equli-sync-omega} holds for $\omega^{\ast} = 0$ is equivalent to the feasibility of the power flow equation
\begin{align}\label{eq:equli-sync-omega0}
 \nabla U (\boldsymbol{\delta}^\ast) =&  \ \boldsymbol{p} + \boldsymbol{u}^\ast\,,
    \end{align}
that is, there exist some $\boldsymbol{\delta}^*$ solving \eqref{eq:equli-sync-omega0}.  This is a standing assumption of this manuscript. In fact, if  \eqref{eq:equli-sync-omega0} is feasible, then there are many solutions it.  Consequently, we seek to select among the feasible solutions by optimizing certain performance metrics, which we describe next.

\subsection{Performance Assessment}\label{ssec:metric}
For the design of frequency control strategies, not only frequency performance but also economic factors must be taken into account. 
%Therefore, both of them should be considered when designing a control law for $\boldsymbol{u}$. 
Moreover, the secure and efficient operation of power systems relies on properly controlled frequency and cost in both slow and fast timescales. Thus, we now introduce the frequency and economic performance metrics used in this manuscript based on different timescales. 

\subsubsection{Steady-State Performance Metrics} Our control objective in the long run is to achieve the nominal frequency restoration, i.e., $\boldsymbol{\omega}^\ast=\mathbbold{0}_n$, as well as the lowest steady-state aggregate operational cost $C(\boldsymbol{u}^\ast):=\sum_{i=1}^n C_i(u_i^{\ast})$, where the cost function $C_i(u_i)$ quantifies either the generation cost on a generator bus or the user disutility on a load bus for contributing $u_i$. This results in the following constrained optimization problem called \emph{optimal steady-state economic dispatch problem}:
\begin{subequations}\label{eq:opt-ss}
	\begin{eqnarray}
		\label{eq:edp2.a}
		\min_{\boldsymbol{u}^\ast} &&      C(\boldsymbol{u}^\ast):=\sum_{i=1}^n C_i(u_i^{\ast})    \\
		\label{eq:edp2.b}
		\mathrm{s.t.} &&  
		\sum_{i=1}^n p_i+\sum_{i=1}^n u_i^\ast=0 \,,
	\end{eqnarray}	\label{eq:edp2}%
\end{subequations}
where \eqref{eq:edp2.b} is a necessary constraint on the steady-state controllable power injections $\boldsymbol{u}^\ast$ in order to achieve $\boldsymbol{\omega}^\ast=\mathbbold{0}_n$ as discussed in Section~\ref{ssec:goal}. We adopt the standard assumption that  the cost function $C_i(u_i)$ is strictly convex and continuously differentiable~\cite{DORFLER2017Auto, you2021tac}. Then, the optimization problem \eqref{eq:opt-ss} has a convex objective function and an affine equality constraint. Thus, by the Karush-Kuhn-Tucker conditions~\cite[Chapter 5.5.3]{Boyd2004convex}, $\boldsymbol{u}^\ast$ is the unique minimizer of \eqref{eq:opt-ss} if and only if it ensures \emph{identical marginal costs}~\cite{Zhao2015acc, Johannes2016ecc, DORFLER2017Auto, SCHIFFER2017auto, weitenberg2018robust}, i.e., 
\begin{align}\label{eq:id-marginal}
\nabla C_i (u_i^\ast) = \nabla C_j (u_j^\ast)\,,\qquad\forall i,j\in\mathcal{N}\,.
\end{align}


%where the instantenous cost function $C_i(u_i)$ quantifies either the generation cost on a generator bus or the user disutility on a load bus for its participation in frequency control.

%where the widely used assumption that the instantaneous cost function $C_i(u_i)$ is strictly convex and continuously differentiable~\cite{DORFLER2017Auto, you2021tac} with respect to $u_i$ is adopted.

\subsubsection{Transient Performance Metrics} Following sudden major power disturbances, the transient frequency dip can be large in the first few seconds, especially in low-inertia power systems. This may trigger undesired protection measures and even cause cascading failures. Thus, besides the steady-state performance, one should also pay attention to the transient frequency performance with moderate economic cost. With this aim, we define the following transient performance metrics evaluated along the trajectories of the system \eqref{eq:sys-dyn-theta}:
\begin{itemize}
\item \emph{Frequency Nadir} is the maximum frequency deviation from the nominal frequency on each bus during the transient response, i.e., 
\begin{equation}\label{eq:Nadir}
	\|\omega_i\|_\infty := \max_{t\geq0} |\omega_i(t)|\,.
\end{equation}
\item \emph{Economic cost} measures the average cost during time horizon $T$, i.e.
%either the generation cost on a generator bus or the user disutility on a load bus for its participation in frequency control during a time horizon $T$, i.e.,
\begin{equation*}
\bar{C}_{i,T} :=  \dfrac{1}{T}\int_{0}^T C_i(u_i(t)) \mathrm{d}t\,. \end{equation*}
\end{itemize}
Then the \emph{optimal transient frequency control problem} becomes:
\begin{subequations}\label{eq:opt-ts}
	\begin{eqnarray}
		\label{eq:opt-ts-obj}
		\min_{\boldsymbol{u}} &&      \sum_{i \in \mathcal{G}} \|\omega_i\|_\infty +\rho\sum_{i=1}^n\bar{C}_{i,T}   \\
		\label{eq:opt-ts-con}
		\mathrm{s.t.} &&  
		\boldsymbol{u}\ \mathrm{stabilize}\ \eqref{eq:sys-dyn-theta}\,,
	\end{eqnarray}
\end{subequations}
%
%\marginJC{A bit odd to write "(1) and u stabilizes (1)". Maybe just "u stabilizes (1)"?}
%
where $\rho>0$ is the coefficient for tradeoff between the frequency performance and the economic cost. Note that we impose the stability requirement on $\boldsymbol{u}$ as a hard constraint in the optimization problem \eqref{eq:opt-ts}, which will play a pivotal role in its design.

\subsection{Reinforcement Learning for Frequency Control}
Our goal is to design an optimal stabilizing controller that brings the system \eqref{eq:sys-dyn-theta} to an equilibrium that restores the nominal frequency, i.e., $\boldsymbol{\omega}^\ast=\mathbbold{0}_n$, and solves the optimal steady-state economic dispatch problem  \eqref{eq:opt-ss}, while solving the optimal transient frequency control problem \eqref{eq:opt-ts} at the same time. A good starting point to achieve our steady-state control goal is the well-known DAI control. However, it is not straightforward how to also optimize the transient performance. This is hard to be done purely by conventional optimization methods since power systems are nonlinear and power disturbances are unknown. Therefore, we would like to integrate RL into DAI to jointly optimize steady-state and transient performance. 
%
%\marginJC{I think there is a lot of stuff in this paragraph that requires context. For instance, we talk about the "well-known DAI", but we have not introduced it yet. I think we can move most of this discussion to the literature review of the intro, and instead here focus on stating our problem statement/approach to it with the mathematical elements known to the reader now, which are what we have introduced in Sections I.A-C.}
%
% Existing works on secondary frequency control typically focus on either optimizing the steady-state performance by a principled design of fixed updating rules for control dynamics~\cite{Zhao2015acc, DORFLER2017Auto, SCHIFFER2017auto, weitenberg2018exponential} or optimizing the transient performance by a pure learning of good control policies without provable steady-state performance. 
% Therefore, we would like to unify these two perspectives by integrating reinforcement learning (RL) into the well-known distributed averaging-based integral (DAI) control. Basically, RL is employed to seek optimal control policies in terms of the transient performance as a map from the integral variables of DAI to the controllable power injections $\boldsymbol{u}$, while DAI inherently ensures the optimal steady-state performance. Moreover, the closed-loop system stability is provably guaranteed by the special parameterization of $\boldsymbol{u}$.

==> Secondary Control_Arxiv/name.tex <==

To constrain the search space of the set of stabilizing controllers, we derive the structural properties of neural network controllers \textcolor{blue}{from the perspective of Lyapunov stability. More precisely, by finding an appropriate Lyapunov function,} we show that, if \textcolor{blue}{the output of each controller is monotonically} increasing with respect to the local frequency deviation, then the system has a unique equilibrium that is locally exponentially stable. \textcolor{blue}{In addition, we impose this monotonicity as a hard constraint on the neural networks via properly designed weights and biases, which results in piecewise linear controllers to be trained.}  
% The Lyapunov approach allows us to analytically ascertain the stability of the equilibrium for a compact set of points in the state space. The next theorems are the main results of the paper. 


\subsection{Uniqueness of the Equilibrium}
Notably, the \textcolor{blue}{frequency} dynamics of the system in~\eqref{subeq:Dynamic_w} depends only on the voltage phase angle differences, \textcolor{blue}{which means that the same phase shift on each bus will not affect the frequency dynamics. Therefore, for ease of analysis, we make the following change of coordinates to the system in~\eqref{eq:Dynamic}: $$\delta_i:=\theta_i-\dfrac{1}{n}\sum_{i=1}^{n} \theta_i\,,$$
where $\boldsymbol{\delta}:=\left(\delta_i, i \in \mathcal{V} \right) \in \real^n$ can be understood as the center-of-inertia coordinates~\cite{weitenberg2018robust}. Then, the system dynamics in~\eqref{eq:Dynamic} can be written as}
\begin{subequations}\label{eq:equlibrium_change_cor}
    \begin{align}
\dot{\delta_i} &=\omega_i-\frac{1}{n}\sum_{i=1}^n\omega_i\,, \\
 M_{i}\dot{\omega}_{i} &=P_{m,i}- D_i \omega_i-u_i({\omega}_i)-\sum_{j=1}^{n}B_{i j}\sin(\delta_i-\delta_j)\,,
    \end{align}
\end{subequations}
whose equilibrium points can be characterized by the lemma below.

\begin{lem}[Synchronous solution]\label{lemma:exis-sync} If there exists any equilibrium point $(\boldsymbol{\delta}^\ast, \boldsymbol{\omega}^\ast)$ of~\eqref{eq:equlibrium_change_cor}, then it must satisfy 
\begin{subequations}\label{eq:equli-sync}
    \begin{align}
\omega_i^\ast &=\omega^\ast\,, \label{eq:equli-sync-omega}\\
 0 &=P_{m,i}- D_i \omega^\ast-u_i(\omega^\ast)-\sum_{j=1}^{n}B_{i j}\sin(\delta_i^\ast-\delta_j^\ast)\,,\label{eq:equli-sync-delta}
    \end{align}
\end{subequations}
where the synchronous frequency $\omega^\ast$ is determined by
\begin{align}\label{eq:sync-fre}
    \sum_{i=1}^n u_i(\omega^\ast)+\omega^\ast\sum_{i=1}^n D_i=\sum_{i=1}^n P_{m,i}\,.
\end{align}
\end{lem}
\begin{proof} 
In steady state, \eqref{eq:equlibrium_change_cor} yields
\begin{subequations}\label{eq:equli}
    \begin{align}
\omega_i^\ast &=\frac{1}{n}\sum_{i=1}^n\omega_i^\ast\,, \label{eq:omega-i-eq}\\
 0 &=P_{m,i}- D_i \omega_i^\ast-u_i(\omega_i^\ast)-\sum_{j=1}^{n}B_{i j}\sin(\delta_i^\ast-\delta_j^\ast)\,.\label{eq:delta-i-eq}
    \end{align}
\end{subequations}
Clearly, \eqref{eq:omega-i-eq} implies that there exists some $\omega^\ast$ such that \eqref{eq:equli-sync-omega} holds. Then, \eqref{eq:delta-i-eq} becomes \eqref{eq:equli-sync-delta}. Moreover, we can characterize $\omega^\ast$ as in \eqref{eq:sync-fre} by summing \eqref{eq:equli-sync-delta} over $i$, where the zero net power flow balance, i.e., $\sum_{i=1}^{n}\sum_{j=1}^{n}B_{i j}\sin(\delta_i^\ast-\delta_j^\ast)=0$, is used. 
\end{proof}

Lemma~\ref{lemma:exis-sync} characterizes any possible equilibrium point of~\eqref{eq:equlibrium_change_cor} as a synchronous solution, where the system frequency deviation synchronizes to $\boldsymbol{\omega}^\ast=\bm{1}\omega^\ast$ such that the total power imbalance can be met by the total frequency response as in \eqref{eq:sync-fre}. Note that the existence of equilibrium points is equivalent to the feasibility of the power flow in \eqref{eq:equli-sync-delta}, which is a standing assumption of this manuscript. Additionally, provided that phase angle differences between neighboring buses are usually small for power systems in steady state, we make another standard assumption throughout this manuscript that     $|\delta_i^\ast-\delta_j^\ast|\in [0,\pi/2), \forall \{i,j\}\in \mathcal{E}$~\cite{weitenberg2018robust, weitenberg2018exponential}.

In general, it is not easy to know which equilibrium point the system will settle into under an arbitrary control law $u_i(\omega_i)$. However, we can show that, if $u_i(\omega_i)$ is monotonically increasing with respect to $\omega_i$, then the equilibrium point is unique, which is the main idea of the next lemma.
\begin{lem}[Unique equilibrium] If the control output $u_i(\omega_i)$ is a monotonically increasing function of the local frequency deviation $\omega_i$, then the equilibrium point described by \eqref{eq:equli-sync} is unique.
\end{lem}
\begin{proof} We begin by showing the uniqueness of $\omega^\ast$. By way of contradiction, suppose that both $\omega^\ast$ and $\omega^\star$ satisfy \eqref{eq:sync-fre}, where $\omega^\ast\neq\omega^\star$. Then, $$\sum_{i=1}^n u_i(\omega^\ast)+\omega^\ast\sum_{i=1}^n D_i=\sum_{i=1}^n u_i(\omega^\star)+\omega^\star\sum_{i=1}^n D_i\,,$$
which yields
\begin{equation}\label{eq:uni-omega-pro}
\sum_{i=1}^n \dfrac{u_i(\omega^\ast)-u_i(\omega^\star)}{\omega^\ast-\omega^\star}=-\sum_{i=1}^n D_i<0\,.    
\end{equation}
However, if $u_i(\omega_i)$ is monotonically increasing, then the left hand side of the equality in \eqref{eq:uni-omega-pro} must be nonnegative, which is a contradiction. Thus, $\omega^\ast$ is unique. Then, the uniqueness of $\boldsymbol{\delta}^\ast$ follows from the same argument as in~\cite[Lemma~1]{weitenberg2018exponential}.
\end{proof}


%  suppose

% Assume that the system \eqref{eq:Dynamic} admits a synchronous solution that for all $i=1,\cdots,N$, we have $(\bm{\theta}^*, \bm{\omega}^*) := (\bm{\theta}_{0}^*+t\omega^*\mathbf{1}_n, \omega^\ast\mathbf{1})$ with $\mathbf{1} \in \mathbb{R}^N $ being the vector of all ones.  



%That means that there is not a fixed equilibrium for system~\eqref{eq:Dynamic} and thus the stability of the system is not well defined. In this subsection, we first show that there exists a unique synchronous frequency given the monotonicity property of the controller in Lemma~\ref{lemma:exis-sync}, and then define a unique equilibrium  in Lemma~\ref{lemma:unique_equlibrium} after a change of coordinate.  



% \begin{lem}[Synchronous solution]\label{lemma:exis-sync} If the control function $u_i(\omega_i)$ are monotonically increasing with respect to $\omega_i$ for all $i=1,\cdots,N$, there exists a unique synchronous frequency $\omega^*$ given by $\sum_{i=1}^Nu_i(\omega^*)+\omega^*\sum_{i=1}^ND_i=\sum_{i=1}^NP_{m,i}$ suppose the feasibility of power flow at $\omega^*$. The angle in~\eqref{eq:Dynamic} admits a synchronous solution that for all $i=1,\cdots,N$, $\theta_i^*=\theta_{i,0}^*+t\omega^*$ defined by

%  suppose

% Assume that the system \eqref{eq:Dynamic} admits a synchronous solution that for all $i=1,\cdots,N$, we have $(\bm{\theta}^*, \bm{\omega}^*) := (\bm{\theta}_{0}^*+t\omega^*\mathbf{1}_n, \omega^\ast\mathbf{1})$ with $\mathbf{1} \in \mathbb{R}^N $ being the vector of all ones.  
%  \begin{subequations}\label{eq:equlibrium}
%     \begin{align}
%     \dot{\theta}_i^*=& \omega^*,\label{subeq:equ_delta}\\
%     0=& P_{m,i}-
%     D_i \omega^* - u_i(\omega^*)- \sum_{j=1}^N  B_{ij}\sin{\left(\theta_{i,0}^*-\theta_{j,0}^*\right)} \label{subeq:equ_omega}
%     \end{align}
% \end{subequations}
% \end{lem}
% \begin{proof}
% At the synchronous frequency, $\omega_i=\omega^*$ for all $i=1,\cdots,N$ and thus the system dynamics~\eqref{eq:Dynamic} shrink to~\eqref{subeq:equ_omega},   where~\eqref{subeq:equ_omega} assumes the feasibility of the power flow at $\omega^*$. Note that $B_{ij}=B_{ji}$ for all $i,j=1,\cdots,N$, we have $\sum_{i=1}^N \sum_{j=1}^N  B_{ij}\sin{\left(\theta_{i,0}^*-\theta_{j,0}^*\right)}=0$. Summing over~\eqref{subeq:equ_omega} for all $i=1,\cdots,N$ gives the synchronous frequency $\sum_{i=1}^Nu_i(\omega^*)+\omega^*\sum_{i=1}^ND_i=\sum_{i=1}^NP_{m,i}$. Moreover, since $\sum_{i=1}^ND_i>0$, we have $\sum_{i=1}^Nu_i(\omega)+\omega\sum_{i=1}^ND_i$ monotonically increases with respect to $\omega$. Therefore, $\omega^*$ is a unique synchronous frequency. The solution of power flow equation~\eqref{subeq:equ_omega} at $\omega^*$ gives the set of $\theta_{i,0}^*$.
% \end{proof}


% Since angle $\theta^*$ rotates with the same synchronous frequency $\omega^*$, the angle difference is fixed. This subsequently leads to a fixed equilibrium point if introducing a change of coordinates for the phase angle~\cite{weitenberg2018robust}. Let $\delta_i=\theta_i-\sum_{i=1}^{n} \theta_i$ be angle in the center-of-inertia coordinates. In these coordinates, the system (1) becomes


%  \begin{subequations}\label{eq:equlibrium_change_cor}
%     \begin{align}
% \dot{\delta_i} &=\omega_i-\frac{1}{n}\sum_{i=1}^n\omega_i \\
%  M_{i}\dot{\omega}_{i} &=P_{m,i}- D_i \omega_i-u_i({\omega}_i)-\sum_{j=1}^{N}B_{i j}\sin(\delta_i-\delta_j)
%     \end{align}
% \end{subequations}
%The next lemma shows that the dynamics after the change of coordinates have an unique equilibrium.


% \begin{assumption}[Security constraint]~\cite[Assumption~2]{weitenberg2018robust } \label{assumption:angle_difference}
% The angle difference is such that $\delta_i-\delta_j \in \left[-\frac{\pi}{2}+\rho, \frac{\pi}{2}-\rho\right]$ for a sufficiently small positive constant scalar. The space of $\delta$ is denoted by $\Theta :=\left \{\delta| \delta_i-\delta_j \in \left[-\frac{\pi}{2}+\rho, \frac{\pi}{2}-\rho\right] \right \}$.
% \end{assumption}

% Remark 1: Inspired by~\cite{weitenberg2018robust}, we adopt a positive constant $\rho$ as  an extra margin  on the constraint to quantify the decay of the Lyapunov function we will use to derive a  stabilizing controller.


% \begin{lemma}[Unique Equilibrium]~\cite[Lemma~1]{weitenberg2018exponential }\label{lemma:unique_equlibrium}
% Given the uniqueness of synchronous frequency $\omega^*$ in Lemma~\ref{lemma:exis-sync}, if $|\delta_i-\delta_j|\in [0,\pi/2)$ for all $ (i,j)\in \mathcal{E}$, the system~\eqref{eq:equlibrium_change_cor} has an unique equilibrium  $\{(\delta^*,\omega^*)|\sum_{i=1}^Nu_i(\omega^*)+\omega^*\sum_{i=1}^ND_i-\sum_{i=1}^NP_{m,i}=0, \quad P_{m,i}-
%     D_i \omega^* - u_i(\omega^*)- \sum_{j=1}^n  B_{ij}\sin{\left(\delta_{i}^*-\delta_{j}^*\right)} , i =1, \dots, N\}$. 
% If the control function $u_i(\omega_i)$ are monotonically increasing with respect to $\omega_i$ for all $i=1,\cdots,N$, then there exists a unique synchronous frequency $\omega^*$ given by $\sum_{i=1}^Nu_i(\omega^*)+\omega^*\sum_{i=1}^ND_i=\sum_{i=1}^NP_{m,i}$. there exists unique $\delta^*$ such that $P_{m,i}-
%     D_i \omega^* - u_i(\omega^*)- \sum_{j=1}^n  B_{ij}\sin{\left(\delta_{i}^*-\delta_{j}^*\right)}$ for all $ i =1, \dots, N$.
%\end{lemma}
%\begin{proof}
 
 
 
% Under the unique synchronous frequency $\omega^*$, the angle $\delta^*$ in synchronous solution needs to satisfy $
% \sum_{j=1}^n  B_{ij}\sin{\left(\delta_{i}^*-\delta_{j}^*\right)} = P_{m,i}-
%     D_i \omega^* - u_i(\omega^*) $
% The system~\eqref{eq:equlibrium_change_cor} and~\eqref{eq:Dynamic} share the same unique synchronous  frequency $\omega^*$ by following the same line of proof in Lemma~\ref{lemma:exis-sync}. According to~\cite[Lemma~1]{weitenberg2018exponential }, if $|\delta_i-\delta_j|\in [0,\pi/2)$ for all $ (i,j)\in \mathcal{E}$ there exist a unique set of $\delta^*$ such that $
% \sum_{j=1}^n  B_{ij}\sin{\left(\delta_{i}^*-\delta_{j}^*\right)} = P_{m,i}-
%     D_i \omega^* - u_i(\omega^*) $ for all $ i =1, \dots, N$. 
% \end{proof}



%Lyapunov's method asertain the stability of the equilibrium point of a nonlinear dynamic system without numerical integraion, which forms a powerful tool to investigate the general structure property of the controllers that guarantee the transient stability of the system \cite{sauer2017power} .



\subsection{Lyapunov Stability Analysis}
Having characterized the equilibrium point of \eqref{eq:equlibrium_change_cor}, we are now ready to investigate the system stability by first finding an effective Lyapunov function $V(\boldsymbol{\delta}, \boldsymbol{\omega})$ such that $V(\boldsymbol{\delta}^\ast, \boldsymbol{\omega}^\ast)=0$ and $V(\boldsymbol{\delta}, \boldsymbol{\omega})>0, \forall(\boldsymbol{\delta}, \boldsymbol{\omega})\in \mathcal{D}\setminus{(\boldsymbol{\delta}^\ast, \boldsymbol{\omega}^\ast)}$ with the domain $\mathcal{D}:=\! \Set*{(\boldsymbol{\delta}, \boldsymbol{\omega})\in \real^n \times \real^n}{|\delta_i-\delta_j|\in [0,\pi/2), \forall \{i,j\}\in \mathcal{E}}$. Inspired by~\cite{weitenberg2018robust}, we consider the following Lyapunov function candidate:
\begin{align}\label{eq: Lyapunov}
V(\boldsymbol{\delta}, \boldsymbol{\omega})=&\ \frac{1}{2}\sum_{i=1}^{n} M_i(\omega_{i}-\omega^\ast)^{2}+W_\mathrm{p}(\boldsymbol{\delta})+\epsilon W_\mathrm{c}(\boldsymbol{\delta}, \boldsymbol{\omega})
\end{align}
with
\begin{subequations}
\begin{align}
    W_\mathrm{p}(\boldsymbol{\delta}) := 
&-\frac{1}{2}\sum_{i=1}^{n} \sum_{j=1}^{n} B_{ij}\left( \cos(\delta_{ij}) -\cos(\delta_{ij}^*)\right)\nonumber\\
&-\sum_{i=1}^{n}\sum_{j=1}^{n} B_{ij} \sin(\delta_{ij}^*)( \delta_{i}-\delta_{i}^*)\,,\label{eq:Wp}\\
W_\mathrm{c}(\boldsymbol{\delta}, \boldsymbol{\omega}):=&\sum_{i=1}^{n} \sum_{j=1}^{n}B_{ij}\left(  \sin(\delta_{ij})-\sin(\delta_{ij}^*)\right)M_i(\omega_i-\omega^\ast)\,,\nonumber
\end{align}
\end{subequations}
where $\epsilon>0$ is a tunable parameter that should be set small enough. Here, the first term is the kinetic energy of the turbines, the second term is the potential energy of the system stored in the inductive transmission
lines of the power network, and the last cross term between kinetic and potential energies is included for the purpose of proving the exponential stability, which should be clear later. Strictly speaking, this function is not a ``true'' Lyapunov function since it is not nonnegative in the entire state space, i.e., $\forall (\boldsymbol{\delta}, \boldsymbol{\omega})\in \real^n \times \real^n$. That is, it is not bounded from below. Thus, we use it only to show that trajectories starting not too far away from the equilibrium point would converge to it. To see that $V(\boldsymbol{\delta}, \boldsymbol{\omega})$ is a well-defined Lyapunov function on $\mathcal{D}$, it suffices to show the lemma below.  

\begin{lem}[Bounds on Lyapunov function]\label{lemma:Pos_Lyapunov}
$\forall (\boldsymbol{\delta}, \boldsymbol{\omega})\!\in\! \mathcal{D}$, the Lyapunov function $V(\boldsymbol{\delta}, \boldsymbol{\omega})$ in~\eqref{eq: Lyapunov} satisfies
$$
\alpha_{1}(\|\delta-\delta^*\|_2^{2}+\|\omega-\omega^*\|_2^{2}) \leq V(\boldsymbol{\delta}, \boldsymbol{\omega}) \leq \alpha_{2}(\|\delta-\delta^*\|_2^{2}+\|\omega-\omega^*\|_2^{2})
$$
for some constants $\alpha_{1}>0$ and $\alpha_{2}>0$.
\end{lem}
\begin{proof}
The proof is similar to the one of~\cite[Lemma~14]{weitenberg2018robust}, which bounds $V(\boldsymbol{\delta}, \boldsymbol{\omega})$ term by term. Firstly, the kinetic energy term is easily bounded by Rayleigh-Ritz theorem~\cite{Horn2012MA} as
\begin{align}\label{eq:bound-Wk}
     \frac{1}{2}\lambda_\mathrm{min}(\boldsymbol{M})||\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast||^2_2\leq \frac{1}{2}\sum_{i=1}^{n}M_i(\omega_{i}-\omega^\ast)^{2}\leq\frac{1}{2}\lambda_\mathrm{max}(\boldsymbol{M})||\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast||^2_2\,.
\end{align}
Then, with a direct application of~\cite[Lemma~4]{weitenberg2018exponential}, the potential energy term $W_\mathrm{p}(\boldsymbol{\delta})$ in \eqref{eq:Wp} can be bounded by 
\begin{align}\label{eq:bound-Wp}
\beta_{1}\left\|\boldsymbol{\delta}-\boldsymbol{\delta}^{\ast}\right\|_2^2 \leq W_\mathrm{p}(\boldsymbol{\delta}) \leq \beta_{2}\left\|\boldsymbol{\delta}-\boldsymbol{\delta}^{\ast}\right\|_2^2    
\end{align}
for some constants $\beta_{1}>0$ and $\beta_{2}>0$. To deal with the cross term $W_\mathrm{c}(\boldsymbol{\delta})$, we define $p_{\mathrm{e},i}(\boldsymbol{\delta}):=\sum_{j=1}^{n} B_{ij} \sin(\delta_{ij})$. Then, $W_\mathrm{c}(\boldsymbol{\delta}) =\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)^T\!\boldsymbol{M}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)$. Clearly, $-|W_\mathrm{c}(\boldsymbol{\delta})|\leq W_\mathrm{c}(\boldsymbol{\delta})\leq|W_\mathrm{c}(\boldsymbol{\delta})|$. Now, as shown in the proof of~\cite[Lemma~1]{weitenberg2018exponential}, $\forall \boldsymbol{x},\boldsymbol{y}\in\real^{n}$, the inequality $2|\boldsymbol{x}^T\boldsymbol{y}|\leq||\boldsymbol{x}||^2_2+||\boldsymbol{y}||^2_2$
holds. Thus, we have
\begin{align*}
|W_\mathrm{c}(\boldsymbol{\delta})|\leq&\ \dfrac{1}{2}\left(||\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)||^2_2+||\boldsymbol{M}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)||^2_2\right)\nonumber \\
\leq&\ \dfrac{1}{2}\left(\gamma_2||\boldsymbol{\delta}\!-\!\boldsymbol{\delta}^\ast||^2_2+\lambda_\mathrm{max}(\boldsymbol{M})^2||\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast||^2_2\right)\,,
\end{align*}
where the second inequality comes from~\cite[Lemma~4]{weitenberg2018exponential} and Rayleigh-Ritz theorem.
% \begin{align}
%     &\frac{1}{2}\sum_{i=1}^{n} M_i(\omega_{i}-\omega^\ast)^{2} + \epsilon W_\mathrm{c}(\boldsymbol{\delta}, \boldsymbol{\omega})\nonumber\\=&\dfrac{1}{2}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)^T\!\boldsymbol{M}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast) + \epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)^T\!\boldsymbol{M}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)\nonumber\\
%     =&\dfrac{1}{2}\begin{bmatrix}
% \boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})-\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\\ 
% \boldsymbol{\omega}-\boldsymbol{\omega}^\ast
% \end{bmatrix}^T
% \!\!\begin{bmatrix}
% \boldsymbol{0} & \!\!\epsilon\boldsymbol{M}\\ 
% \epsilon\boldsymbol{M} & \!\!\boldsymbol{M}
% \end{bmatrix}\!
% \begin{bmatrix}
% \boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})-\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\\ 
% \boldsymbol{\omega}-\boldsymbol{\omega}^\ast
% \end{bmatrix}\!\,.
% \end{align}
% By~\cite[Lemma~5]{weitenberg2018exponential}, we have
% $$
% \begin{bmatrix}
% -\epsilon\boldsymbol{I} & \boldsymbol{0}\\ 
% \boldsymbol{0}& \boldsymbol{M}-\epsilon\boldsymbol{M}^2 
% \end{bmatrix}
% \preceq 
% \begin{bmatrix}
% \boldsymbol{0} & \!\!\epsilon\boldsymbol{M}\\ 
% \epsilon\boldsymbol{M} & \!\!\boldsymbol{M}
% \end{bmatrix}
% \preceq 
% \begin{bmatrix}
% \epsilon\boldsymbol{I} & \boldsymbol{0}\\ 
% \boldsymbol{0}& \epsilon\boldsymbol{M}^2 +\boldsymbol{I}
% \end{bmatrix}
% $$
Hence, 
\begin{align}\label{eq:bound-Wc}
&-\dfrac{1}{2}\left(\gamma_2||\boldsymbol{\delta}\!-\!\boldsymbol{\delta}^\ast||^2_2+\lambda_\mathrm{max}(\boldsymbol{M})^2||\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast||^2_2\right)\\
&\leq W_\mathrm{c}(\boldsymbol{\delta})\leq \dfrac{1}{2}\left(\gamma_2||\boldsymbol{\delta}\!-\!\boldsymbol{\delta}^\ast||^2_2+\lambda_\mathrm{max}(\boldsymbol{M})^2||\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast||^2_2\right)\,.\nonumber
\end{align}
Finally, combining \eqref{eq:bound-Wk}, \eqref{eq:bound-Wp}, and \eqref{eq:bound-Wc} we can bound the entire Lyapunov function $V(\boldsymbol{\delta}, \boldsymbol{\omega})$ as in \eqref{} with
$$
\begin{aligned}
\alpha_{1} &:=\dfrac{1}{2}\min \left(\lambda_\mathrm{min}(\boldsymbol{M})-\epsilon \lambda_\mathrm{max}(\boldsymbol{M})^2, 2\beta_{1}-\epsilon \gamma_{2}\right)>0\,, \\
\alpha_{2} &:=\dfrac{1}{2}\max \left(\lambda_\mathrm{max}(\boldsymbol{M})+\epsilon \lambda_\mathrm{max}(\boldsymbol{M})^2, 2\beta_2+\epsilon \gamma_{2}\right)>0\,,
\end{aligned}
$$
for sufficiently small $\epsilon>0$.
\end{proof}

It follows directly from Lemma~\ref{lemma:Pos_Lyapunov} that $V(\boldsymbol{\delta}^\ast, \boldsymbol{\omega}^\ast)=0$ and $V(\boldsymbol{\delta}, \boldsymbol{\omega})>0, \forall(\boldsymbol{\delta}, \boldsymbol{\omega})\in \mathcal{D}\setminus{(\boldsymbol{\delta}^\ast, \boldsymbol{\omega}^\ast)}$, which means that the Lyapunov function $V(\boldsymbol{\delta}, \boldsymbol{\omega})$ in~\eqref{eq: Lyapunov} is well-defined. Thus, we can examine the system stability through the time derivative $\dot{V}(\boldsymbol{\delta}, \boldsymbol{\omega})$, whose expression is provided in the next lemma.   

\begin{lem}[Time derivative of Lyapunov function]\label{lemma: dot_V}
The time derivative of the Lyapunov function $V(\boldsymbol{\delta}, \boldsymbol{\omega})$ defined in~\eqref{eq: Lyapunov} is given by 
\begin{align}\label{eq:Vdot}
\dot{V}(\boldsymbol{\delta}, \boldsymbol{\omega}) =&-\!\begin{bmatrix}\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\\\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast\end{bmatrix}^T\!\!\boldsymbol{Q}(\boldsymbol{\delta})\begin{bmatrix}\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\\\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast\end{bmatrix}\\
&-\left[\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast \!\!+\! \epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)\right]^T\left(\boldsymbol{u}(\boldsymbol{\omega})-\boldsymbol{u}(\boldsymbol{\omega}^\ast)\right)\nonumber
\end{align}
with
\begin{equation}
\boldsymbol{Q}(\boldsymbol{\delta}):=
    \begin{bmatrix}
\epsilon\boldsymbol{I}  & \dfrac{\epsilon}{2}\boldsymbol{D} \\  \dfrac{\epsilon}{2}\boldsymbol{D}  & \boldsymbol{D}-\dfrac{\epsilon}{2}(\boldsymbol{H}(\boldsymbol{\delta})\boldsymbol{M}+\boldsymbol{M}\boldsymbol{H}(\boldsymbol{\delta}))
\end{bmatrix}\succ 0\,,
\end{equation}
where $\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}) := \left(p_{\mathrm{e},i}(\boldsymbol{\delta}):=\sum_{j=1}^{n} B_{ij} \sin(\delta_{ij}), i \in \mathcal{V} \right) \in \real^n$ and $\boldsymbol{H}(\boldsymbol{\delta})=\nabla \boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}):=\left[ H_{ij}\right]\in \real^{n \times n}$ such that 
\begin{align}\label{eq:Lij}
    H_{ij}:=
    \begin{dcases}
    -B_{ij}\cos(\delta_{ij}) & \text{if}\ i\neq j\\
    \sum_{j^\prime=1,j^\prime\neq i}^n B_{ij\prime}\cos(\delta_{ij\prime})& \text{if}\ i=j
    \end{dcases}\,,\qquad\forall i,j \in \left[n\right]\,.
\end{align}
% \begin{equation}
% \mathbf{Q}=
%     &\begin{bmatrix}
% \epsilon\mathbf{I}  & \frac{1}{2}\epsilon(\mathbf{D}+\mathbf{K(\omega)}) \\  \frac{1}{2}\epsilon(\mathbf{D}+\mathbf{K(\omega)})  & (\mathbf{D}+\mathbf{K(\omega)})-\frac{\epsilon}{2}(\mathbf{H(\delta)}\mathbf{M}+\mathbf{M}\mathbf{H(\delta)})
% \end{bmatrix} 
% \end{equation}
\end{lem}
\begin{proof}
We start by computing the partial derivatives of $V(\boldsymbol{\delta}, \boldsymbol{\omega})$ with respect to each state, i.e.,
% \begin{subequations}\label{eq: Lyapunov_derivative_partial
% }
% \begin{align}
% \begin{split}
% \frac{\partial V(\delta,\omega) }{\partial \delta_i}&=-P_{e,i}(\delta^*)+ \sum_{j=1}^{N} B_{ij} \sin(\delta_i-\delta_j) \\
% &\quad+\epsilon\sum_{j=1}^NB_{ij}cos(\delta_{ij})\left(M_i(\omega_i-\omega^*)-M_j(\omega_j-\omega^*)\right)
% \end{split}
% \label{subeq: Lyapunov_partial_delta}\\
% \frac{\partial V(\delta,\omega) }{\partial \omega_i}&=M_i\left((\omega_i-\omega^*)+\epsilon\sum_{j=1}^NB_{ij}\left(  \sin(\delta_{ij})-\sin(\delta_{ij}^*)\right)\right)\label{subeq: Lyapunov_partial_w} 
% \end{align}
% \end{subequations}
\begin{subequations}\label{eq: Lyapunov_derivative_partial
}
\begin{align}
\frac{\partial V }{\partial \delta_i}&=p_{\mathrm{e},i}(\boldsymbol{\delta})-p_{\mathrm{e},i}(\boldsymbol{\delta}^\ast) +\epsilon\!\!\sum_{j=1,j\neq i}^nB_{ij}\cos(\delta_{ij})M_i(\omega_i-\omega^\ast)\nonumber\\
&\quad-\epsilon\!\!\sum_{j=1,j\neq i}^n B_{ij}\cos(\delta_{ij})M_j(\omega_j-\omega^\ast)\,,\nonumber
\label{subeq: Lyapunov_partial_delta}\\
\frac{\partial V }{\partial \omega_i}&=M_i\left[\omega_i-\omega^\ast+\epsilon\left(p_{\mathrm{e},i}(\boldsymbol{\delta})-p_{\mathrm{e},i}(\boldsymbol{\delta}^\ast)\right)\right]\,.\nonumber\label{subeq: Lyapunov_partial_w} 
\end{align}
\end{subequations}



% An equilibrium point of the dynamic system is a state $(\delta,\omega)$ where $w_{i}=0$ for $i \in \mathcal{B}$ and $P_{i}= \sum_{j=1}^{N} B_{ij} \sin(\delta_i-\delta_j)$  for $(i, j) \in \mathcal{E},$ i.e., where all frequency deviations are zero and branch power flow equals to the injections. 









% The total derivative of $V$ with respect to $t$ is 
% \begin{equation} \label{eq: Lyapunov_derivative}
%  \begin{aligned} 
% \dot{V}(\delta,\omega) &=\sum_{i=1}^{N}\left(\frac{\partial V(\delta,\omega) }{\partial \delta_i} \dot{\delta_i}+\frac{\partial V(\delta,\omega) }{\partial \omega_i}\dot{\omega_i}\right)
% \\
% &=\sum_{i=1}^{N}\left(P_{e,i}(\delta)-P_{e,i}(\delta^*)\right)\left(\omega_i-\frac{1}{n}\sum_{i=1}^n\omega_i \right)\\ 
% &\quad+\epsilon\left(\sum_{j=1}^NB_{ij}\cos(\delta_{ij})\left(M_i(\omega_i-\omega^*)-M_j(\omega_j-\omega^*)\right)\right)\\
% &\quad\quad\left(\omega_i-\frac{1}{n}\sum_{i=1}^n\omega_i \right)\\
% &\quad+M_i\left((\omega_i-\omega^*)+\epsilon(P_{e,i}(\delta)-P_{e,i}(\delta^*))\right)\left(P_{m,i}- D_i \omega_i-u_i({\omega}_i)-P_{e,i}(\delta)\right)
% \\
% &=-\sum_{i=1}^{N}  (\omega_i-\omega^*) (u_i(\omega_i)-u_i(\omega^*))\\
% &\quad\quadd -\sum_{i=1}^{N}D_i (\omega_i-\omega^*)^2\\
% &\quad\quadd +\epsilon\sum_{i=1}^{N} \xi_i\left(-D_i(\omega_i-\omega^*)-(u_i(\omega_i)-u_i(\omega^*))-\xi_i\right)
% \end{aligned}
% \end{equation}
Therefore, the time derivative of $V(\boldsymbol{\delta}, \boldsymbol{\omega})$ is 
\begin{equation*} 
 \begin{aligned} 
&\dot{V}(\boldsymbol{\delta}, \boldsymbol{\omega}) \\
=&\sum_{i=1}^{n}\left(\frac{\partial V }{\partial \delta_i} \dot{\delta}_i+\frac{\partial V }{\partial \omega_i}\dot{\omega}_i\right)
\\
% =&\ \!\!\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)+\epsilon\boldsymbol{H}(\boldsymbol{\delta})\boldsymbol{M}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)\right)^T\left(\boldsymbol{\omega}-\bm{1}\frac{\bm{1}^T\boldsymbol{\omega}}{n}\right)\\
% &\ \!\!+\!\left[\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast \!\!+\! \epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)\right]^T\!\!\left(P_m\!-\!\boldsymbol{D}\boldsymbol{\omega}\!-\!\boldsymbol{u}(\boldsymbol{\omega})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\right)\\
=&\ \!\!\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)+\epsilon\boldsymbol{H}(\boldsymbol{\delta})\boldsymbol{M}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)\right)^T\left(\boldsymbol{\omega}-\bm{1}\frac{\bm{1}^T\boldsymbol{\omega}}{n}\right)\\
&\ \!\!+\!\left[\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast \!\!+\! \epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)\right]^T\!\!\left(P_m\!-\!\boldsymbol{D}\boldsymbol{\omega}\!-\!\boldsymbol{u}(\boldsymbol{\omega})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\right)\\
&+\underbrace{\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\!+\!\epsilon\boldsymbol{H}(\boldsymbol{\delta})\boldsymbol{M}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)\right)^T\left(\bm{1}\frac{\bm{1}^T\boldsymbol{\omega}}{n}\!-\!\bm{1}\omega^\ast\right)}_{=0}\\
&\ \!\!-\!\left[\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast \!\!+\! \epsilon\!\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)\right]^T\!\!\underbrace{\left(\!P_m\!\!-\!\!\boldsymbol{D}\boldsymbol{\omega}^\ast\!\!\!-\!\boldsymbol{u}(\boldsymbol{\omega}^\ast)\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\!\right)}_{=\boldsymbol{0}}
\\
=&\ \epsilon\left(\boldsymbol{H}(\boldsymbol{\delta})\boldsymbol{M}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)\right)^T(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)-(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)^T\boldsymbol{D}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)\\
&-\epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)^T\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)\\&-\epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)^T\boldsymbol{D}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)\\
&-\left[\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast \!\!+\! \epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)\right]^T\left(\boldsymbol{u}(\boldsymbol{\omega})-\boldsymbol{u}(\boldsymbol{\omega}^\ast)\right)\,,
\end{aligned}
\end{equation*}
which is exactly \eqref{eq:Vdot}. Note that the extra terms in the second equality are added to construct a quadratic format without affecting the the original value of  $\dot{V}(\boldsymbol{\delta}, \boldsymbol{\omega})$ since $\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})^T\bm{1}=\bm{0}$, $\boldsymbol{H}(\boldsymbol{\delta})^T\bm{1}=\bm{0}$, and $P_m\!-\!\boldsymbol{D}\boldsymbol{\omega}^\ast\!-\!\boldsymbol{u}(\boldsymbol{\omega}^\ast)\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)=0$ by the condition at the equilibrium given in \eqref{eq:equli-sync-delta}. 

It remains to show that $\boldsymbol{Q}(\boldsymbol{\delta})\succ0$, which follows directly from the fact that the Schur complement of the block $\epsilon \boldsymbol{I}$ in $\boldsymbol{Q}(\boldsymbol{\delta})$ is positive definite, i.e., $$\boldsymbol{D}-\dfrac{\epsilon}{2}(\boldsymbol{H}(\boldsymbol{\delta})\boldsymbol{M}+\boldsymbol{M}\boldsymbol{H}(\boldsymbol{\delta}))-\frac{\epsilon}{4} \boldsymbol{D}^2\succ 0$$ for sufficiently small $\epsilon$.
% The matrix $\mathbf{H(\delta)}$ is the derivative of $P_e(\delta)$ with respect to $\delta$ and equals to
% \begin{equation}\label{eq:J_delta_w}
%     \begin{split}
%      &\mathbf{H(\delta)}=\\
%     &\begin{bmatrix}
% \begin{smallmatrix}
% \sum_{j=1,j\neq 1}^N B_{1j}\cos{\delta_{1j}} &\hspace{0.5cm} -B_{12}\cos{\delta_{12}} \hspace{0.6cm}   \cdots\hspace{0.6cm}  -B_{1N}\cos{\delta_{1N}}\\
%   -B_{21}\cos{\delta_{21}}& \sum_{j=1,j\neq 2}^N B_{2j}\cos{\delta_{2j}}\quad  \cdots\quad  -B_{2N}\cos{\delta_{2N}}\\
%   \vdots &\ddots\\
%  - B_{N1}\cos{\delta_{N1}}&\hspace{0.8cm}\cdots \hspace{1cm} \sum_{j=1,j\neq N}^N B_{Nj}\cos{\delta_{Nj}}
% \end{smallmatrix}
% \end{bmatrix} \\
%     \end{split},
% \end{equation}
% \textcolor{red}{
% which is a graph Laplacian matrix and equals to 
% $L \operatorname{diag}\left(\left\{B_{i j} \cos \left(\delta_{ij}\right)\right\}_{\{i, j\} \in \mathcal{E}}\right) L^{T}$ with $L \in \mathbb{R}^{N \times|\mathcal{E}|}$ be the  (oriented) incidence matrix~\cite{dorfler2013synchronization}. Since $\delta \in \Theta$, then $\cos \left(\delta_{ij}\right)>0$ for all $i,j=1,\cdots,N$ and thus $\mathbf{H(\delta)}\succeq 0$. To add it later!} 
\end{proof}

From Lemma~\ref{lemma: dot_V} we can see that $u_i(\omega_i)$ plays a part in the cross term $\left[\boldsymbol{\omega}-\boldsymbol{\omega}^\ast + \epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})-\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)\right]^T\left(\boldsymbol{u}(\boldsymbol{\omega})-\boldsymbol{u}(\boldsymbol{\omega}^\ast)\right)$ of $\dot{V}(\boldsymbol{\delta}, \boldsymbol{\omega})$, which in general complicates the analysis of $\dot{V}(\boldsymbol{\delta}, \boldsymbol{\omega})$. However, it is not hard to observe that this cross term is nonnegative for sufficiently small $\epsilon$ if $u_i(\omega_i)$ is monotonically increasing with respect to $\omega_i$, which further implies that $\dot{V}(\boldsymbol{\delta}, \boldsymbol{\omega})<0$, $\forall(\boldsymbol{\delta}, \boldsymbol{\omega})\in \mathcal{D}\setminus{(\boldsymbol{\delta}^\ast, \boldsymbol{\omega}^\ast)}$. Thus, if $u_i(\omega_i)$ is monotonically increasing with respect to $\omega_i$, the system is locally asymptotically stable at the equilibrium point $(\boldsymbol{\delta}^\ast, \boldsymbol{\omega}^\ast)$. Actually, in this case, we can even show local exponential stability as in the next theorem. 
\begin{thm}[Local exponential stability]\label{theorem:Exponential_stable}
If the control output $u_i(\omega_i)$ is a monotonically increasing function of the local frequency deviation $\omega_i$, then the equilibrium point $(\boldsymbol{\delta}^\ast, \boldsymbol{\omega}^\ast)$ described by \eqref{eq:equli-sync} is locally exponentially stable.
\end{thm}

\begin{proof}
%A local Lyapunov function $\begingroup\color{black} V(\delta,\omega)\endgroup$ for the dynamic system represented by  \eqref{eq:Dynamic} is \cite{weitenberg2018robust, weitenberg2018exponential}
% \cite{arapostathis1982global,dobson1989towards,chang1995direct,vu2015lyapunov}
% \begin{equation}\label{eq: Lyapunov}
% \begin{aligned}
% V(\delta,\omega)=&\frac{1}{2}\sum_{i=1}^{N} M_i(\omega_{i}-\omega^*)^{2}-\sum_{i=1}^{N}\sum_{j=1}^{N} B_{ij} \sin(\delta_{ij}^*)( \delta_{i}-\delta_{i}^*) \\
% &-\frac{1}{2}\sum_{i=1}^{N} \sum_{j=1}^{N} B_{ij}\left( \cos(\delta_{ij}) -\cos(\delta_{ij}^*)\right)
% \\
% &+\epsilon\sum_{i=1}^{N} \sum_{j=1}^{N}B_{ij}\left(  \sin(\delta_{ij})-\sin(\delta_{ij}^*)\right)M_i(\omega_i-\omega^*)
% \end{aligned}\end{equation}
% The term $ \frac{1}{2}\sum_{i=1}^{N} M_i(\omega_{i}-\omega^*)^{2} $
% represents the kinetic energy of the turbines and the term $\sum_{i=1}^{N}\sum_{j=1}^{N} B_{ij} \sin(\delta_{ij}^*)( \delta_{i}-\delta_{i}^*) -\frac{1}{2}\sum_{i=1}^{N} \sum_{j=1}^{N} B_{ij}\left( \cos(\delta_{ij}) -\cos(\delta_{ij}^*)\right)$
% is the potential energy of the system stored in the inductive
% lines in the power grid network.
% This function is not a ``true'' Lyapunov function since it is not non-negative on the entire state space (it is not bounded from below) for all $\delta\in \mathbb{R}^N$, and it is used to show that trajectories that start not too far away from the equilibrium point would converge to it. By Lemma~\ref{lemma:Pos_Lyapunov}, the Lyapunov function $V(\delta, \omega)$ in~\eqref{eq: Lyapunov} 
% satisfies
% \begin{equation}\label{eq:bound_Lyapunov}
% \beta_{1}(\|\delta-\delta^*\|_2^{2}+\|\omega-\omega^*\|_2^{2}) \leq V(\delta, \omega) \leq \beta_{2}(\|\delta-\delta^*\|_2^{2}+\|\omega-\omega^*\|_2^{2})
% \end{equation}
% for some positive constants $\beta_{1}$ and $\beta_{2}$, with $\delta \in \Theta$, provided that $\epsilon$ is sufficiently small. 
% Therefore, the function $V(\delta, \omega)$ 
%is a qualified Lyapunov function for the area $\left \{(\delta,\omega)|\delta \in \Theta, \omega\in \mathbb{R}^N  \right \}$. 
The key is to show that, if $u_i(\omega_i)$ is monotonically increasing with respect to $\omega_i$, then there exists a constant $c>0$ such that $\dot{V}(\boldsymbol{\delta}, \boldsymbol{\omega})\leq -cV(\boldsymbol{\delta}, \boldsymbol{\omega})$.

We start by bounding the quadratic term related to $\boldsymbol{Q}(\boldsymbol{\delta})$ in \eqref{eq:Vdot} as follows:
\begin{align}
    &\begin{bmatrix}\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\nonumber\\\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast\end{bmatrix}^T\!\!\boldsymbol{Q}(\boldsymbol{\delta})\begin{bmatrix}\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\nonumber\\\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast\end{bmatrix}\nonumber\\&\geq \lambda_\mathrm{min}(\boldsymbol{Q}(\boldsymbol{\delta}))\left(||\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)||^2_2+||\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast||^2_2\right)
    \nonumber\\&\geq \lambda_\mathrm{min}(\boldsymbol{Q}(\boldsymbol{\delta}))\left(\gamma_1||\boldsymbol{\delta}\!-\!\boldsymbol{\delta}^\ast||^2_2+||\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast||^2_2\right)
    \nonumber\\&\geq \lambda_\mathrm{min}(\boldsymbol{Q}(\boldsymbol{\delta}))\min(1, \gamma_1)\left(||\boldsymbol{\delta}\!-\!\boldsymbol{\delta}^\ast||^2_2+||\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast||^2_2\right)
    \nonumber\\&\geq \lambda_\mathrm{min}(\boldsymbol{Q}(\boldsymbol{\delta}))\min(1, \gamma_1)\dfrac{1}{\alpha_2}V(\boldsymbol{\delta}, \boldsymbol{\omega}) \nonumber
    \\&\geq c V(\boldsymbol{\delta}, \boldsymbol{\omega})\label{eq:bound-Q}
\end{align}
with $$c:=\left(\min_{\boldsymbol{\delta}:|\delta_i-\delta_j|\in [0,\pi/2), \forall \{i,j\}\in \mathcal{E}} \!\lambda_\mathrm{min}(\boldsymbol{Q}(\boldsymbol{\delta}))\right)\dfrac{\min(1, \gamma_1)}{\alpha_2}>0\,,$$
where the first inequality is by Rayleigh-Ritz theorem, the second inequality is by~\cite[Lemma~4]{weitenberg2018exponential}, and the fourth inequality is by Lemma~\ref{lemma:Pos_Lyapunov}.

We now show rigorously that, if $u_i(\omega_i)$ is monotonically increasing with respect to $\omega_i$, then the cross term related to them in \eqref{eq:Vdot} is nonnegative for sufficiently small $\epsilon$. Define
\begin{align*}
    k_{i}(\omega_i):=
    \begin{dcases}
    \dfrac{u_i(\omega_i)-u_i(\omega_i^\ast)}{\omega_i-\omega_i^\ast} & \text{if}\ \omega_i \neq\omega_i^\ast\\
    0& \text{if}\ \omega_i=\omega_i^\ast
    \end{dcases}\,,\quad\forall i \in \left[n\right]\,.
\end{align*}
Then, $\boldsymbol{K}(\boldsymbol{\omega}) := \diag{k_{i}(\omega_i), i \in \mathcal{V}} \in \real^{n \times n}\succeq0$ if $u_i(\omega_i)$ is monotonically increasing with respect to $\omega_i$. Hence, 
\begin{align}\label{eq:bound-cross}
&\left[\boldsymbol{\omega}-\boldsymbol{\omega}^\ast + \epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})-\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)\right]^T\left(\boldsymbol{u}(\boldsymbol{\omega})-\boldsymbol{u}(\boldsymbol{\omega}^\ast)\right)\nonumber\\=&\left(\boldsymbol{\omega}-\boldsymbol{\omega}^\ast\right)^T\boldsymbol{K}(\boldsymbol{\omega})\left(\boldsymbol{\omega}-\boldsymbol{\omega}^\ast\right)\nonumber\\ &+\epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})-\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)^T\boldsymbol{K}(\boldsymbol{\omega})\left(\boldsymbol{\omega}-\boldsymbol{\omega}^\ast\right)\nonumber\\\geq&\ \!0\,,  \end{align}
for small enough $\epsilon$.

Finally, combining \eqref{eq:Vdot}, \eqref{eq:bound-Q}, and \eqref{eq:bound-cross}, we have $\dot{V}(\boldsymbol{\delta}, \boldsymbol{\omega})\leq -c V(\boldsymbol{\delta}, \boldsymbol{\omega})$.
% $\sum_{i=1}^{N}P_{e,i}(\delta)=\sum_{i=1}^{N}P_{e,i}(\delta^*)=0$, and $\sum_{i=1}^{N}\sum_{j=1}^NB_{ij}\cos(\delta_{ij})\left(M_i(\omega_i-\omega^*)-M_j(\omega_j-\omega^*)\right)=0$
% where $\xi_i=\sum_{j=1}^{N}B_{ij}\left(  \sin(\delta_{ij})-\sin(\delta_{ij}^*)\right)$.
% Let $k_i(\omega_i)= \left(u_i(\omega_i)-u_i(\omega_i^*)\right)/\left(\omega_i-\omega_i^*\right)$
% if $\omega_i\neq\omega_i^*$ and $k_i(\omega_i)=0$ if $\omega_i=\omega_i^*$. Denote $\mathbf{K(\omega)}=\text{diag}(k_1(\omega_1),\cdots,k_N(\omega_N))$ and thus $u_(\omega)-u(\omega^*)=\mathbf{K(\omega)}(\omega-\omega^*)$. Let $\mathbf{M}=\text{diag}(M_1,\cdots,M_N)$ and $\mathbf{D}=\text{diag}(D_1,\cdots,D_N)$, $\chi =\text{col}(P_e(\delta)-P_e(\delta^*), \omega-\omega^*)$, Lemma~\ref{lemma: dot_V} shows that
% \begin{equation}
% \dot{V}(\delta,\omega) &=- \chi^\top\left( \mathbf{\hat{Q}}+\mathbf{\Delta Q}\right)\chi
% \end{equation}
% where
% \begin{equation}
% \mathbf{Q}=
%     &\begin{bmatrix}
% \epsilon\mathbf{I}  & \frac{1}{2}\epsilon(\mathbf{D}+\mathbf{K(\omega)}) \\  \frac{1}{2}\epsilon(\mathbf{D}+\mathbf{K(\omega)})  & (\mathbf{D}+\mathbf{K(\omega)})-\frac{\epsilon}{2}(\mathbf{H(\delta)}\mathbf{M}+\mathbf{M}\mathbf{H(\delta)})
% \end{bmatrix} 
% \end{equation}
% \begin{equation*}
% \mathbf{\Delta Q}=
%     &\begin{bmatrix}
% \mathbf{0}  & \frac{1}{2}\epsilon\mathbf{K(\omega)} \\  \frac{1}{2}\epsilon\mathbf{K(\omega)}  & \mathbf{K(\omega)} 
% \end{bmatrix} ,
% \end{equation*}
% \begin{equation}\label{eq:hat_Q}
% \mathbf{\hat{Q}}=
%     &\begin{bmatrix}
% \epsilon\mathbf{I}  & \frac{1}{2}\epsilon\mathbf{D} \\  \frac{1}{2}\epsilon\mathbf{D}  & \mathbf{D}-\frac{\epsilon}{2}(\mathbf{H(\delta)}\mathbf{M}+\mathbf{M}\mathbf{H(\delta)})
% \end{bmatrix} ,
% \end{equation}
% and $\mathbf{H(\delta)}\succeq0$ is a graph Laplacian matrix (details can be found in Lemma~\ref{lemma: dot_V}). By Lemma~\ref{lemma:Bounded_Lyapunov}, there exists a positive constant $c$ such that $\chi^\top \mathbf{\hat{Q}}\chi\leq -c\dot{V}(\delta, \omega)$.
%Hence,  $\chi^\top \mathbf{\hat{Q}}\chi\leq -\beta_4||\chi||^2_2 $ where $\beta_4:=\min_{\delta\in \Theta }\lambda_{min}\left(\mathbf{\hat{Q}}\right).$
% By Lemma~\ref{lemma:bound_potential_func}, there exists a constant $\beta_3^\prime$ such that
% \begin{equation}
%     ||P_e(\delta)-P_e(\delta^*)||^2_2\geq \beta_3^\prime||\delta-\delta^*||_2^2
% \end{equation}
% Then $||\chi||^2_2=||P_e(\delta)-P_e(\delta^*)||^2_2 +||\omega_i-\omega_i^*||^2_2\geq \min(1, \beta_3^\prime)(||\delta-\delta^*||^2_2 +||\omega_i-\omega_i^*||^2_2) $. Hence, $||\chi||^2_2\geq \beta_3(||\delta-\delta^*||^2_2 +||\omega_i-\omega_i^*||^2_2)$ where $\beta_3:= \min(1, \beta_3^\prime).$ 
%Therefore $\chi^\top \mathbf{\hat{Q}}\chi\leq -\beta_4||\chi||^2_2 \leq -\beta_3\beta_4(||\delta-\delta^*||^2_2 +||\omega_i-\omega_i^*||^2_2)\leq -\frac{\beta_3\beta_4}{\beta_2}V(\delta,\omega).$ We finish the proof by taking $c=\frac{\beta_3\beta_4}{\beta_2}$.
% Note that $\mathbf{K(\omega)}$ depends on the learned controller. To elimate such dependence in proof, we define 
%When $u_i(\omega_i)$ are monotonically increasing with respect to $\omega_i$ for all $i=1,\cdots,N$, we have $\mathbf{K(\omega)}\succeq 0$. Hence, $- \chi^\top\mathbf{\Delta Q}\chi=(\omega-\omega^*)^\top\mathbf{K(\omega)}(\omega-\omega^*)+\epsilon (\omega-\omega^*)^\top\mathbf{K(\omega)} \left(P_e(\delta)-P_e(\delta^*)\right)\leq 0$ for sufficiently small $\epsilon$.  Therefore , $\dot{V}(\delta,\omega)\leq\chi^\top \mathbf{\hat{Q}}\chi\leq -c\dot{V}(\delta, \omega)$ and thus the equilibrium is exponential stable.
% The equilibrium is locally asymptotically stable when $\dot{V}(\delta,\omega)\leq 0$ with equality only reached at the equilibrium. If the function $u_i(\omega_i)$ monotonic increases with $\omega_i$, then $u_i(\omega_i)\geq u_i(\omega^*)$ is the same sign with $(\omega_i\geq\omega^*$ for all $i=1,\cdots,N$. 
% Since $\D_i\geq 0$ abd $\sum_{i=1}^ND_i>0$, we have\eqref{eq: Lyapunov_derivative}, $\dot{V}(\delta,\omega)< 0$ for $\omega_i\neq \omega^*$. 
% Note this condition is distributed in the sense that it needs to be satisfied at each of the buses. 
% , in the sense that it is only for each of  In this way, stability requirement of the total system can be satisfied by the constraint on the action of each bus distributively.
% By the Krasovski-Lasalle principle~\cite{aastrom2010feedback}, the constraint on control action can be further relaxed to include equality, i.e.,  $\omega_i u_i(\omega_i) \geq 0$.
% Define the set $S=\left\{(\delta,\omega) \in \Omega_{r}: \dot{V}(\delta,\omega)=0\right\}$ where the derivative of  Lyapunov equals to zero. For a trajectory to remain
% in this set we must have $\omega_i = 0$ or $u_i(\omega_i)=0$. 
% Consider one point where $\omega_i \neq 0$ while $u_i(\omega_i)=0$. Using the dynamics \eqref{subeq:Dynamic_delta} we have $\dot{\delta_i}\neq 0$, this implies that $\dot{\omega_i}\neq 0$ if $u_i(\omega_i)=0$. Therefore, points with $\omega_i \neq 0$ are not in the invariant set inside $S$. In other words, $S$ contains no invariant sets other than the states that $w_i=0$.  Then from the  Krasovski-Lasalle principle, we can conclude that the state $(\delta,\omega)$ where $w_{i}=0$ and $P_{i}= \sum_{j=1}^{N} B_{ij} \sin(\delta_i-\delta_j)$  for $(i, j) \in \mathcal{E},$ is locally asymptotically stable. 
\end{proof}

The qualifier ``local'' in Theorem~\ref{theorem:Exponential_stable} is important since we need to assume that the trajectories start within a bounded region of the equilibrium point. This region has no constraints on $\omega$, and requires $\delta$ constrained in the region denoted by $\Theta :=\left \{\delta| \delta_i-\delta_j \in \left(-\frac{\pi}{2}, \frac{\pi}{2}\right) \right \}$ ~\cite{weitenberg2018robust}, which is sufficiently large to include almost all practical scenarios.
% Note that the small positive constant $\rho$ is utilized as  an extra margin on the constraint to quantify the decay of the Lyapunov function we will use to derive a  stabilizing controller. 
% The region is sufficiently large to include almost all practical scenarios.
% This region is derived based on well understood power system energy (or Lyapunov) functions~\cite{arapostathis1982global,dobson1989towards,chang1995direct,vu2015lyapunov} and can be explicitly characterized. 
% The region is quite large, since it includes all states where $\delta_i$ that satisfy $|\delta_i-\delta_j|\in [0,\pi/2)$ (no constraints on $\omega$), which include almost all practical scenarios.
% ~(see Appendix~\ref{app:region} for more details). 
% The next theorem shows that if controllers have more structure, a desirable rate of convergence can be obtained.
% \begin{theorem}\label{theorem:Exponential_stable}
% If the control function $u_i(\omega_i)$ are monotonically increasing with respect to $\omega_i$ for all $i=1,\cdots,N$, then the equilibrium point is locally exponentially stable.
% \end{theorem}
Theorem~\ref{theorem:Exponential_stable} gives structural properties\footnote{These are sometimes called extended class $\kappa$ functions} for controllers that guarantee exponential stability for \emph{all system parameter and topologies}. Namely, if the controllers satisfy the conditions in the theorems, they would be locally stabilizing for any network. Therefore, the optimal performance comes from training on a particular network, but the stability guarantees do not. This robustness to uncertainties is a key advantage of defining the structure of networks compared to purely model-free RL approaches. 

The design of neural networks that satisfy these properties is given in the next section (Section~\ref{sec:design}). %The proof of 
% Theorem~\ref{theorem:Asymptotic_stable} is given below and the proof of 
%Theorem~\ref{theorem:Exponential_stable} is given below.
% in the Appendix~\ref{appendices:Monotonic_Function}. 

\subsection{Design of Neural Network Controllers} \label{sec:design}
In this paper, we parametrize the controllers $u_i$ by a single hidden layer neural network. 
We assume that the processes such as automatic generation
control (AGC) adjust the power setpoint of generators to make the net power injection around zero, i.e., $\sum_{i=1}^{N}P_{m,i}=0$. For controllers $u(\omega)$ that provide primary frequency response, we let function $u(0)=0$ to make zero action when there is no frequency deviation. 
By Theorem
% s~\ref{theorem:Asymptotic_stable} and
~\ref{theorem:Exponential_stable}, we design the weights and the biases of the neural networks to have the following structures \highlight{such that  the controller will be locally exponentially stabilizing}:
% To incorporate the inequality constraints \eqref{subeq:Discrete_optimization_bound}-\eqref{subeq:Discrete_optimization_Mono} on control action, we aim to design the neural network structure for control function at each bus that satisfy:
\begin{enumerate}
    % \item $u_{\varphi_i}(\omega_i)$ has the same sign as $\omega_i$ 
    \item $u_{\varphi_i}(\omega_i)$ is monotonically increasing
    \item $u_{\varphi_i}(\omega_i)=0$ for $\omega_i=0$
    \item  $\underline{u}_i \leq u_{\varphi_i}(\omega_i)\leq \overline{u}_i$ (saturation constraints) 
\end{enumerate}
%The first two requirement is equivalent to design a monotonic increasing function through the origin. Note the the rectified linear unit (ReLU) function $\sigma(x)$ is linear with $x$ when activated $(x>0)$ and equals to zero when $(x\leq0)$, we construct the monotonic increasing function through the origin by stacking the ReLU function using: 
%\begin{equation}\label{eq:Mono_u}
%    u_i(\omega_i)=Q_i^+\sigma(\mathbf{1}w_i+b_i^+)+Q_i^-\sigma(\mathbf{1}w_i+b_i^-)
%\end{equation}  
%where $Q_i^+$ is the weights vector of bus $i$ and $Q_i^+=[q_i^1,q_i^2,\cdots,q_i^m]^\intercal$; $b_i$ is the bias vector of bus $i$ and $b_i^+=[b_i^1,b_i^2,\cdots,b_i^m]^\intercal$. $\sigma$ stands for the element-wise ReLU operator. $\mathbf{1}\in \mathbb{R}^m$ is the column vector where all the element is one. \\



The first two requirements are equivalent to designing a monotonic increasing function through the origin. This is constructed by decomposing the function into positive and negative parts as $f_i(\omega_i)=f_i^+(\omega_i)+f_i^-(\omega_i)$, where $f_i^+(\omega_i)$ is monotonic increasing for $\omega_i>0$ and zero when $\omega_i\leq0$; $f_i^-(\omega_i)$ is monotonic increasing for $\omega_i<0$ and zero when $\omega_i\geq0$. The saturation constraints can be satisfied by hard thresholding the output of the neural network. 


The function $f_i^+(\omega_i)$ and $f_i^-(\omega_i)$ are constructed using a single-layer neural network designed by stacking the ReLU function. Let $m$ be the number of hidden units. For $f_i^+(\omega_i)$, let  $q_i=[\begin{matrix}
 q_i^{1}& q_i^{2} & \cdots&q_i^{m}
\end{matrix}]$ be the weight vector of bus $i$; $b_i=[\begin{matrix} b_i^{1}& b_i^{2} & \cdots &b_i^{m}\end{matrix}]^\intercal$ be the corresponding bias vector. For $f_i^-(\omega_i)$, let $z_i=[\begin{matrix} z_i^{1}&z_i^{2}&\cdots&z_i^{m}\end{matrix}]$ be the weights vector and $c_i=[\begin{matrix} c_i^{1}& c_i^{2} & \cdots & c_i^{m}\end{matrix}]^\intercal$ be the bias vector. Denote $\mathbf{1}\in \mathbb{R}^m$ as the all $1$'s column vector. The detailed construction of $f_i^+(\omega_i)$ and $f_i^-(\omega_i)$ is given in Lemma~\ref{lemma:u_f+}. 
\begin{lemma}\label{lemma:u_f+}
Let $\sigma(x)=\max(x,0)$ be the ReLU function.  The stacked ReLU function constructed by \eqref{eq:f+} is monotonic increasing for $\omega_i>0$ and zero when $\omega_i\leq 0$.
\begin{subequations}\label{eq:f+}
\begin{align}
     &f_i^+(\omega_i)=q_i\sigma(\mathbf{1}\omega_i+b_i)\\
     \mbox{where }
     &\sum_{j=1}^{l} q_i^{j}\geq 0, \quad \forall l=1,2,\cdots,m
     \label{eq:f+2}\\
     & b_i^{1}=0, b_i^{l}\leq b_i^{(l-1)}, \quad \forall l=2,3,\cdots,m\label{eq:f+3}
\end{align}
\end{subequations}
 The stacked ReLU function constructed by \eqref{eq:f-} is monotonic increasing for $\omega_i< 0$ and zero when $\omega_i\geq 0$.
\begin{subequations}\label{eq:f-}
\begin{align}
     &f_i^-(\omega_i)=z_i\sigma(-\mathbf{1}\omega_i+c_i)\\
     \mbox{where } 
     &\sum_{j=1}^{l} z_i^{j}\leq 0, \quad \forall l=1,2,\cdots,m\label{eq:f-2}\\
     & c_i^{1}=0, c_i^{l}\leq c_i^{(l-1)}, \quad \forall l=2,3,\cdots,m\label{eq:f-3}
\end{align}
\end{subequations}
\end{lemma}


\begin{proof}
 Note that the ReLU function $\sigma(x)$ is linear with $x$ when activated $(x>0)$ and equals to zero when deactivated $(x \leq 0)$, we construct the monotonic increasing function $f_i^+(\omega_i)$ by stacking the function $g_i^l(\omega_i)=q_i^{l}\sigma(\omega_i+b_i^{l})$ as illustrated by Fig.~\ref{fig:Mono_Structure}. Since 
$b_i^{1+}=0$ and $b_i^{l+}\leq b_i^{(l-1)+}, \forall 1\leq l \leq m$, $g_i^l(\omega_i)$  is activated in sequence from $g_i^1(\omega_i)$ to $g_i^m(\omega_i)$ with the increase of $\omega_i$. In this way, the stacked function is a piece-wise linear function and the slope for each piece is $\sum_{j=1}^{l} q_i^j$. 
Monotonic property can be satisfied as long as the slope of all the pieces are positive, i.e., $\sum_{j=1}^{l} q_i^l\geq 0, \forall 1\leq l \leq m$. Similarly, $f_i^-(\omega_i)$ also construct by ReLU function activated for negative $w_i$ in sequence corresponding to $c_i^l$ for $l=1,\cdots,m$. $\sum_{j=1}^{l} z_i^{j}\leq 0$ means that all the slop of the piece-wise linear function is positive and therefore guarantees monotone.
\begin{figure}[t]	
	\centering
	\includegraphics[scale=0.68]{Mono_Structure.png}
	\caption{Stacked ReLU neural network to formulate a monotonic increasing function through the origin}
	\label{fig:Mono_Structure}
\end{figure}
\end{proof}
Note that there still exists inequality constraints in \eqref{eq:f+} and \eqref{eq:f-}, which makes the training of the neural networks cumbersome.  We can reformulate the weights to get a equivalent representation that is easier to deal with in training. Define the non-negative vectors $\hat{q}_i=\left[\begin{matrix} \hat{q}_i^{1}&\cdots&\hat{q}_i^{m}\end{matrix}\right]$ and $\hat{b}_i=\left[\begin{matrix}\hat{b}_i^{1}&\cdots&\hat{b}_i^{m}\end{matrix}\right]^\intercal$. Then, \eqref{eq:f+2} is satisfied if $q_i^{1}=\hat{q}_i^{1}$, $q_i^{l}=\hat{q}_i^{l}-\hat{q}_i^{(l-1)}$ for  $l=2,\cdots,m$. \eqref{eq:f+3} is satisfied if $b_i^{1}=0$, $ b_i^{l}=-\sum_{j=2}^{l} \hat{b}_i^{j}$ for  $l=2,\cdots,m$. 
Similarly, define $\hat{z}_i=\left[\begin{matrix}\hat{z}_i^{1}&\cdots&\hat{z}_i^{m}\end{matrix}\right]\geq 0$  and $\hat{c}_i=\left[\begin{matrix}\hat{c}_i^{1}&\cdots&\hat{c}_i^{m}\end{matrix}\right]^\intercal\geq 0$. Then, \eqref{eq:f-2} is satisfied if $z_i^{1}=-\hat{z}_i^{1}$, $ z_i^{l}=-\hat{z}_i^{l}+\hat{z}_i^{(l-1)}$ for  $l=2,\cdots,m$. \eqref{eq:f-3} is satisfied if $c_i^{1}=0$, $ c_i^{l}=-\sum_{j=2}^{l} \hat{c}_i^{l}$ for  $l=2,\cdots,m$. If the dead-band of the frequency deviation within the range $[-d,d]$ is required, it can be easily satisfied by setting $b_i^2=-d, q_i^1=0$ and  $c_i^2=-d, z_i^1=0$ in \eqref{eq:f+} and \eqref{eq:f-}.\footnote{A deadband is often enforced for generator droop control to reduce mechanical stress. For inverters, we do not do not set mandatory dead-band.}

The next Theorem states the converse of Lemma~\ref{lemma:u_f+}, that is, the constructions in \eqref{eq:f+} and \eqref{eq:f-} suffice to approximate all functions of interest. 
\begin{theorem}\label{theorem:Universial Approximation}
Let $r(x)$ be any continuous, Lipschitz and bounded monotonic function through the origin with bounded derivatives, mapping compact set $\mathbb{X}$ to  $ \mathbb{R}$.  Then there exists a function $f(x)=f^+(x)+f^-(x)$ constructed by \eqref{eq:f+} and \eqref{eq:f-} such that, for any $\epsilon$ and any $x \in \mathbb{X}$, $\left|r(x)-f(x)\right|<\epsilon$. 
\end{theorem}

The proof is given in Appendix~\ref{appendices:stacked-ReLU}. Note that $f(x)$ is a single-layer neural network. When approximating an arbitrary function, the number of neurons and the height will depend on $\epsilon$.
Since the controller in this paper is bounded, the stacked-ReLU neural network with limited number of neurons is sufficient for parameterization. The last step is to bound the output of the neural networks, which can be done easily using ReLU activation functions. 
\begin{lemma}\label{lemma:u_f+-}
 The neural network controller $u_i$ given below is a monotonic increasing function through the origin and bounded in $[\underline{u}_i, \overline{u}_i]$ for all $i=1,\cdots,N$:
\begin{equation}\label{eq:u_f+-}
\begin{split}
    u_i(\omega_i)=&\overline{u}_i-\sigma(\overline{u}_i -f_i^+(\omega_i)-f_i^-(\omega_i))\\
    &+\sigma(\underline{u}_i -f_i^+(\omega_i)-f_i^-(\omega_i))
\end{split}
\end{equation}
\end{lemma}
The proof of this lemma is by inspection. 

% Note that the construction \eqref{eq:u_f+-} is equivalent to the function $f(\omega_i)$ bounded by $\left[\overline{u}_i,\underline{u}_i\right]$. This means that the control network for $u_i(\omega_i)$ can universally approximate any function that fulfills the three constraints \eqref{subeq:Discrete_optimization_bound}-\eqref{subeq:Discrete_optimization_Mono}. 
% Furthermore, requirement 3) is accomplished by the hard constraints imposed by  the rectified linear unit (ReLU) function $\sigma(x)=\max(0,x)$. We firstly 
% elaborate the construction of neural network controller by Lemma~\ref{lemma:u_f+-}-Lemma~\ref{lemma:u_f-}.  Then we show by Theorem~\ref{theorem:Universial Approximation} that   
% the proposed construction can universally approximate any functions that fulfill the three requirements. 







%Theorem~\ref{theorem:Universial Approximation} states that the proposed structure in Lemma~\ref{lemma:u_f+-} can universally approximate any function satisfy the three requirements. 




%(**The following one paragraph is copied from the book \cite{aastrom2010feedback}. This may be attached in Appendix)
%Theorem (Krasovski-Lasalle principle). Let $V: \mathbb{R}^{n} \rightarrow \mathbb{R}$ be a locally positive definite function such that on the compact set $\Omega_{r}=\left\{x \in \mathbb{R}^{n}: V(x) \leq r\right\}$ we have $\dot{V}(x) \leq 0 .$ Define
%\[
%S=\left\{x \in \Omega_{r}: \dot{V}(x)=0\right\}
%\]
%As $t \rightarrow \infty,$ the trajectory tends to the largest invariant set inside $S ;$ i.e., its $\omega$ limit set is contained inside the largest invariant set in S. In particular, if $S$ contains $\mathrm{no}$ invariant sets other than $x=0,$ then 0 is asymptotically stable. 


%\subsection{Monotonic function requirement from optimality condition}\label{section:Monotonic_function}
%In order to further realize exponential stability, we enforce that the control function $u_i(\omega_i)$ for each bus $i$ is monotonic increasing with $\omega_i$. We prove that monotonic increasing control function is a sufficient condition for exponential stability as follows.





==> Secondary Control_Arxiv/simulation.tex <==
In this section, we provide numerical validation for the performance of our RL-DAI on the $39$-bus New England system~\cite{athay1979practical}. First, we will train the optimal control policy $\boldsymbol{u}(\boldsymbol{s})=\left(u_i(s_i;\Xi_i(d)), i \in \mathcal{N} \right)$ for the RL-DAI on the power system model as described in Section~\ref{ssec:RNN-train}. Then, we will validate the performance of the trained RL-DAI in response to sudden step changes in power. 

% \begin{figure}[ht]
% \centering
% \includegraphics[width=0.95\columnwidth]{figures/fre_OS.eps}
% \caption{Frequency deviations in the original system without additional frequency control $\boldsymbol{u}$ when a $\SI{-3}{\pu}$ step change in power injection is introduced to buses $13$, $21$, and $27$.}
% \label{fig:sw-simu}
% \end{figure}


% First, we will train the optimal control policy $\boldsymbol{u}(\boldsymbol{s})=\left(u_i(s_i;\Xi_i(d)), i \in \mathcal{N} \right)$ for the RL-DAI on an ideal power system model as described in Section~\ref{ssec:RNN-train}. Then, we will validate the performance of the well-trained RL-DAI on a more realistic power system test case in Power System Toolbox (PST) [28] for Matlab. 

The dynamic model of the $39$-bus New
England system contains $10$ generator buses and $29$ load buses, whose union is denoted as $\mathcal{N}$. Each of the $10$ generator buses is distinctly indexed by some $i\in\left\{30,\ldots,39\right\}:=\mathcal{G}$ and each of the $29$ load buses is distinctly indexed by some $i\in\left\{1,\ldots,29\right\}:=\mathcal{L}$. The generator inertia constant $m_i$, the voltage magnitude $v_i$, and the  susceptance $B_{ij}$ are directly obtained from the dataset. Given that the values of frequency sensitivity coefficients are not provided by the dataset, we set $\alpha_i = \SI{150}{\pu}$, $\forall i\in\mathcal{G}$, and $\alpha_i= \SI{100}{\pu}$, $\forall i\in\mathcal{L}$.\footnote{All per unit values are on the system base, where the system power base
is $S_0=\SI{100}{\mega\VA}$ and the nominal system frequency is $f_0=\SI{50}{\hertz}$.}

We then add frequency control $u_i$ governed by our RL-DAI to each bus, where there is a connected underlying communication graph $\left(\mathcal{V},\mathcal{E}_\mathrm{Q} \right)$.
% is represented by the blue dashed lines in Fig.~\ref{fig:39bus} with $Q_{ij}=125$, $\forall \{i,j\} \in\mathcal{E}_\mathrm{Q}$.
The operational cost functions are assumed to be $C_i(u_i)= c_i u_i^4/4+b_i, \forall i\in\mathcal{N},$ where the
cost coefficients $c_i$ and $b_i$ are generated randomly from $(0,1)$ and $(0,0.001)$, respectively. Thus, $\forall i\in\mathcal{N}$, $\nabla C_i(u_i)=c_i u_i^3$ by \eqref{eq:cost-power-grad} and $\zeta_i=c_i^{1/3}$ by \eqref{eq:zeta}, which determines the evolution of the integral variable $s_i$ in RL-DAI according to \eqref{eq:DAI-s-general}. Then we train the control policy $\boldsymbol{u}(\boldsymbol{s})=\left(u_i(s_i;\Xi_i(d)), i \in \mathcal{N} \right)$ as described in Section~\ref{sec:RL}.

\subsection{Training of Stacked ReLU Monotonic Neural Networks}
Following the RNN-based RL algorithm illustrated in Section~\ref{ssec:RNN-train}, we can train the stacked ReLU monotonic neural networks that construct control policy $\boldsymbol{u}(\boldsymbol{s})$ satisfying Assumption~\ref{ass-cost-grad-scale} for RL-DAI. Specifically, each sample of system trajectory is generated by disturbing random step power changes $\boldsymbol{p}$ to the system that is initially at a given supply-demand balanced setpoint, where each $p_i$ is drawn uniformly from $(-5,5)\SI{}{\pu}$. %We use a neural network with one hidden layer with 40 neurons (ReLU activation function) and the continuous system is discretized with a sampling interval of 0.5ms. We train with 50 epochs, each with 64 batches with a learning rate of 0.4 (exponentially decayed). 
The values of all the hyperparameters mentioned in Section~\ref{ssec:RNN-train} are summarized as follows: $\rho=0.01$, $d=20$, $h=\SI{0.5}{\milli\second}$, $T=\SI{2.5}{\second}$, $|\mathcal{B}|=64$, $E=50$, and $\xi=0.4$ (exponentially decayed).
% The values of all the hyperparameters mentioned in Section~\ref{ssec:RNN-train} are:  summarized in Table~\ref{table:parameter}. 
% As shown in Fig.~\ref{fig:loss-traj}, the loss $J$ is reduced by around $30\%$ after the training of RL-DAI.

% \begin{table}[!ht]
% \renewcommand{\arraystretch}{1.3}
% \centering
% \caption{Hyperparameters for RNN-Based RL}
% \begin{threeparttable}[t]
% \begin{tabular}{c|c|c}
% \arrayrulecolor[rgb]{.7,.8,.9}
% \hline\hline
% Hyperparameters & Symbol & Value\\
% \hline
% Tradeoff coefficient & $\rho$ & $0.01$\\
% \hline
% Number of hidden neurons & $2d$ & $40$ \\
% \hline
% Sampling interval & $h$ & \SI{0.5}{\milli\second} \\
% \hline
% Time horizon  & $T$ & \SI{2.5}{\second} \\
% \hline
% Batch size
% & $|\mathcal{B}|$ & $64$ \\
% \hline
% Number of
% epochs & $E$ & $50$ \\ 
% \hline
% Learning rate & $\xi$ & $0.4$ (exponentially decayed)\\
% \hline\hline
% \end{tabular}
% \end{threeparttable}
% \label{table:parameter}
% \end{table}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=0.95\columnwidth]{figures/loss_nonlinear.eps}
% \caption{Loss over epochs for training RL-DAI.}
% \label{fig:loss-traj}
% \end{figure}



% \begin{figure}[t!]
% \centering
% \subfigure[Frequency deviations on generator buses]
% {\includegraphics[width=0.9\columnwidth]{figures/fre_RLDAI.eps}\label{fig:RLDAI-fre}}
% %\hfil
% \subfigure[Integral variables]
% {\includegraphics[width=0.9\columnwidth]{figures/s_RLDAI.eps}\label{fig:s_RL-DAI}}
% % %\hfil
% \subfigure[Controllable power injections]
% {\includegraphics[width=0.9\columnwidth]{figures/u_RLDAI.eps}\label{fig:u_RL-DAI}}
% %\hfil
% \subfigure[Marginal costs]
% {\includegraphics[width=0.9\columnwidth]{figures/mc_RLDAI.eps}\label{fig:mc_RL-DAI}}
% %\hfil
% \subfigure[Operational costs]
% {\includegraphics[width=0.9\columnwidth]{figures/oc_RLDAI.eps}\label{fig:op-cost-RA-DAI}}
% \caption{Performance of the system under RL-DAI when a $\SI{-3}{\pu}$ step change in power injection is introduced to buses $13$, $21$, and $27$.}
% \label{fig:perform-RLDAI}
% \end{figure}


\subsection{Time-Domain Responses Following Power imbalances}
For the purpose of comparison, the frequency deviation
of the original system without additional frequency control $\boldsymbol{u}$ when there is a step change
of $\SI{3}{\pu}$ in power consumption at buses $13$, $21$, and $27$ is provided in Fig.~\ref{fig:sw-simu}. Clearly, in the absence of proper control, there exists noticeable steady-state frequency deviation from the nominal frequency. The performance
of the system under RL-DAI in the same scenario is given in Fig.~\ref{fig:perform-RLDAI}. Some observations are in order. First, observe from Fig.~\ref{fig:RLDAI-fre} that RL-DAI can perfectly restore the frequencies to the nominal value as predicted by Theorem~\ref{thm:equilibrium}. Second, Fig.~\ref{fig:mc_RL-DAI} confirms that RL-DAI help generators and loads asymptotically achieve identical marginal costs and thus the optimal steady-state economic dispatch problem is solved. Third, a comparison between Fig.~\ref{fig:sw-simu} and Fig.~\ref{fig:RLDAI-fre} shows that RL-DAI improves the frequency Nadir.
Last but not least, the nuances between the shapes of the trajectories of $\boldsymbol{s}$ and $\boldsymbol{u}$ in Fig.~\ref{fig:s_RL-DAI} and Fig.~\ref{fig:u_RL-DAI} are indicators of the nonlinearity of the learned control policy $\boldsymbol{u}(\boldsymbol{s})$. Clearly, this nonlinearity has not jeopardized the stability of the system.

\begin{figure}[t!]
\centering
\includegraphics[width=0.96\columnwidth]{fre_OS-eps-converted-to.pdf}
\caption{Frequency deviations in the original system without additional frequency control $\boldsymbol{u}$ when a $\SI{-3}{\pu}$ step change in power injection is introduced to buses $13$, $21$, and $27$.}
\label{fig:sw-simu}
\end{figure}

\begin{figure}[t!]
\centering
\subfigure[Frequency deviations on generator buses]
{\includegraphics[width=0.96\columnwidth]{fre_RLDAI-eps-converted-to.pdf}\label{fig:RLDAI-fre}}
%\hfil
\subfigure[Integral variables]
{\includegraphics[width=0.96\columnwidth]{s_RLDAI-eps-converted-to.pdf}\label{fig:s_RL-DAI}}
% %\hfil
\subfigure[Controllable power injections]
{\includegraphics[width=0.96\columnwidth]{u_RLDAI-eps-converted-to.pdf}\label{fig:u_RL-DAI}}
%\hfil
\subfigure[Marginal costs]
{\includegraphics[width=0.96\columnwidth]{mc_RLDAI-eps-converted-to.pdf}\label{fig:mc_RL-DAI}}
%\hfil
\subfigure[Operational costs]
{\includegraphics[width=0.96\columnwidth]{oc_RLDAI-eps-converted-to.pdf}\label{fig:op-cost-RA-DAI}}
\caption{Performance of the system under RL-DAI when a $\SI{-3}{\pu}$ step change in power injection is introduced to buses $13$, $21$, and $27$.}
\label{fig:perform-RLDAI}
\end{figure}


==> name.tex <==

To constrain the search space of the set of stabilizing controllers, we derive the structural properties of neural network controllers \textcolor{blue}{from the perspective of Lyapunov stability. More precisely, by finding an appropriate Lyapunov function,} we show that, if \textcolor{blue}{the output of each controller is monotonically} increasing with respect to the local frequency deviation, then the system has a unique equilibrium that is locally exponentially stable. \textcolor{blue}{In addition, we impose this monotonicity as a hard constraint on the neural networks via properly designed weights and biases, which results in piecewise linear controllers to be trained.}  
% The Lyapunov approach allows us to analytically ascertain the stability of the equilibrium for a compact set of points in the state space. The next theorems are the main results of the paper. 


\subsection{Uniqueness of the Equilibrium}
Notably, the \textcolor{blue}{frequency} dynamics of the system in~\eqref{subeq:Dynamic_w} depends only on the voltage phase angle differences, \textcolor{blue}{which means that the same phase shift on each bus will not affect the frequency dynamics. Therefore, for ease of analysis, we make the following change of coordinates to the system in~\eqref{eq:Dynamic}: $$\delta_i:=\theta_i-\dfrac{1}{n}\sum_{i=1}^{n} \theta_i\,,$$
where $\boldsymbol{\delta}:=\left(\delta_i, i \in \mathcal{V} \right) \in \real^n$ can be understood as the center-of-inertia coordinates~\cite{weitenberg2018robust}. Then, the system dynamics in~\eqref{eq:Dynamic} can be written as}
\begin{subequations}\label{eq:equlibrium_change_cor}
    \begin{align}
\dot{\delta_i} &=\omega_i-\frac{1}{n}\sum_{i=1}^n\omega_i\,, \\
 M_{i}\dot{\omega}_{i} &=P_{m,i}- D_i \omega_i-u_i({\omega}_i)-\sum_{j=1}^{n}B_{i j}\sin(\delta_i-\delta_j)\,,
    \end{align}
\end{subequations}
whose equilibrium points can be characterized by the lemma below.

\begin{lem}[Synchronous solution]\label{lemma:exis-sync} If there exists any equilibrium point $(\boldsymbol{\delta}^\ast, \boldsymbol{\omega}^\ast)$ of~\eqref{eq:equlibrium_change_cor}, then it must satisfy 
\begin{subequations}\label{eq:equli-sync}
    \begin{align}
\omega_i^\ast &=\omega^\ast\,, \label{eq:equli-sync-omega}\\
 0 &=P_{m,i}- D_i \omega^\ast-u_i(\omega^\ast)-\sum_{j=1}^{n}B_{i j}\sin(\delta_i^\ast-\delta_j^\ast)\,,\label{eq:equli-sync-delta}
    \end{align}
\end{subequations}
where the synchronous frequency $\omega^\ast$ is determined by
\begin{align}\label{eq:sync-fre}
    \sum_{i=1}^n u_i(\omega^\ast)+\omega^\ast\sum_{i=1}^n D_i=\sum_{i=1}^n P_{m,i}\,.
\end{align}
\end{lem}
\begin{proof} 
In steady state, \eqref{eq:equlibrium_change_cor} yields
\begin{subequations}\label{eq:equli}
    \begin{align}
\omega_i^\ast &=\frac{1}{n}\sum_{i=1}^n\omega_i^\ast\,, \label{eq:omega-i-eq}\\
 0 &=P_{m,i}- D_i \omega_i^\ast-u_i(\omega_i^\ast)-\sum_{j=1}^{n}B_{i j}\sin(\delta_i^\ast-\delta_j^\ast)\,.\label{eq:delta-i-eq}
    \end{align}
\end{subequations}
Clearly, \eqref{eq:omega-i-eq} implies that there exists some $\omega^\ast$ such that \eqref{eq:equli-sync-omega} holds. Then, \eqref{eq:delta-i-eq} becomes \eqref{eq:equli-sync-delta}. Moreover, we can characterize $\omega^\ast$ as in \eqref{eq:sync-fre} by summing \eqref{eq:equli-sync-delta} over $i$, where the zero net power flow balance, i.e., $\sum_{i=1}^{n}\sum_{j=1}^{n}B_{i j}\sin(\delta_i^\ast-\delta_j^\ast)=0$, is used. 
\end{proof}

Lemma~\ref{lemma:exis-sync} characterizes any possible equilibrium point of~\eqref{eq:equlibrium_change_cor} as a synchronous solution, where the system frequency deviation synchronizes to $\boldsymbol{\omega}^\ast=\bm{1}\omega^\ast$ such that the total power imbalance can be met by the total frequency response as in \eqref{eq:sync-fre}. Note that the existence of equilibrium points is equivalent to the feasibility of the power flow in \eqref{eq:equli-sync-delta}, which is a standing assumption of this manuscript. Additionally, provided that phase angle differences between neighboring buses are usually small for power systems in steady state, we make another standard assumption throughout this manuscript that     $|\delta_i^\ast-\delta_j^\ast|\in [0,\pi/2), \forall \{i,j\}\in \mathcal{E}$~\cite{weitenberg2018robust, weitenberg2018exponential}.

In general, it is not easy to know which equilibrium point the system will settle into under an arbitrary control law $u_i(\omega_i)$. However, we can show that, if $u_i(\omega_i)$ is monotonically increasing with respect to $\omega_i$, then the equilibrium point is unique, which is the main idea of the next lemma.
\begin{lem}[Unique equilibrium] If the control output $u_i(\omega_i)$ is a monotonically increasing function of the local frequency deviation $\omega_i$, then the equilibrium point described by \eqref{eq:equli-sync} is unique.
\end{lem}
\begin{proof} We begin by showing the uniqueness of $\omega^\ast$. By way of contradiction, suppose that both $\omega^\ast$ and $\omega^\star$ satisfy \eqref{eq:sync-fre}, where $\omega^\ast\neq\omega^\star$. Then, $$\sum_{i=1}^n u_i(\omega^\ast)+\omega^\ast\sum_{i=1}^n D_i=\sum_{i=1}^n u_i(\omega^\star)+\omega^\star\sum_{i=1}^n D_i\,,$$
which yields
\begin{equation}\label{eq:uni-omega-pro}
\sum_{i=1}^n \dfrac{u_i(\omega^\ast)-u_i(\omega^\star)}{\omega^\ast-\omega^\star}=-\sum_{i=1}^n D_i<0\,.    
\end{equation}
However, if $u_i(\omega_i)$ is monotonically increasing, then the left hand side of the equality in \eqref{eq:uni-omega-pro} must be nonnegative, which is a contradiction. Thus, $\omega^\ast$ is unique. Then, the uniqueness of $\boldsymbol{\delta}^\ast$ follows from the same argument as in~\cite[Lemma~1]{weitenberg2018exponential}.
\end{proof}


%  suppose

% Assume that the system \eqref{eq:Dynamic} admits a synchronous solution that for all $i=1,\cdots,N$, we have $(\bm{\theta}^*, \bm{\omega}^*) := (\bm{\theta}_{0}^*+t\omega^*\mathbf{1}_n, \omega^\ast\mathbf{1})$ with $\mathbf{1} \in \mathbb{R}^N $ being the vector of all ones.  



%That means that there is not a fixed equilibrium for system~\eqref{eq:Dynamic} and thus the stability of the system is not well defined. In this subsection, we first show that there exists a unique synchronous frequency given the monotonicity property of the controller in Lemma~\ref{lemma:exis-sync}, and then define a unique equilibrium  in Lemma~\ref{lemma:unique_equlibrium} after a change of coordinate.  



% \begin{lem}[Synchronous solution]\label{lemma:exis-sync} If the control function $u_i(\omega_i)$ are monotonically increasing with respect to $\omega_i$ for all $i=1,\cdots,N$, there exists a unique synchronous frequency $\omega^*$ given by $\sum_{i=1}^Nu_i(\omega^*)+\omega^*\sum_{i=1}^ND_i=\sum_{i=1}^NP_{m,i}$ suppose the feasibility of power flow at $\omega^*$. The angle in~\eqref{eq:Dynamic} admits a synchronous solution that for all $i=1,\cdots,N$, $\theta_i^*=\theta_{i,0}^*+t\omega^*$ defined by

%  suppose

% Assume that the system \eqref{eq:Dynamic} admits a synchronous solution that for all $i=1,\cdots,N$, we have $(\bm{\theta}^*, \bm{\omega}^*) := (\bm{\theta}_{0}^*+t\omega^*\mathbf{1}_n, \omega^\ast\mathbf{1})$ with $\mathbf{1} \in \mathbb{R}^N $ being the vector of all ones.  
%  \begin{subequations}\label{eq:equlibrium}
%     \begin{align}
%     \dot{\theta}_i^*=& \omega^*,\label{subeq:equ_delta}\\
%     0=& P_{m,i}-
%     D_i \omega^* - u_i(\omega^*)- \sum_{j=1}^N  B_{ij}\sin{\left(\theta_{i,0}^*-\theta_{j,0}^*\right)} \label{subeq:equ_omega}
%     \end{align}
% \end{subequations}
% \end{lem}
% \begin{proof}
% At the synchronous frequency, $\omega_i=\omega^*$ for all $i=1,\cdots,N$ and thus the system dynamics~\eqref{eq:Dynamic} shrink to~\eqref{subeq:equ_omega},   where~\eqref{subeq:equ_omega} assumes the feasibility of the power flow at $\omega^*$. Note that $B_{ij}=B_{ji}$ for all $i,j=1,\cdots,N$, we have $\sum_{i=1}^N \sum_{j=1}^N  B_{ij}\sin{\left(\theta_{i,0}^*-\theta_{j,0}^*\right)}=0$. Summing over~\eqref{subeq:equ_omega} for all $i=1,\cdots,N$ gives the synchronous frequency $\sum_{i=1}^Nu_i(\omega^*)+\omega^*\sum_{i=1}^ND_i=\sum_{i=1}^NP_{m,i}$. Moreover, since $\sum_{i=1}^ND_i>0$, we have $\sum_{i=1}^Nu_i(\omega)+\omega\sum_{i=1}^ND_i$ monotonically increases with respect to $\omega$. Therefore, $\omega^*$ is a unique synchronous frequency. The solution of power flow equation~\eqref{subeq:equ_omega} at $\omega^*$ gives the set of $\theta_{i,0}^*$.
% \end{proof}


% Since angle $\theta^*$ rotates with the same synchronous frequency $\omega^*$, the angle difference is fixed. This subsequently leads to a fixed equilibrium point if introducing a change of coordinates for the phase angle~\cite{weitenberg2018robust}. Let $\delta_i=\theta_i-\sum_{i=1}^{n} \theta_i$ be angle in the center-of-inertia coordinates. In these coordinates, the system (1) becomes


%  \begin{subequations}\label{eq:equlibrium_change_cor}
%     \begin{align}
% \dot{\delta_i} &=\omega_i-\frac{1}{n}\sum_{i=1}^n\omega_i \\
%  M_{i}\dot{\omega}_{i} &=P_{m,i}- D_i \omega_i-u_i({\omega}_i)-\sum_{j=1}^{N}B_{i j}\sin(\delta_i-\delta_j)
%     \end{align}
% \end{subequations}
%The next lemma shows that the dynamics after the change of coordinates have an unique equilibrium.


% \begin{assumption}[Security constraint]~\cite[Assumption~2]{weitenberg2018robust } \label{assumption:angle_difference}
% The angle difference is such that $\delta_i-\delta_j \in \left[-\frac{\pi}{2}+\rho, \frac{\pi}{2}-\rho\right]$ for a sufficiently small positive constant scalar. The space of $\delta$ is denoted by $\Theta :=\left \{\delta| \delta_i-\delta_j \in \left[-\frac{\pi}{2}+\rho, \frac{\pi}{2}-\rho\right] \right \}$.
% \end{assumption}

% Remark 1: Inspired by~\cite{weitenberg2018robust}, we adopt a positive constant $\rho$ as  an extra margin  on the constraint to quantify the decay of the Lyapunov function we will use to derive a  stabilizing controller.


% \begin{lemma}[Unique Equilibrium]~\cite[Lemma~1]{weitenberg2018exponential }\label{lemma:unique_equlibrium}
% Given the uniqueness of synchronous frequency $\omega^*$ in Lemma~\ref{lemma:exis-sync}, if $|\delta_i-\delta_j|\in [0,\pi/2)$ for all $ (i,j)\in \mathcal{E}$, the system~\eqref{eq:equlibrium_change_cor} has an unique equilibrium  $\{(\delta^*,\omega^*)|\sum_{i=1}^Nu_i(\omega^*)+\omega^*\sum_{i=1}^ND_i-\sum_{i=1}^NP_{m,i}=0, \quad P_{m,i}-
%     D_i \omega^* - u_i(\omega^*)- \sum_{j=1}^n  B_{ij}\sin{\left(\delta_{i}^*-\delta_{j}^*\right)} , i =1, \dots, N\}$. 
% If the control function $u_i(\omega_i)$ are monotonically increasing with respect to $\omega_i$ for all $i=1,\cdots,N$, then there exists a unique synchronous frequency $\omega^*$ given by $\sum_{i=1}^Nu_i(\omega^*)+\omega^*\sum_{i=1}^ND_i=\sum_{i=1}^NP_{m,i}$. there exists unique $\delta^*$ such that $P_{m,i}-
%     D_i \omega^* - u_i(\omega^*)- \sum_{j=1}^n  B_{ij}\sin{\left(\delta_{i}^*-\delta_{j}^*\right)}$ for all $ i =1, \dots, N$.
%\end{lemma}
%\begin{proof}
 
 
 
% Under the unique synchronous frequency $\omega^*$, the angle $\delta^*$ in synchronous solution needs to satisfy $
% \sum_{j=1}^n  B_{ij}\sin{\left(\delta_{i}^*-\delta_{j}^*\right)} = P_{m,i}-
%     D_i \omega^* - u_i(\omega^*) $
% The system~\eqref{eq:equlibrium_change_cor} and~\eqref{eq:Dynamic} share the same unique synchronous  frequency $\omega^*$ by following the same line of proof in Lemma~\ref{lemma:exis-sync}. According to~\cite[Lemma~1]{weitenberg2018exponential }, if $|\delta_i-\delta_j|\in [0,\pi/2)$ for all $ (i,j)\in \mathcal{E}$ there exist a unique set of $\delta^*$ such that $
% \sum_{j=1}^n  B_{ij}\sin{\left(\delta_{i}^*-\delta_{j}^*\right)} = P_{m,i}-
%     D_i \omega^* - u_i(\omega^*) $ for all $ i =1, \dots, N$. 
% \end{proof}



%Lyapunov's method asertain the stability of the equilibrium point of a nonlinear dynamic system without numerical integraion, which forms a powerful tool to investigate the general structure property of the controllers that guarantee the transient stability of the system \cite{sauer2017power} .



\subsection{Lyapunov Stability Analysis}
Having characterized the equilibrium point of \eqref{eq:equlibrium_change_cor}, we are now ready to investigate the system stability by first finding an effective Lyapunov function $V(\boldsymbol{\delta}, \boldsymbol{\omega})$ such that $V(\boldsymbol{\delta}^\ast, \boldsymbol{\omega}^\ast)=0$ and $V(\boldsymbol{\delta}, \boldsymbol{\omega})>0, \forall(\boldsymbol{\delta}, \boldsymbol{\omega})\in \mathcal{D}\setminus{(\boldsymbol{\delta}^\ast, \boldsymbol{\omega}^\ast)}$ with the domain $\mathcal{D}:=\! \Set*{(\boldsymbol{\delta}, \boldsymbol{\omega})\in \real^n \times \real^n}{|\delta_i-\delta_j|\in [0,\pi/2), \forall \{i,j\}\in \mathcal{E}}$. Inspired by~\cite{weitenberg2018robust}, we consider the following Lyapunov function candidate:
\begin{align}\label{eq: Lyapunov}
V(\boldsymbol{\delta}, \boldsymbol{\omega})=&\ \frac{1}{2}\sum_{i=1}^{n} M_i(\omega_{i}-\omega^\ast)^{2}+W_\mathrm{p}(\boldsymbol{\delta})+\epsilon W_\mathrm{c}(\boldsymbol{\delta}, \boldsymbol{\omega})
\end{align}
with
\begin{subequations}
\begin{align}
    W_\mathrm{p}(\boldsymbol{\delta}) := 
&-\frac{1}{2}\sum_{i=1}^{n} \sum_{j=1}^{n} B_{ij}\left( \cos(\delta_{ij}) -\cos(\delta_{ij}^*)\right)\nonumber\\
&-\sum_{i=1}^{n}\sum_{j=1}^{n} B_{ij} \sin(\delta_{ij}^*)( \delta_{i}-\delta_{i}^*)\,,\label{eq:Wp}\\
W_\mathrm{c}(\boldsymbol{\delta}, \boldsymbol{\omega}):=&\sum_{i=1}^{n} \sum_{j=1}^{n}B_{ij}\left(  \sin(\delta_{ij})-\sin(\delta_{ij}^*)\right)M_i(\omega_i-\omega^\ast)\,,\nonumber
\end{align}
\end{subequations}
where $\epsilon>0$ is a tunable parameter that should be set small enough. Here, the first term is the kinetic energy of the turbines, the second term is the potential energy of the system stored in the inductive transmission
lines of the power network, and the last cross term between kinetic and potential energies is included for the purpose of proving the exponential stability, which should be clear later. Strictly speaking, this function is not a ``true'' Lyapunov function since it is not nonnegative in the entire state space, i.e., $\forall (\boldsymbol{\delta}, \boldsymbol{\omega})\in \real^n \times \real^n$. That is, it is not bounded from below. Thus, we use it only to show that trajectories starting not too far away from the equilibrium point would converge to it. To see that $V(\boldsymbol{\delta}, \boldsymbol{\omega})$ is a well-defined Lyapunov function on $\mathcal{D}$, it suffices to show the lemma below.  

\begin{lem}[Bounds on Lyapunov function]\label{lemma:Pos_Lyapunov}
$\forall (\boldsymbol{\delta}, \boldsymbol{\omega})\!\in\! \mathcal{D}$, the Lyapunov function $V(\boldsymbol{\delta}, \boldsymbol{\omega})$ in~\eqref{eq: Lyapunov} satisfies
$$
\alpha_{1}(\|\delta-\delta^*\|_2^{2}+\|\omega-\omega^*\|_2^{2}) \leq V(\boldsymbol{\delta}, \boldsymbol{\omega}) \leq \alpha_{2}(\|\delta-\delta^*\|_2^{2}+\|\omega-\omega^*\|_2^{2})
$$
for some constants $\alpha_{1}>0$ and $\alpha_{2}>0$.
\end{lem}
\begin{proof}
The proof is similar to the one of~\cite[Lemma~14]{weitenberg2018robust}, which bounds $V(\boldsymbol{\delta}, \boldsymbol{\omega})$ term by term. Firstly, the kinetic energy term is easily bounded by Rayleigh-Ritz theorem~\cite{Horn2012MA} as
\begin{align}\label{eq:bound-Wk}
     \frac{1}{2}\lambda_\mathrm{min}(\boldsymbol{M})||\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast||^2_2\leq \frac{1}{2}\sum_{i=1}^{n}M_i(\omega_{i}-\omega^\ast)^{2}\leq\frac{1}{2}\lambda_\mathrm{max}(\boldsymbol{M})||\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast||^2_2\,.
\end{align}
Then, with a direct application of~\cite[Lemma~4]{weitenberg2018exponential}, the potential energy term $W_\mathrm{p}(\boldsymbol{\delta})$ in \eqref{eq:Wp} can be bounded by 
\begin{align}\label{eq:bound-Wp}
\beta_{1}\left\|\boldsymbol{\delta}-\boldsymbol{\delta}^{\ast}\right\|_2^2 \leq W_\mathrm{p}(\boldsymbol{\delta}) \leq \beta_{2}\left\|\boldsymbol{\delta}-\boldsymbol{\delta}^{\ast}\right\|_2^2    
\end{align}
for some constants $\beta_{1}>0$ and $\beta_{2}>0$. To deal with the cross term $W_\mathrm{c}(\boldsymbol{\delta})$, we define $p_{\mathrm{e},i}(\boldsymbol{\delta}):=\sum_{j=1}^{n} B_{ij} \sin(\delta_{ij})$. Then, $W_\mathrm{c}(\boldsymbol{\delta}) =\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)^T\!\boldsymbol{M}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)$. Clearly, $-|W_\mathrm{c}(\boldsymbol{\delta})|\leq W_\mathrm{c}(\boldsymbol{\delta})\leq|W_\mathrm{c}(\boldsymbol{\delta})|$. Now, as shown in the proof of~\cite[Lemma~1]{weitenberg2018exponential}, $\forall \boldsymbol{x},\boldsymbol{y}\in\real^{n}$, the inequality $2|\boldsymbol{x}^T\boldsymbol{y}|\leq||\boldsymbol{x}||^2_2+||\boldsymbol{y}||^2_2$
holds. Thus, we have
\begin{align*}
|W_\mathrm{c}(\boldsymbol{\delta})|\leq&\ \dfrac{1}{2}\left(||\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)||^2_2+||\boldsymbol{M}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)||^2_2\right)\nonumber \\
\leq&\ \dfrac{1}{2}\left(\gamma_2||\boldsymbol{\delta}\!-\!\boldsymbol{\delta}^\ast||^2_2+\lambda_\mathrm{max}(\boldsymbol{M})^2||\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast||^2_2\right)\,,
\end{align*}
where the second inequality comes from~\cite[Lemma~4]{weitenberg2018exponential} and Rayleigh-Ritz theorem.
% \begin{align}
%     &\frac{1}{2}\sum_{i=1}^{n} M_i(\omega_{i}-\omega^\ast)^{2} + \epsilon W_\mathrm{c}(\boldsymbol{\delta}, \boldsymbol{\omega})\nonumber\\=&\dfrac{1}{2}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)^T\!\boldsymbol{M}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast) + \epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)^T\!\boldsymbol{M}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)\nonumber\\
%     =&\dfrac{1}{2}\begin{bmatrix}
% \boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})-\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\\ 
% \boldsymbol{\omega}-\boldsymbol{\omega}^\ast
% \end{bmatrix}^T
% \!\!\begin{bmatrix}
% \boldsymbol{0} & \!\!\epsilon\boldsymbol{M}\\ 
% \epsilon\boldsymbol{M} & \!\!\boldsymbol{M}
% \end{bmatrix}\!
% \begin{bmatrix}
% \boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})-\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\\ 
% \boldsymbol{\omega}-\boldsymbol{\omega}^\ast
% \end{bmatrix}\!\,.
% \end{align}
% By~\cite[Lemma~5]{weitenberg2018exponential}, we have
% $$
% \begin{bmatrix}
% -\epsilon\boldsymbol{I} & \boldsymbol{0}\\ 
% \boldsymbol{0}& \boldsymbol{M}-\epsilon\boldsymbol{M}^2 
% \end{bmatrix}
% \preceq 
% \begin{bmatrix}
% \boldsymbol{0} & \!\!\epsilon\boldsymbol{M}\\ 
% \epsilon\boldsymbol{M} & \!\!\boldsymbol{M}
% \end{bmatrix}
% \preceq 
% \begin{bmatrix}
% \epsilon\boldsymbol{I} & \boldsymbol{0}\\ 
% \boldsymbol{0}& \epsilon\boldsymbol{M}^2 +\boldsymbol{I}
% \end{bmatrix}
% $$
Hence, 
\begin{align}\label{eq:bound-Wc}
&-\dfrac{1}{2}\left(\gamma_2||\boldsymbol{\delta}\!-\!\boldsymbol{\delta}^\ast||^2_2+\lambda_\mathrm{max}(\boldsymbol{M})^2||\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast||^2_2\right)\\
&\leq W_\mathrm{c}(\boldsymbol{\delta})\leq \dfrac{1}{2}\left(\gamma_2||\boldsymbol{\delta}\!-\!\boldsymbol{\delta}^\ast||^2_2+\lambda_\mathrm{max}(\boldsymbol{M})^2||\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast||^2_2\right)\,.\nonumber
\end{align}
Finally, combining \eqref{eq:bound-Wk}, \eqref{eq:bound-Wp}, and \eqref{eq:bound-Wc} we can bound the entire Lyapunov function $V(\boldsymbol{\delta}, \boldsymbol{\omega})$ as in \eqref{} with
$$
\begin{aligned}
\alpha_{1} &:=\dfrac{1}{2}\min \left(\lambda_\mathrm{min}(\boldsymbol{M})-\epsilon \lambda_\mathrm{max}(\boldsymbol{M})^2, 2\beta_{1}-\epsilon \gamma_{2}\right)>0\,, \\
\alpha_{2} &:=\dfrac{1}{2}\max \left(\lambda_\mathrm{max}(\boldsymbol{M})+\epsilon \lambda_\mathrm{max}(\boldsymbol{M})^2, 2\beta_2+\epsilon \gamma_{2}\right)>0\,,
\end{aligned}
$$
for sufficiently small $\epsilon>0$.
\end{proof}

It follows directly from Lemma~\ref{lemma:Pos_Lyapunov} that $V(\boldsymbol{\delta}^\ast, \boldsymbol{\omega}^\ast)=0$ and $V(\boldsymbol{\delta}, \boldsymbol{\omega})>0, \forall(\boldsymbol{\delta}, \boldsymbol{\omega})\in \mathcal{D}\setminus{(\boldsymbol{\delta}^\ast, \boldsymbol{\omega}^\ast)}$, which means that the Lyapunov function $V(\boldsymbol{\delta}, \boldsymbol{\omega})$ in~\eqref{eq: Lyapunov} is well-defined. Thus, we can examine the system stability through the time derivative $\dot{V}(\boldsymbol{\delta}, \boldsymbol{\omega})$, whose expression is provided in the next lemma.   

\begin{lem}[Time derivative of Lyapunov function]\label{lemma: dot_V}
The time derivative of the Lyapunov function $V(\boldsymbol{\delta}, \boldsymbol{\omega})$ defined in~\eqref{eq: Lyapunov} is given by 
\begin{align}\label{eq:Vdot}
\dot{V}(\boldsymbol{\delta}, \boldsymbol{\omega}) =&-\!\begin{bmatrix}\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\\\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast\end{bmatrix}^T\!\!\boldsymbol{Q}(\boldsymbol{\delta})\begin{bmatrix}\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\\\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast\end{bmatrix}\\
&-\left[\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast \!\!+\! \epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)\right]^T\left(\boldsymbol{u}(\boldsymbol{\omega})-\boldsymbol{u}(\boldsymbol{\omega}^\ast)\right)\nonumber
\end{align}
with
\begin{equation}
\boldsymbol{Q}(\boldsymbol{\delta}):=
    \begin{bmatrix}
\epsilon\boldsymbol{I}  & \dfrac{\epsilon}{2}\boldsymbol{D} \\  \dfrac{\epsilon}{2}\boldsymbol{D}  & \boldsymbol{D}-\dfrac{\epsilon}{2}(\boldsymbol{H}(\boldsymbol{\delta})\boldsymbol{M}+\boldsymbol{M}\boldsymbol{H}(\boldsymbol{\delta}))
\end{bmatrix}\succ 0\,,
\end{equation}
where $\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}) := \left(p_{\mathrm{e},i}(\boldsymbol{\delta}):=\sum_{j=1}^{n} B_{ij} \sin(\delta_{ij}), i \in \mathcal{V} \right) \in \real^n$ and $\boldsymbol{H}(\boldsymbol{\delta})=\nabla \boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}):=\left[ H_{ij}\right]\in \real^{n \times n}$ such that 
\begin{align}\label{eq:Lij}
    H_{ij}:=
    \begin{dcases}
    -B_{ij}\cos(\delta_{ij}) & \text{if}\ i\neq j\\
    \sum_{j^\prime=1,j^\prime\neq i}^n B_{ij\prime}\cos(\delta_{ij\prime})& \text{if}\ i=j
    \end{dcases}\,,\qquad\forall i,j \in \left[n\right]\,.
\end{align}
% \begin{equation}
% \mathbf{Q}=
%     &\begin{bmatrix}
% \epsilon\mathbf{I}  & \frac{1}{2}\epsilon(\mathbf{D}+\mathbf{K(\omega)}) \\  \frac{1}{2}\epsilon(\mathbf{D}+\mathbf{K(\omega)})  & (\mathbf{D}+\mathbf{K(\omega)})-\frac{\epsilon}{2}(\mathbf{H(\delta)}\mathbf{M}+\mathbf{M}\mathbf{H(\delta)})
% \end{bmatrix} 
% \end{equation}
\end{lem}
\begin{proof}
We start by computing the partial derivatives of $V(\boldsymbol{\delta}, \boldsymbol{\omega})$ with respect to each state, i.e.,
% \begin{subequations}\label{eq: Lyapunov_derivative_partial
% }
% \begin{align}
% \begin{split}
% \frac{\partial V(\delta,\omega) }{\partial \delta_i}&=-P_{e,i}(\delta^*)+ \sum_{j=1}^{N} B_{ij} \sin(\delta_i-\delta_j) \\
% &\quad+\epsilon\sum_{j=1}^NB_{ij}cos(\delta_{ij})\left(M_i(\omega_i-\omega^*)-M_j(\omega_j-\omega^*)\right)
% \end{split}
% \label{subeq: Lyapunov_partial_delta}\\
% \frac{\partial V(\delta,\omega) }{\partial \omega_i}&=M_i\left((\omega_i-\omega^*)+\epsilon\sum_{j=1}^NB_{ij}\left(  \sin(\delta_{ij})-\sin(\delta_{ij}^*)\right)\right)\label{subeq: Lyapunov_partial_w} 
% \end{align}
% \end{subequations}
\begin{subequations}\label{eq: Lyapunov_derivative_partial
}
\begin{align}
\frac{\partial V }{\partial \delta_i}&=p_{\mathrm{e},i}(\boldsymbol{\delta})-p_{\mathrm{e},i}(\boldsymbol{\delta}^\ast) +\epsilon\!\!\sum_{j=1,j\neq i}^nB_{ij}\cos(\delta_{ij})M_i(\omega_i-\omega^\ast)\nonumber\\
&\quad-\epsilon\!\!\sum_{j=1,j\neq i}^n B_{ij}\cos(\delta_{ij})M_j(\omega_j-\omega^\ast)\,,\nonumber
\label{subeq: Lyapunov_partial_delta}\\
\frac{\partial V }{\partial \omega_i}&=M_i\left[\omega_i-\omega^\ast+\epsilon\left(p_{\mathrm{e},i}(\boldsymbol{\delta})-p_{\mathrm{e},i}(\boldsymbol{\delta}^\ast)\right)\right]\,.\nonumber\label{subeq: Lyapunov_partial_w} 
\end{align}
\end{subequations}



% An equilibrium point of the dynamic system is a state $(\delta,\omega)$ where $w_{i}=0$ for $i \in \mathcal{B}$ and $P_{i}= \sum_{j=1}^{N} B_{ij} \sin(\delta_i-\delta_j)$  for $(i, j) \in \mathcal{E},$ i.e., where all frequency deviations are zero and branch power flow equals to the injections. 









% The total derivative of $V$ with respect to $t$ is 
% \begin{equation} \label{eq: Lyapunov_derivative}
%  \begin{aligned} 
% \dot{V}(\delta,\omega) &=\sum_{i=1}^{N}\left(\frac{\partial V(\delta,\omega) }{\partial \delta_i} \dot{\delta_i}+\frac{\partial V(\delta,\omega) }{\partial \omega_i}\dot{\omega_i}\right)
% \\
% &=\sum_{i=1}^{N}\left(P_{e,i}(\delta)-P_{e,i}(\delta^*)\right)\left(\omega_i-\frac{1}{n}\sum_{i=1}^n\omega_i \right)\\ 
% &\quad+\epsilon\left(\sum_{j=1}^NB_{ij}\cos(\delta_{ij})\left(M_i(\omega_i-\omega^*)-M_j(\omega_j-\omega^*)\right)\right)\\
% &\quad\quad\left(\omega_i-\frac{1}{n}\sum_{i=1}^n\omega_i \right)\\
% &\quad+M_i\left((\omega_i-\omega^*)+\epsilon(P_{e,i}(\delta)-P_{e,i}(\delta^*))\right)\left(P_{m,i}- D_i \omega_i-u_i({\omega}_i)-P_{e,i}(\delta)\right)
% \\
% &=-\sum_{i=1}^{N}  (\omega_i-\omega^*) (u_i(\omega_i)-u_i(\omega^*))\\
% &\quad\quadd -\sum_{i=1}^{N}D_i (\omega_i-\omega^*)^2\\
% &\quad\quadd +\epsilon\sum_{i=1}^{N} \xi_i\left(-D_i(\omega_i-\omega^*)-(u_i(\omega_i)-u_i(\omega^*))-\xi_i\right)
% \end{aligned}
% \end{equation}
Therefore, the time derivative of $V(\boldsymbol{\delta}, \boldsymbol{\omega})$ is 
\begin{equation*} 
 \begin{aligned} 
&\dot{V}(\boldsymbol{\delta}, \boldsymbol{\omega}) \\
=&\sum_{i=1}^{n}\left(\frac{\partial V }{\partial \delta_i} \dot{\delta}_i+\frac{\partial V }{\partial \omega_i}\dot{\omega}_i\right)
\\
% =&\ \!\!\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)+\epsilon\boldsymbol{H}(\boldsymbol{\delta})\boldsymbol{M}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)\right)^T\left(\boldsymbol{\omega}-\bm{1}\frac{\bm{1}^T\boldsymbol{\omega}}{n}\right)\\
% &\ \!\!+\!\left[\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast \!\!+\! \epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)\right]^T\!\!\left(P_m\!-\!\boldsymbol{D}\boldsymbol{\omega}\!-\!\boldsymbol{u}(\boldsymbol{\omega})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\right)\\
=&\ \!\!\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)+\epsilon\boldsymbol{H}(\boldsymbol{\delta})\boldsymbol{M}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)\right)^T\left(\boldsymbol{\omega}-\bm{1}\frac{\bm{1}^T\boldsymbol{\omega}}{n}\right)\\
&\ \!\!+\!\left[\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast \!\!+\! \epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)\right]^T\!\!\left(P_m\!-\!\boldsymbol{D}\boldsymbol{\omega}\!-\!\boldsymbol{u}(\boldsymbol{\omega})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\right)\\
&+\underbrace{\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\!+\!\epsilon\boldsymbol{H}(\boldsymbol{\delta})\boldsymbol{M}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)\right)^T\left(\bm{1}\frac{\bm{1}^T\boldsymbol{\omega}}{n}\!-\!\bm{1}\omega^\ast\right)}_{=0}\\
&\ \!\!-\!\left[\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast \!\!+\! \epsilon\!\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)\right]^T\!\!\underbrace{\left(\!P_m\!\!-\!\!\boldsymbol{D}\boldsymbol{\omega}^\ast\!\!\!-\!\boldsymbol{u}(\boldsymbol{\omega}^\ast)\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\!\right)}_{=\boldsymbol{0}}
\\
=&\ \epsilon\left(\boldsymbol{H}(\boldsymbol{\delta})\boldsymbol{M}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)\right)^T(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)-(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)^T\boldsymbol{D}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)\\
&-\epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)^T\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)\\&-\epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)^T\boldsymbol{D}(\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast)\\
&-\left[\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast \!\!+\! \epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)\right]^T\left(\boldsymbol{u}(\boldsymbol{\omega})-\boldsymbol{u}(\boldsymbol{\omega}^\ast)\right)\,,
\end{aligned}
\end{equation*}
which is exactly \eqref{eq:Vdot}. Note that the extra terms in the second equality are added to construct a quadratic format without affecting the the original value of  $\dot{V}(\boldsymbol{\delta}, \boldsymbol{\omega})$ since $\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})^T\bm{1}=\bm{0}$, $\boldsymbol{H}(\boldsymbol{\delta})^T\bm{1}=\bm{0}$, and $P_m\!-\!\boldsymbol{D}\boldsymbol{\omega}^\ast\!-\!\boldsymbol{u}(\boldsymbol{\omega}^\ast)\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)=0$ by the condition at the equilibrium given in \eqref{eq:equli-sync-delta}. 

It remains to show that $\boldsymbol{Q}(\boldsymbol{\delta})\succ0$, which follows directly from the fact that the Schur complement of the block $\epsilon \boldsymbol{I}$ in $\boldsymbol{Q}(\boldsymbol{\delta})$ is positive definite, i.e., $$\boldsymbol{D}-\dfrac{\epsilon}{2}(\boldsymbol{H}(\boldsymbol{\delta})\boldsymbol{M}+\boldsymbol{M}\boldsymbol{H}(\boldsymbol{\delta}))-\frac{\epsilon}{4} \boldsymbol{D}^2\succ 0$$ for sufficiently small $\epsilon$.
% The matrix $\mathbf{H(\delta)}$ is the derivative of $P_e(\delta)$ with respect to $\delta$ and equals to
% \begin{equation}\label{eq:J_delta_w}
%     \begin{split}
%      &\mathbf{H(\delta)}=\\
%     &\begin{bmatrix}
% \begin{smallmatrix}
% \sum_{j=1,j\neq 1}^N B_{1j}\cos{\delta_{1j}} &\hspace{0.5cm} -B_{12}\cos{\delta_{12}} \hspace{0.6cm}   \cdots\hspace{0.6cm}  -B_{1N}\cos{\delta_{1N}}\\
%   -B_{21}\cos{\delta_{21}}& \sum_{j=1,j\neq 2}^N B_{2j}\cos{\delta_{2j}}\quad  \cdots\quad  -B_{2N}\cos{\delta_{2N}}\\
%   \vdots &\ddots\\
%  - B_{N1}\cos{\delta_{N1}}&\hspace{0.8cm}\cdots \hspace{1cm} \sum_{j=1,j\neq N}^N B_{Nj}\cos{\delta_{Nj}}
% \end{smallmatrix}
% \end{bmatrix} \\
%     \end{split},
% \end{equation}
% \textcolor{red}{
% which is a graph Laplacian matrix and equals to 
% $L \operatorname{diag}\left(\left\{B_{i j} \cos \left(\delta_{ij}\right)\right\}_{\{i, j\} \in \mathcal{E}}\right) L^{T}$ with $L \in \mathbb{R}^{N \times|\mathcal{E}|}$ be the  (oriented) incidence matrix~\cite{dorfler2013synchronization}. Since $\delta \in \Theta$, then $\cos \left(\delta_{ij}\right)>0$ for all $i,j=1,\cdots,N$ and thus $\mathbf{H(\delta)}\succeq 0$. To add it later!} 
\end{proof}

From Lemma~\ref{lemma: dot_V} we can see that $u_i(\omega_i)$ plays a part in the cross term $\left[\boldsymbol{\omega}-\boldsymbol{\omega}^\ast + \epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})-\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)\right]^T\left(\boldsymbol{u}(\boldsymbol{\omega})-\boldsymbol{u}(\boldsymbol{\omega}^\ast)\right)$ of $\dot{V}(\boldsymbol{\delta}, \boldsymbol{\omega})$, which in general complicates the analysis of $\dot{V}(\boldsymbol{\delta}, \boldsymbol{\omega})$. However, it is not hard to observe that this cross term is nonnegative for sufficiently small $\epsilon$ if $u_i(\omega_i)$ is monotonically increasing with respect to $\omega_i$, which further implies that $\dot{V}(\boldsymbol{\delta}, \boldsymbol{\omega})<0$, $\forall(\boldsymbol{\delta}, \boldsymbol{\omega})\in \mathcal{D}\setminus{(\boldsymbol{\delta}^\ast, \boldsymbol{\omega}^\ast)}$. Thus, if $u_i(\omega_i)$ is monotonically increasing with respect to $\omega_i$, the system is locally asymptotically stable at the equilibrium point $(\boldsymbol{\delta}^\ast, \boldsymbol{\omega}^\ast)$. Actually, in this case, we can even show local exponential stability as in the next theorem. 
\begin{thm}[Local exponential stability]\label{theorem:Exponential_stable}
If the control output $u_i(\omega_i)$ is a monotonically increasing function of the local frequency deviation $\omega_i$, then the equilibrium point $(\boldsymbol{\delta}^\ast, \boldsymbol{\omega}^\ast)$ described by \eqref{eq:equli-sync} is locally exponentially stable.
\end{thm}

\begin{proof}
%A local Lyapunov function $\begingroup\color{black} V(\delta,\omega)\endgroup$ for the dynamic system represented by  \eqref{eq:Dynamic} is \cite{weitenberg2018robust, weitenberg2018exponential}
% \cite{arapostathis1982global,dobson1989towards,chang1995direct,vu2015lyapunov}
% \begin{equation}\label{eq: Lyapunov}
% \begin{aligned}
% V(\delta,\omega)=&\frac{1}{2}\sum_{i=1}^{N} M_i(\omega_{i}-\omega^*)^{2}-\sum_{i=1}^{N}\sum_{j=1}^{N} B_{ij} \sin(\delta_{ij}^*)( \delta_{i}-\delta_{i}^*) \\
% &-\frac{1}{2}\sum_{i=1}^{N} \sum_{j=1}^{N} B_{ij}\left( \cos(\delta_{ij}) -\cos(\delta_{ij}^*)\right)
% \\
% &+\epsilon\sum_{i=1}^{N} \sum_{j=1}^{N}B_{ij}\left(  \sin(\delta_{ij})-\sin(\delta_{ij}^*)\right)M_i(\omega_i-\omega^*)
% \end{aligned}\end{equation}
% The term $ \frac{1}{2}\sum_{i=1}^{N} M_i(\omega_{i}-\omega^*)^{2} $
% represents the kinetic energy of the turbines and the term $\sum_{i=1}^{N}\sum_{j=1}^{N} B_{ij} \sin(\delta_{ij}^*)( \delta_{i}-\delta_{i}^*) -\frac{1}{2}\sum_{i=1}^{N} \sum_{j=1}^{N} B_{ij}\left( \cos(\delta_{ij}) -\cos(\delta_{ij}^*)\right)$
% is the potential energy of the system stored in the inductive
% lines in the power grid network.
% This function is not a ``true'' Lyapunov function since it is not non-negative on the entire state space (it is not bounded from below) for all $\delta\in \mathbb{R}^N$, and it is used to show that trajectories that start not too far away from the equilibrium point would converge to it. By Lemma~\ref{lemma:Pos_Lyapunov}, the Lyapunov function $V(\delta, \omega)$ in~\eqref{eq: Lyapunov} 
% satisfies
% \begin{equation}\label{eq:bound_Lyapunov}
% \beta_{1}(\|\delta-\delta^*\|_2^{2}+\|\omega-\omega^*\|_2^{2}) \leq V(\delta, \omega) \leq \beta_{2}(\|\delta-\delta^*\|_2^{2}+\|\omega-\omega^*\|_2^{2})
% \end{equation}
% for some positive constants $\beta_{1}$ and $\beta_{2}$, with $\delta \in \Theta$, provided that $\epsilon$ is sufficiently small. 
% Therefore, the function $V(\delta, \omega)$ 
%is a qualified Lyapunov function for the area $\left \{(\delta,\omega)|\delta \in \Theta, \omega\in \mathbb{R}^N  \right \}$. 
The key is to show that, if $u_i(\omega_i)$ is monotonically increasing with respect to $\omega_i$, then there exists a constant $c>0$ such that $\dot{V}(\boldsymbol{\delta}, \boldsymbol{\omega})\leq -cV(\boldsymbol{\delta}, \boldsymbol{\omega})$.

We start by bounding the quadratic term related to $\boldsymbol{Q}(\boldsymbol{\delta})$ in \eqref{eq:Vdot} as follows:
\begin{align}
    &\begin{bmatrix}\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\nonumber\\\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast\end{bmatrix}^T\!\!\boldsymbol{Q}(\boldsymbol{\delta})\begin{bmatrix}\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\nonumber\\\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast\end{bmatrix}\nonumber\\&\geq \lambda_\mathrm{min}(\boldsymbol{Q}(\boldsymbol{\delta}))\left(||\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})\!-\!\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)||^2_2+||\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast||^2_2\right)
    \nonumber\\&\geq \lambda_\mathrm{min}(\boldsymbol{Q}(\boldsymbol{\delta}))\left(\gamma_1||\boldsymbol{\delta}\!-\!\boldsymbol{\delta}^\ast||^2_2+||\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast||^2_2\right)
    \nonumber\\&\geq \lambda_\mathrm{min}(\boldsymbol{Q}(\boldsymbol{\delta}))\min(1, \gamma_1)\left(||\boldsymbol{\delta}\!-\!\boldsymbol{\delta}^\ast||^2_2+||\boldsymbol{\omega}\!-\!\boldsymbol{\omega}^\ast||^2_2\right)
    \nonumber\\&\geq \lambda_\mathrm{min}(\boldsymbol{Q}(\boldsymbol{\delta}))\min(1, \gamma_1)\dfrac{1}{\alpha_2}V(\boldsymbol{\delta}, \boldsymbol{\omega}) \nonumber
    \\&\geq c V(\boldsymbol{\delta}, \boldsymbol{\omega})\label{eq:bound-Q}
\end{align}
with $$c:=\left(\min_{\boldsymbol{\delta}:|\delta_i-\delta_j|\in [0,\pi/2), \forall \{i,j\}\in \mathcal{E}} \!\lambda_\mathrm{min}(\boldsymbol{Q}(\boldsymbol{\delta}))\right)\dfrac{\min(1, \gamma_1)}{\alpha_2}>0\,,$$
where the first inequality is by Rayleigh-Ritz theorem, the second inequality is by~\cite[Lemma~4]{weitenberg2018exponential}, and the fourth inequality is by Lemma~\ref{lemma:Pos_Lyapunov}.

We now show rigorously that, if $u_i(\omega_i)$ is monotonically increasing with respect to $\omega_i$, then the cross term related to them in \eqref{eq:Vdot} is nonnegative for sufficiently small $\epsilon$. Define
\begin{align*}
    k_{i}(\omega_i):=
    \begin{dcases}
    \dfrac{u_i(\omega_i)-u_i(\omega_i^\ast)}{\omega_i-\omega_i^\ast} & \text{if}\ \omega_i \neq\omega_i^\ast\\
    0& \text{if}\ \omega_i=\omega_i^\ast
    \end{dcases}\,,\quad\forall i \in \left[n\right]\,.
\end{align*}
Then, $\boldsymbol{K}(\boldsymbol{\omega}) := \diag{k_{i}(\omega_i), i \in \mathcal{V}} \in \real^{n \times n}\succeq0$ if $u_i(\omega_i)$ is monotonically increasing with respect to $\omega_i$. Hence, 
\begin{align}\label{eq:bound-cross}
&\left[\boldsymbol{\omega}-\boldsymbol{\omega}^\ast + \epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})-\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)\right]^T\left(\boldsymbol{u}(\boldsymbol{\omega})-\boldsymbol{u}(\boldsymbol{\omega}^\ast)\right)\nonumber\\=&\left(\boldsymbol{\omega}-\boldsymbol{\omega}^\ast\right)^T\boldsymbol{K}(\boldsymbol{\omega})\left(\boldsymbol{\omega}-\boldsymbol{\omega}^\ast\right)\nonumber\\ &+\epsilon\left(\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta})-\boldsymbol{p}_\mathrm{e}(\boldsymbol{\delta}^\ast)\right)^T\boldsymbol{K}(\boldsymbol{\omega})\left(\boldsymbol{\omega}-\boldsymbol{\omega}^\ast\right)\nonumber\\\geq&\ \!0\,,  \end{align}
for small enough $\epsilon$.

Finally, combining \eqref{eq:Vdot}, \eqref{eq:bound-Q}, and \eqref{eq:bound-cross}, we have $\dot{V}(\boldsymbol{\delta}, \boldsymbol{\omega})\leq -c V(\boldsymbol{\delta}, \boldsymbol{\omega})$.
% $\sum_{i=1}^{N}P_{e,i}(\delta)=\sum_{i=1}^{N}P_{e,i}(\delta^*)=0$, and $\sum_{i=1}^{N}\sum_{j=1}^NB_{ij}\cos(\delta_{ij})\left(M_i(\omega_i-\omega^*)-M_j(\omega_j-\omega^*)\right)=0$
% where $\xi_i=\sum_{j=1}^{N}B_{ij}\left(  \sin(\delta_{ij})-\sin(\delta_{ij}^*)\right)$.
% Let $k_i(\omega_i)= \left(u_i(\omega_i)-u_i(\omega_i^*)\right)/\left(\omega_i-\omega_i^*\right)$
% if $\omega_i\neq\omega_i^*$ and $k_i(\omega_i)=0$ if $\omega_i=\omega_i^*$. Denote $\mathbf{K(\omega)}=\text{diag}(k_1(\omega_1),\cdots,k_N(\omega_N))$ and thus $u_(\omega)-u(\omega^*)=\mathbf{K(\omega)}(\omega-\omega^*)$. Let $\mathbf{M}=\text{diag}(M_1,\cdots,M_N)$ and $\mathbf{D}=\text{diag}(D_1,\cdots,D_N)$, $\chi =\text{col}(P_e(\delta)-P_e(\delta^*), \omega-\omega^*)$, Lemma~\ref{lemma: dot_V} shows that
% \begin{equation}
% \dot{V}(\delta,\omega) &=- \chi^\top\left( \mathbf{\hat{Q}}+\mathbf{\Delta Q}\right)\chi
% \end{equation}
% where
% \begin{equation}
% \mathbf{Q}=
%     &\begin{bmatrix}
% \epsilon\mathbf{I}  & \frac{1}{2}\epsilon(\mathbf{D}+\mathbf{K(\omega)}) \\  \frac{1}{2}\epsilon(\mathbf{D}+\mathbf{K(\omega)})  & (\mathbf{D}+\mathbf{K(\omega)})-\frac{\epsilon}{2}(\mathbf{H(\delta)}\mathbf{M}+\mathbf{M}\mathbf{H(\delta)})
% \end{bmatrix} 
% \end{equation}
% \begin{equation*}
% \mathbf{\Delta Q}=
%     &\begin{bmatrix}
% \mathbf{0}  & \frac{1}{2}\epsilon\mathbf{K(\omega)} \\  \frac{1}{2}\epsilon\mathbf{K(\omega)}  & \mathbf{K(\omega)} 
% \end{bmatrix} ,
% \end{equation*}
% \begin{equation}\label{eq:hat_Q}
% \mathbf{\hat{Q}}=
%     &\begin{bmatrix}
% \epsilon\mathbf{I}  & \frac{1}{2}\epsilon\mathbf{D} \\  \frac{1}{2}\epsilon\mathbf{D}  & \mathbf{D}-\frac{\epsilon}{2}(\mathbf{H(\delta)}\mathbf{M}+\mathbf{M}\mathbf{H(\delta)})
% \end{bmatrix} ,
% \end{equation}
% and $\mathbf{H(\delta)}\succeq0$ is a graph Laplacian matrix (details can be found in Lemma~\ref{lemma: dot_V}). By Lemma~\ref{lemma:Bounded_Lyapunov}, there exists a positive constant $c$ such that $\chi^\top \mathbf{\hat{Q}}\chi\leq -c\dot{V}(\delta, \omega)$.
%Hence,  $\chi^\top \mathbf{\hat{Q}}\chi\leq -\beta_4||\chi||^2_2 $ where $\beta_4:=\min_{\delta\in \Theta }\lambda_{min}\left(\mathbf{\hat{Q}}\right).$
% By Lemma~\ref{lemma:bound_potential_func}, there exists a constant $\beta_3^\prime$ such that
% \begin{equation}
%     ||P_e(\delta)-P_e(\delta^*)||^2_2\geq \beta_3^\prime||\delta-\delta^*||_2^2
% \end{equation}
% Then $||\chi||^2_2=||P_e(\delta)-P_e(\delta^*)||^2_2 +||\omega_i-\omega_i^*||^2_2\geq \min(1, \beta_3^\prime)(||\delta-\delta^*||^2_2 +||\omega_i-\omega_i^*||^2_2) $. Hence, $||\chi||^2_2\geq \beta_3(||\delta-\delta^*||^2_2 +||\omega_i-\omega_i^*||^2_2)$ where $\beta_3:= \min(1, \beta_3^\prime).$ 
%Therefore $\chi^\top \mathbf{\hat{Q}}\chi\leq -\beta_4||\chi||^2_2 \leq -\beta_3\beta_4(||\delta-\delta^*||^2_2 +||\omega_i-\omega_i^*||^2_2)\leq -\frac{\beta_3\beta_4}{\beta_2}V(\delta,\omega).$ We finish the proof by taking $c=\frac{\beta_3\beta_4}{\beta_2}$.
% Note that $\mathbf{K(\omega)}$ depends on the learned controller. To elimate such dependence in proof, we define 
%When $u_i(\omega_i)$ are monotonically increasing with respect to $\omega_i$ for all $i=1,\cdots,N$, we have $\mathbf{K(\omega)}\succeq 0$. Hence, $- \chi^\top\mathbf{\Delta Q}\chi=(\omega-\omega^*)^\top\mathbf{K(\omega)}(\omega-\omega^*)+\epsilon (\omega-\omega^*)^\top\mathbf{K(\omega)} \left(P_e(\delta)-P_e(\delta^*)\right)\leq 0$ for sufficiently small $\epsilon$.  Therefore , $\dot{V}(\delta,\omega)\leq\chi^\top \mathbf{\hat{Q}}\chi\leq -c\dot{V}(\delta, \omega)$ and thus the equilibrium is exponential stable.
% The equilibrium is locally asymptotically stable when $\dot{V}(\delta,\omega)\leq 0$ with equality only reached at the equilibrium. If the function $u_i(\omega_i)$ monotonic increases with $\omega_i$, then $u_i(\omega_i)\geq u_i(\omega^*)$ is the same sign with $(\omega_i\geq\omega^*$ for all $i=1,\cdots,N$. 
% Since $\D_i\geq 0$ abd $\sum_{i=1}^ND_i>0$, we have\eqref{eq: Lyapunov_derivative}, $\dot{V}(\delta,\omega)< 0$ for $\omega_i\neq \omega^*$. 
% Note this condition is distributed in the sense that it needs to be satisfied at each of the buses. 
% , in the sense that it is only for each of  In this way, stability requirement of the total system can be satisfied by the constraint on the action of each bus distributively.
% By the Krasovski-Lasalle principle~\cite{aastrom2010feedback}, the constraint on control action can be further relaxed to include equality, i.e.,  $\omega_i u_i(\omega_i) \geq 0$.
% Define the set $S=\left\{(\delta,\omega) \in \Omega_{r}: \dot{V}(\delta,\omega)=0\right\}$ where the derivative of  Lyapunov equals to zero. For a trajectory to remain
% in this set we must have $\omega_i = 0$ or $u_i(\omega_i)=0$. 
% Consider one point where $\omega_i \neq 0$ while $u_i(\omega_i)=0$. Using the dynamics \eqref{subeq:Dynamic_delta} we have $\dot{\delta_i}\neq 0$, this implies that $\dot{\omega_i}\neq 0$ if $u_i(\omega_i)=0$. Therefore, points with $\omega_i \neq 0$ are not in the invariant set inside $S$. In other words, $S$ contains no invariant sets other than the states that $w_i=0$.  Then from the  Krasovski-Lasalle principle, we can conclude that the state $(\delta,\omega)$ where $w_{i}=0$ and $P_{i}= \sum_{j=1}^{N} B_{ij} \sin(\delta_i-\delta_j)$  for $(i, j) \in \mathcal{E},$ is locally asymptotically stable. 
\end{proof}

The qualifier ``local'' in Theorem~\ref{theorem:Exponential_stable} is important since we need to assume that the trajectories start within a bounded region of the equilibrium point. This region has no constraints on $\omega$, and requires $\delta$ constrained in the region denoted by $\Theta :=\left \{\delta| \delta_i-\delta_j \in \left(-\frac{\pi}{2}, \frac{\pi}{2}\right) \right \}$ ~\cite{weitenberg2018robust}, which is sufficiently large to include almost all practical scenarios.
% Note that the small positive constant $\rho$ is utilized as  an extra margin on the constraint to quantify the decay of the Lyapunov function we will use to derive a  stabilizing controller. 
% The region is sufficiently large to include almost all practical scenarios.
% This region is derived based on well understood power system energy (or Lyapunov) functions~\cite{arapostathis1982global,dobson1989towards,chang1995direct,vu2015lyapunov} and can be explicitly characterized. 
% The region is quite large, since it includes all states where $\delta_i$ that satisfy $|\delta_i-\delta_j|\in [0,\pi/2)$ (no constraints on $\omega$), which include almost all practical scenarios.
% ~(see Appendix~\ref{app:region} for more details). 
% The next theorem shows that if controllers have more structure, a desirable rate of convergence can be obtained.
% \begin{theorem}\label{theorem:Exponential_stable}
% If the control function $u_i(\omega_i)$ are monotonically increasing with respect to $\omega_i$ for all $i=1,\cdots,N$, then the equilibrium point is locally exponentially stable.
% \end{theorem}
Theorem~\ref{theorem:Exponential_stable} gives structural properties\footnote{These are sometimes called extended class $\kappa$ functions} for controllers that guarantee exponential stability for \emph{all system parameter and topologies}. Namely, if the controllers satisfy the conditions in the theorems, they would be locally stabilizing for any network. Therefore, the optimal performance comes from training on a particular network, but the stability guarantees do not. This robustness to uncertainties is a key advantage of defining the structure of networks compared to purely model-free RL approaches. 

The design of neural networks that satisfy these properties is given in the next section (Section~\ref{sec:design}). %The proof of 
% Theorem~\ref{theorem:Asymptotic_stable} is given below and the proof of 
%Theorem~\ref{theorem:Exponential_stable} is given below.
% in the Appendix~\ref{appendices:Monotonic_Function}. 

\subsection{Design of Neural Network Controllers} \label{sec:design}
In this paper, we parametrize the controllers $u_i$ by a single hidden layer neural network. 
We assume that the processes such as automatic generation
control (AGC) adjust the power setpoint of generators to make the net power injection around zero, i.e., $\sum_{i=1}^{N}P_{m,i}=0$. For controllers $u(\omega)$ that provide primary frequency response, we let function $u(0)=0$ to make zero action when there is no frequency deviation. 
By Theorem
% s~\ref{theorem:Asymptotic_stable} and
~\ref{theorem:Exponential_stable}, we design the weights and the biases of the neural networks to have the following structures \highlight{such that  the controller will be locally exponentially stabilizing}:
% To incorporate the inequality constraints \eqref{subeq:Discrete_optimization_bound}-\eqref{subeq:Discrete_optimization_Mono} on control action, we aim to design the neural network structure for control function at each bus that satisfy:
\begin{enumerate}
    % \item $u_{\varphi_i}(\omega_i)$ has the same sign as $\omega_i$ 
    \item $u_{\varphi_i}(\omega_i)$ is monotonically increasing
    \item $u_{\varphi_i}(\omega_i)=0$ for $\omega_i=0$
    \item  $\underline{u}_i \leq u_{\varphi_i}(\omega_i)\leq \overline{u}_i$ (saturation constraints) 
\end{enumerate}
%The first two requirement is equivalent to design a monotonic increasing function through the origin. Note the the rectified linear unit (ReLU) function $\sigma(x)$ is linear with $x$ when activated $(x>0)$ and equals to zero when $(x\leq0)$, we construct the monotonic increasing function through the origin by stacking the ReLU function using: 
%\begin{equation}\label{eq:Mono_u}
%    u_i(\omega_i)=Q_i^+\sigma(\mathbf{1}w_i+b_i^+)+Q_i^-\sigma(\mathbf{1}w_i+b_i^-)
%\end{equation}  
%where $Q_i^+$ is the weights vector of bus $i$ and $Q_i^+=[q_i^1,q_i^2,\cdots,q_i^m]^\intercal$; $b_i$ is the bias vector of bus $i$ and $b_i^+=[b_i^1,b_i^2,\cdots,b_i^m]^\intercal$. $\sigma$ stands for the element-wise ReLU operator. $\mathbf{1}\in \mathbb{R}^m$ is the column vector where all the element is one. \\



The first two requirements are equivalent to designing a monotonic increasing function through the origin. This is constructed by decomposing the function into positive and negative parts as $f_i(\omega_i)=f_i^+(\omega_i)+f_i^-(\omega_i)$, where $f_i^+(\omega_i)$ is monotonic increasing for $\omega_i>0$ and zero when $\omega_i\leq0$; $f_i^-(\omega_i)$ is monotonic increasing for $\omega_i<0$ and zero when $\omega_i\geq0$. The saturation constraints can be satisfied by hard thresholding the output of the neural network. 


The function $f_i^+(\omega_i)$ and $f_i^-(\omega_i)$ are constructed using a single-layer neural network designed by stacking the ReLU function. Let $m$ be the number of hidden units. For $f_i^+(\omega_i)$, let  $q_i=[\begin{matrix}
 q_i^{1}& q_i^{2} & \cdots&q_i^{m}
\end{matrix}]$ be the weight vector of bus $i$; $b_i=[\begin{matrix} b_i^{1}& b_i^{2} & \cdots &b_i^{m}\end{matrix}]^\intercal$ be the corresponding bias vector. For $f_i^-(\omega_i)$, let $z_i=[\begin{matrix} z_i^{1}&z_i^{2}&\cdots&z_i^{m}\end{matrix}]$ be the weights vector and $c_i=[\begin{matrix} c_i^{1}& c_i^{2} & \cdots & c_i^{m}\end{matrix}]^\intercal$ be the bias vector. Denote $\mathbf{1}\in \mathbb{R}^m$ as the all $1$'s column vector. The detailed construction of $f_i^+(\omega_i)$ and $f_i^-(\omega_i)$ is given in Lemma~\ref{lemma:u_f+}. 
\begin{lemma}\label{lemma:u_f+}
Let $\sigma(x)=\max(x,0)$ be the ReLU function.  The stacked ReLU function constructed by \eqref{eq:f+} is monotonic increasing for $\omega_i>0$ and zero when $\omega_i\leq 0$.
\begin{subequations}\label{eq:f+}
\begin{align}
     &f_i^+(\omega_i)=q_i\sigma(\mathbf{1}\omega_i+b_i)\\
     \mbox{where }
     &\sum_{j=1}^{l} q_i^{j}\geq 0, \quad \forall l=1,2,\cdots,m
     \label{eq:f+2}\\
     & b_i^{1}=0, b_i^{l}\leq b_i^{(l-1)}, \quad \forall l=2,3,\cdots,m\label{eq:f+3}
\end{align}
\end{subequations}
 The stacked ReLU function constructed by \eqref{eq:f-} is monotonic increasing for $\omega_i< 0$ and zero when $\omega_i\geq 0$.
\begin{subequations}\label{eq:f-}
\begin{align}
     &f_i^-(\omega_i)=z_i\sigma(-\mathbf{1}\omega_i+c_i)\\
     \mbox{where } 
     &\sum_{j=1}^{l} z_i^{j}\leq 0, \quad \forall l=1,2,\cdots,m\label{eq:f-2}\\
     & c_i^{1}=0, c_i^{l}\leq c_i^{(l-1)}, \quad \forall l=2,3,\cdots,m\label{eq:f-3}
\end{align}
\end{subequations}
\end{lemma}


\begin{proof}
 Note that the ReLU function $\sigma(x)$ is linear with $x$ when activated $(x>0)$ and equals to zero when deactivated $(x \leq 0)$, we construct the monotonic increasing function $f_i^+(\omega_i)$ by stacking the function $g_i^l(\omega_i)=q_i^{l}\sigma(\omega_i+b_i^{l})$ as illustrated by Fig.~\ref{fig:Mono_Structure}. Since 
$b_i^{1+}=0$ and $b_i^{l+}\leq b_i^{(l-1)+}, \forall 1\leq l \leq m$, $g_i^l(\omega_i)$  is activated in sequence from $g_i^1(\omega_i)$ to $g_i^m(\omega_i)$ with the increase of $\omega_i$. In this way, the stacked function is a piece-wise linear function and the slope for each piece is $\sum_{j=1}^{l} q_i^j$. 
Monotonic property can be satisfied as long as the slope of all the pieces are positive, i.e., $\sum_{j=1}^{l} q_i^l\geq 0, \forall 1\leq l \leq m$. Similarly, $f_i^-(\omega_i)$ also construct by ReLU function activated for negative $w_i$ in sequence corresponding to $c_i^l$ for $l=1,\cdots,m$. $\sum_{j=1}^{l} z_i^{j}\leq 0$ means that all the slop of the piece-wise linear function is positive and therefore guarantees monotone.
\begin{figure}[t]	
	\centering
	\includegraphics[scale=0.68]{Mono_Structure.png}
	\caption{Stacked ReLU neural network to formulate a monotonic increasing function through the origin}
	\label{fig:Mono_Structure}
\end{figure}
\end{proof}
Note that there still exists inequality constraints in \eqref{eq:f+} and \eqref{eq:f-}, which makes the training of the neural networks cumbersome.  We can reformulate the weights to get a equivalent representation that is easier to deal with in training. Define the non-negative vectors $\hat{q}_i=\left[\begin{matrix} \hat{q}_i^{1}&\cdots&\hat{q}_i^{m}\end{matrix}\right]$ and $\hat{b}_i=\left[\begin{matrix}\hat{b}_i^{1}&\cdots&\hat{b}_i^{m}\end{matrix}\right]^\intercal$. Then, \eqref{eq:f+2} is satisfied if $q_i^{1}=\hat{q}_i^{1}$, $q_i^{l}=\hat{q}_i^{l}-\hat{q}_i^{(l-1)}$ for  $l=2,\cdots,m$. \eqref{eq:f+3} is satisfied if $b_i^{1}=0$, $ b_i^{l}=-\sum_{j=2}^{l} \hat{b}_i^{j}$ for  $l=2,\cdots,m$. 
Similarly, define $\hat{z}_i=\left[\begin{matrix}\hat{z}_i^{1}&\cdots&\hat{z}_i^{m}\end{matrix}\right]\geq 0$  and $\hat{c}_i=\left[\begin{matrix}\hat{c}_i^{1}&\cdots&\hat{c}_i^{m}\end{matrix}\right]^\intercal\geq 0$. Then, \eqref{eq:f-2} is satisfied if $z_i^{1}=-\hat{z}_i^{1}$, $ z_i^{l}=-\hat{z}_i^{l}+\hat{z}_i^{(l-1)}$ for  $l=2,\cdots,m$. \eqref{eq:f-3} is satisfied if $c_i^{1}=0$, $ c_i^{l}=-\sum_{j=2}^{l} \hat{c}_i^{l}$ for  $l=2,\cdots,m$. If the dead-band of the frequency deviation within the range $[-d,d]$ is required, it can be easily satisfied by setting $b_i^2=-d, q_i^1=0$ and  $c_i^2=-d, z_i^1=0$ in \eqref{eq:f+} and \eqref{eq:f-}.\footnote{A deadband is often enforced for generator droop control to reduce mechanical stress. For inverters, we do not do not set mandatory dead-band.}

The next Theorem states the converse of Lemma~\ref{lemma:u_f+}, that is, the constructions in \eqref{eq:f+} and \eqref{eq:f-} suffice to approximate all functions of interest. 
\begin{theorem}\label{theorem:Universial Approximation}
Let $r(x)$ be any continuous, Lipschitz and bounded monotonic function through the origin with bounded derivatives, mapping compact set $\mathbb{X}$ to  $ \mathbb{R}$.  Then there exists a function $f(x)=f^+(x)+f^-(x)$ constructed by \eqref{eq:f+} and \eqref{eq:f-} such that, for any $\epsilon$ and any $x \in \mathbb{X}$, $\left|r(x)-f(x)\right|<\epsilon$. 
\end{theorem}

The proof is given in Appendix~\ref{appendices:stacked-ReLU}. Note that $f(x)$ is a single-layer neural network. When approximating an arbitrary function, the number of neurons and the height will depend on $\epsilon$.
Since the controller in this paper is bounded, the stacked-ReLU neural network with limited number of neurons is sufficient for parameterization. The last step is to bound the output of the neural networks, which can be done easily using ReLU activation functions. 
\begin{lemma}\label{lemma:u_f+-}
 The neural network controller $u_i$ given below is a monotonic increasing function through the origin and bounded in $[\underline{u}_i, \overline{u}_i]$ for all $i=1,\cdots,N$:
\begin{equation}\label{eq:u_f+-}
\begin{split}
    u_i(\omega_i)=&\overline{u}_i-\sigma(\overline{u}_i -f_i^+(\omega_i)-f_i^-(\omega_i))\\
    &+\sigma(\underline{u}_i -f_i^+(\omega_i)-f_i^-(\omega_i))
\end{split}
\end{equation}
\end{lemma}
The proof of this lemma is by inspection. 

% Note that the construction \eqref{eq:u_f+-} is equivalent to the function $f(\omega_i)$ bounded by $\left[\overline{u}_i,\underline{u}_i\right]$. This means that the control network for $u_i(\omega_i)$ can universally approximate any function that fulfills the three constraints \eqref{subeq:Discrete_optimization_bound}-\eqref{subeq:Discrete_optimization_Mono}. 
% Furthermore, requirement 3) is accomplished by the hard constraints imposed by  the rectified linear unit (ReLU) function $\sigma(x)=\max(0,x)$. We firstly 
% elaborate the construction of neural network controller by Lemma~\ref{lemma:u_f+-}-Lemma~\ref{lemma:u_f-}.  Then we show by Theorem~\ref{theorem:Universial Approximation} that   
% the proposed construction can universally approximate any functions that fulfill the three requirements. 







%Theorem~\ref{theorem:Universial Approximation} states that the proposed structure in Lemma~\ref{lemma:u_f+-} can universally approximate any function satisfy the three requirements. 




%(**The following one paragraph is copied from the book \cite{aastrom2010feedback}. This may be attached in Appendix)
%Theorem (Krasovski-Lasalle principle). Let $V: \mathbb{R}^{n} \rightarrow \mathbb{R}$ be a locally positive definite function such that on the compact set $\Omega_{r}=\left\{x \in \mathbb{R}^{n}: V(x) \leq r\right\}$ we have $\dot{V}(x) \leq 0 .$ Define
%\[
%S=\left\{x \in \Omega_{r}: \dot{V}(x)=0\right\}
%\]
%As $t \rightarrow \infty,$ the trajectory tends to the largest invariant set inside $S ;$ i.e., its $\omega$ limit set is contained inside the largest invariant set in S. In particular, if $S$ contains $\mathrm{no}$ invariant sets other than $x=0,$ then 0 is asymptotically stable. 


%\subsection{Monotonic function requirement from optimality condition}\label{section:Monotonic_function}
%In order to further realize exponential stability, we enforce that the control function $u_i(\omega_i)$ for each bus $i$ is monotonic increasing with $\omega_i$. We prove that monotonic increasing control function is a sufficient condition for exponential stability as follows.




